Minimal Session Types for the $\pi$-calculus (Extended Version)

Session types are a discipline for the static verification of message-passing programs. A session type specifies a channel's protocol as sequences of exchanges. It is most relevant to investigate session-based concurrency by identifying the essential notions that enable program specification and verification. Following that perspective, prior work identified minimal session types (MSTs), a sub-class of session types without the sequentiality construct, which specifies the structure of communication actions. This formulation of session types led to establish a minimality result: every process typable with standard session types can be compiled down to a process typable using MSTs, which mimics sequentiality in types via additional process synchronizations. Such a minimality result is significant because it justifies session types in terms of themselves, without resorting to external notions; it was proven for a higher-order session pi-calculus, in which values are abstractions (functions from names to processes). In this paper, we study MSTs and their associated minimality result but now for the session pi-calculus, the (first-order) language in which values are names and for which session types have been more widely studied. We first show that this new minimality result can be obtained by composing known results. Then, we develop optimizations of this new minimality result and prove that the associated transformation into processes with MSTs satisfies dynamic correctness.

==> macros/macros-pi-thesis.tex <==


\newcommand{\ltenc}[1]{\map{#1}}
\newcommand{\proveslt}{\proves^{\mathsf{t}}}


\newcommand{\ltab}[1]{l_{\#}[#1]}
\newcommand{\lti}[1]{l_{\mathtt{i}}[#1]}
\newcommand{\lto}[1]{l_{\mathtt{o}}[#1]}
\newcommand{\ltend}{\varnothing[]}
\newcommand{\lttcase}[3]{\langle #1 : #2 \rangle_{i \in I}}
\newcommand{\ltbra}{\langle l_i : \tau_i\rangle_{i \in I}}
\newcommand{\ltcase}[5]{\textbf{case} \ #1 \ \textbf{of}
\ \{#2\_(#3) \triangleright #4\}_{#5}}

\newcommand{\ltc}[1]{\#[#1]}


\makeatletter
\@ifpackageloaded{stix}{%
}{%
  \DeclareFontEncoding{LS2}{}{\noaccents@}
  \DeclareFontSubstitution{LS2}{stix}{m}{n}
  \DeclareSymbolFont{stix@largesymbols}{LS2}{stixex}{m}{n}
  \SetSymbolFont{stix@largesymbols}{bold}{LS2}{stixex}{b}{n}
  \DeclareMathDelimiter{\lBrace}{\mathopen} {stix@largesymbols}{"E8}%
                                            {stix@largesymbols}{"0E}
  \DeclareMathDelimiter{\rBrace}{\mathclose}{stix@largesymbols}{"E9}%
                                            {stix@largesymbols}{"0F}
}
\makeatother
\newcommand{\ltencr}[1]{\lBrace #1 \rBrace}
\newcommand{\ltencrun}[1]{\lBrace #1 \rBrace^{\mathtt{un}}}
\newcommand{\ltencrlin}[1]{\lBrace #1 \rBrace^{\mathtt{lin}}}

\newcommand{\un}[1]{\ensuremath{\mathtt{un}(#1)}}
% \{\!\!\{

% \newcommand{\ltencr}[1]{\{\!\{ #1 \}\!\}}

\newcommand{\ltvar}[2]{#1 \_ #2}



\newcommand{\Boptsb}[3]{\textcolor{\decoptcolor}{\mathbb{A}^{\textsf{sb}}}^{#1}_{#2}\textcolor{\decoptcolor}{\big(}#3\textcolor{\decoptcolor}{\big)}}

==> macros/macros-pi2.tex <==

%%% Possible options:
% ACMBlue, ACMYellow, ACMOrange, ACMRed, ACMLightBlue, ACMGreen, ACMPurple and ACMDarkBlue
% \newcommand{\deccolor}{ACMRed}
\newcommand{\deccolor}{red}
% \newcommand{\decoptcolor}{ACMDarkBlue}
\newcommand{\decoptcolor}{blue}

\newcommand{\jcheck}[1]{\textcolor{red}{#1}}
\newcommand{\acheck}[1]{\textcolor{blue}{#1}}
%% START Macros by Amelia
\newcommand{\Amelia}[3]{\textcolor{\deccolor}{\mathcal{A'}}^{#1}_{#2}\textcolor{\deccolor}{\big(}#3\textcolor{\deccolor}{\big)}}
\newcommand{\AmeliaMod}[3]{\textcolor{\deccolor}{\mathcal{A}}^{#1}_{#2}\textcolor{\deccolor}{\big(}#3\textcolor{\deccolor}{\big)}}
%\newcommand{\D}[1]{\mathcal{D}(#1)}
\newcommand{\F}[1]{\textcolor{\deccolor}{\mathcal{F}(}#1\textcolor{\deccolor}{)}}
\newcommand{\Do}[1]{\textcolor{\decoptcolor}{\mathcal{F}^\ast(}#1\textcolor{\decoptcolor}{)}}
\newcommand{\msessp}{\ensuremath{\mu\pi}\xspace}

% TODO: check this 
% \newcommand{\mGt}[1]{\mathcal{H}(#1)}
\newcommand{\mGt}[1]{\textcolor{\deccolor}{\mathcal{H}(}#1\textcolor{\deccolor}{)}}
\newcommand{\Gtopt}[1]{\textcolor{\decoptcolor}{\mathcal{H}}^{\textcolor{\decoptcolor}{*}}\textcolor{\decoptcolor}{(}#1\textcolor{\decoptcolor}{)}}

\newcommand{\mRt}[1]{\textcolor{\deccolor}{\mathcal{R'}(}#1\textcolor{\deccolor}{)}}
\newcommand{\mRts}[3]{\textcolor{\deccolor}{\mathcal{R'}^{\star}(}#3\textcolor{\deccolor}{)}}
% \newcommand{\envPropR}{\Phi}



% COMMANDS 

\newcommand{\hidejp}[1]{}

\newcommand{\B}[3]{\mathcal{B}^{#1}_{#2}\big(#3\big)}
\newcommand{\mB}[3]{\mathsf{B}^{#1}_{#2}\big(#3\big)}
\newcommand{\V}[3]{\mathcal{V}^{#1}_{#2}\big(#3\big)}
\newcommand{\mV}[3]{\mathsf{V}^{#1}_{#2}\big(#3\big)}
\newcommand{\Gt}[1]{\mathcal{G}(#1)}
\newcommand{\Rt}[1]{\mathcal{R}(#1)}
\newcommand{\Rts}[3]{\mathcal{R}^{\star}(#3)}
\newcommand{\envR}{\Delta_\mu}
\newcommand{\thetaR}{\Theta_\mu}
\newcommand{\thetax}{\Theta_{\rvar{X}}}
\newcommand{\envPropR}{\Phi}
\newcommand{\D}[1]{\mathcal{D}(#1)}




\newcommand{\mD}[1]{\mathsf{D}(#1)}
\newcommand{\len}[1]{|#1|}
\newcommand{\incrname}[2]{\subst{#1_{#2+1}}{#1_#2}}
\newcommand{\eqprm}{\equiv_{p}}
\newcommand{\prop}{c}
\newcommand{\apropinp}[1]{\abinp{\prop_{#1}}}
\newcommand{\propinp}[1]{\binp{\prop_{#1}}}
\newcommand{\propinpx}[1]{\binp{x_{\prop_{#1}}}}
\newcommand{\propout}[1]{\bout{\dual{\prop_{#1}}}}
\newcommand{\apropout}[1]{\about{\dual{\prop_{#1}}}}
\newcommand{\proprinp}[1]{\binp{\prop^{#1}}}
\newcommand{\proprout}[1]{\bout{\prop^{#1}}}
\newcommand{\proprinpk}[2]{\binp{\prop^{#1}_{#2}}}
\newcommand{\proproutk}[2]{\bout{\dual {\prop^{#1}_{#2}}}}
\newcommand{\aproprout}[1]{\about{\prop^{#1}}}
\newcommand{\propoutx}[1]{\bout{\dual{x_{\prop_{#1}}}}}
\newcommand{\propbout}[1]{\bbout{\dual{\prop_{#1}}}}
\newcommand{\apropbout}[1]{\abbout{\dual{\prop_{#1}}}}

\newcommand{\propinprec}[1]{\binp{\prop^r_{#1}}}
\newcommand{\apropinprec}[1]{\abinp{\prop^r_{#1}}}
\newcommand{\apropoutrec}[1]{\about{\dual{\prop^r_{#1}}}}
\newcommand{\propoutrec}[1]{\bout{\dual{\prop^r_{#1}}}}

\newcommand{\propinprecsh}[1]{\binp{\prop^r_{#1}}}
\newcommand{\apropinprecsh}[1]{\abinp{\prop^r_{#1}}}
\newcommand{\propoutrecsh}[1]{\bout{{\prop^r_{#1}}}}
\newcommand{\apropoutrecsh}[1]{\about{\prop^r_{#1}}}

\newcommand{\psb}{\mathtt{\sessp^{sb}}}
\newcommand{\psr}{\mathtt{\sessp^{sr}}}

\newcommand{\unaryint}[1]{\ensuremath{\textsf{odd}(#1)}}

\newcommand{\Bsimple}[1]{\mathsf{B}(#1)}

\newcommand{\lin}[1]{\mathtt{lin}(#1)}
\newcommand{\sh}[1]{\mathtt{sh}(#1)}

% TODO 
\newcommand{\propsel}[2]{\bsel{\dual{\prop_{#1}}}{#2}}
\newcommand{\propbra}[2]{\bbra{\prop_{#1}}{#2}}

\newcommand{\slhotup}[1]{{#1}^{\leadsto}}
\newcommand{\slhot}[1]{{#1} \leadsto \diamond}
\newcommand{\degree}{l}
\newcommand{\thunk}[1]{\{\!\{#1\}\!\}}
\newcommand{\appthunk}[1]{\mathtt{run}\,{#1}}
%\newcommand{\appendx}[1]{}
\newcommand{\appendx}[1]{#1}

\newcommand{\mugamma}{\gamma}
\newcommand{\misty}{\textsf{MISTY}\xspace}




\newcommand{\fnb}[2]{\mathtt{fnb}(#1,#2)}
\newcommand{\Brec}[3]{\textcolor{\decoptcolor}{\mathbb{A}}^{#1}_{\textcolor{\decoptcolor}{\mathtt{rec}}~#2}\textcolor{\decoptcolor}{\big(}#3\textcolor{\decoptcolor}{\big)}}
\newcommand{\Rrec}[3]{\mathcal{R}^{#1}_{\mathtt{rec}#2}\big(#3\big)}
\newcommand{\Bsb}[3]{\mathcal{B}^{#1}_{\mathtt{sb} \ #2}\big(#3\big)}

\newcommand{\Bopt}[3]{\textcolor{\decoptcolor}{\mathbb{A}}^{#1}_{#2}\textcolor{\decoptcolor}{\big(}#3\textcolor{\decoptcolor}{\big)}}


\newcommand{\Brecd}[4]{\mathcal{B}^{#1}_{\mathtt{rec}#2}\big(#3\big)^{#4}}

\newcommand{\rvardepth}[1]{\ensuremath{\mathsf{recd}(#1)}}
\newcommand{\rvardepthaux}[1]{\ensuremath{\mathsf{recd}'(#1)}}

\newcommand{\Bbra}[3]{\mathcal{L}^{#1}_{#2}\big(#3\big)}
\newcommand{\Bbrafst}[3]{\mathcal{L}^{#1}_{#2}\big(#3\big)}
\newcommand{\Bbrasnd}[1]{\mathcal{R}(#1)}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\newcommand{\wtd}[1]{\widetilde{#1}}
\newcommand{\li}[1]{\widetilde{#1}}

\newcommand{\pfmap}{\Sigma}
\newcommand{\pfmapsmall}{\sigma}

% \newcommand{\lenHO}[1]{\lfloor #1 \rceil}
\newcommand{\lenHO}[1]{\textcolor{\deccolor}{\lfloor} #1 \textcolor{\deccolor}{\rceil}}
\newcommand{\lenHOopt}[1]{\textcolor{\decoptcolor}{\lfloor} #1 \textcolor{\decoptcolor}{\rceil^*}}

%\usepackage{accents}
\newcommand{\dbtilde}[1]{\widehat{#1}}
%\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}
%\newcommand{\dbtilde}[1]{\tilde{\raisebox{0pt}[0.85\height]{$\tilde{#1}$}}}

\newcommand{\indexed}[3]{\mathtt{indexed}_{#3}(#1,#2)}



% NEW COMMANDS FOR BISIMULATION 
\newcommand{\Cb}[3]{\mathcal{C}^{#1}_{#2}\big(#3\big)}
\newcommand{\Cbs}[3]{\widehat{\mathcal{C}}^{#1}_{#2}\big(#3\big)}
\newcommand{\Cbrec}[3]{\mathcal{C}^{#1}_{\mathsf{rec} \ #2}\big(#3\big)}
% \newcommand{\Cbs}[3]{\mathsf{C}^{#1}_{#2}\big(#3\big)}
\newcommand{\Cbsb}[3]{\mathcal{C}^{#1}_{\mathtt{sb} \ #2}\big(#3\big)}
\newcommand{\Dlet}{\mathcal{J}}
\newcommand{\Db}[3]{\Dlet^{#1}_{#2}\big(#3\big)}
\newcommand{\Dbrec}[3]{\Dlet^{#1}_{\mathsf{rec} \ #2}\big(#3\big)}
\newcommand{\Dset}{\Dlet}

\newcommand{\Dbsb}[3]{\Dlet^{#1}_{\mathtt{sb} \ #2}\big(#3\big)}

\newcommand{\fpn}[1]{\ensuremath{\mathsf{fpn}(#1)}}
\newcommand{\nextn}[1]{\ensuremath{\mathsf{next}(#1)}}

\newcommand{\indices}[1]{\ensuremath{\mathsf{index}(#1)}}
\newcommand{\bname}[1]{\ensuremath{\mathsf{bn}(#1)}}

\newcommand{\mstindex}{\ensuremath{l}}

% \usepackage{accents}

% \newcommand{\ddbtilde}[1]{\accentset{\approx}{#1}}
% \newcommand{\vardbtilde}[1]{\wtd{\raisebox{0pt}[0.85\height]{$\wtd{#1}$}}}

% \newcommand{\bns}[1]{\ensuremath{\mathtt{m}(#1)}}
% \newcommand{\wbns}[1]{\ensuremath{\vardbtilde {#1}}}

% \newcommand{\bns}[1]{\ensuremath{\ddbtilde {#1}}}
% \newcommand{\wbns}[1]{\ensuremath{\vardbtilde {#1}}}

% \newcommand{\bns}[1]{\ensuremath{\ddbtilde {#1}}}
% \newcommand{\wbns}[1]{\ensuremath{\vardbtilde {#1}}}

% \newcommand{\bns}[1]{\ensuremath{\tilde {#1}_{m}}}
% \newcommand{\wbns}[1]{\ensuremath{\wtd {#1}_{m}}}


% \newcommand{\bns}[1]{\ensuremath{\tilde {#1#1}}}
% \newcommand{\wbns}[1]{\ensuremath{\Hat {#1}}}

\newcommand{\bns}[1]{\ensuremath{\tilde {#1_*}}}
\newcommand{\wbns}[1]{\ensuremath{\widetilde {#1_*}}}

% \newcommand{\bns}[1]{\ensuremath{\tilde {#1_#1}}}
% \newcommand{\wbns}[1]{\ensuremath{\widetilde {#1_#1}}}

\newcommand{\iname}[1]{\ensuremath{\breve{#1}}}

\newcommand{\vrelate}{\bowtie}
\newcommand{\valuesrelate}{\bowtie_{\mathtt{c}}}

\newcommand{\highlighta}[1]{\colorbox{lightgray}{\ensuremath{#1}}}


% \newcommand{\rfni}[#1]{\mathtt{rfni}(P)}

\newcommand{\valuesrelatev}{\bowtie_{\mathcal{C}}}


% NEW COMMANDS 


\newcommand{\horelm}[5]{#1 \proves #2 #3 #4 \proves #5}
\newcommand{\mstb}{\approx^{\mathtt{M}}}

\newcommand{\numpropam}[1]{\textcolor{\deccolor}{\#(}#1\textcolor{\deccolor}{)}}
\newcommand{\numprop}[1]{\textcolor{\decoptcolor}{\#^*(}#1\textcolor{\decoptcolor}{)}}


\newcommand{\bbralts}[2]{#1 \& #2}
\newcommand{\bsellts}[2]{#1 \oplus #2}
\newcommand{\minnames}[2]{\langle #1 \rangle_{#2}}
\newcommand{\mapcharm}[2]{\langle #1 \rangle^{#2}}
\newcommand{\omapcharm}[1]{\langle #1 \rangle_{\texttt{c}}}

% \newcommand{\Rt}[1]{\textcolor{\decoptcolor}{\mathcal{R}(}#1\textcolor{\decoptcolor}{)}}
% \newcommand{\Rts}[3]{\textcolor{\decoptcolor}{\mathcal{R}^{\star}(}#3\textcolor{\decoptcolor}{)}}

\newcommand{\Rtopt}[1]{\textcolor{\decoptcolor}{\mathcal{R}(}#1\textcolor{\decoptcolor}{)}}
\newcommand{\Rtsopt}[3]{\textcolor{\decoptcolor}{\mathcal{R}^{\star}(}#3\textcolor{\decoptcolor}{)}}

\newcommand{\mhby}[1]{\hby{#1}_{\texttt m}}
\newcommand{\Mhby}[1]{\Hby{#1}_{\texttt m}}

\newcommand{\tr}{\mathsf{tr}}

\newcommand{\initname}[2]{\ensuremath{\subst{#1_{#2}}{#1}}}

\newcommand{\rulename}[2]{\langle \texttt{#1}#2 \rangle}

\newcommand{\Rb}[1]{\ensuremath{\mathcal{R}_{#1}}}

\newcommand{\mstpred}[1]{\textsf{m}(#1)}
\newcommand{\subl}[1]{\textsf{sub}(#1)}
\newcommand{\condpv}[2]{\textsf{cond}(#1,#2)}

\newcommand{\ftriggerm}[3]{#1 \Leftarrow_{\mathtt{m}} #2{\,:\,}#3}
\newcommand{\fotriggerm}[6]{\binp{#1}{#2} \newsp{#3}{\binp{#3}{\wtd y}  \mapcharm{#4}{y}_{#6} \Par \bout{\dual{#3}}{#5} \inact}}


\newcommand{\processrelate}{\diamond}

\newcommand{\rhom}{\ensuremath{\rho_{\mathtt m}}}

\newcommand{\sigmav}{\ensuremath{\sigma_v}}

\newcommand{\empg}{{}}

%\newcommand{\recpx}[1]{\ensuremath{\mathtt{\mathsf{X}}(#1)}}
\newcommand{\recpx}[1]{\ensuremath{\mathsf{frv}(#1)}}

\newcommand{\lenrecpx}[1]{\ensuremath{\#_X(#1)}}

\newcommand{\specx}{\ensuremath{\gamma}}

\newcommand{\recdep}{\ensuremath{d}}

%\newcommand{\lentr}[1]{\ensuremath{\len{#1}_{{tr}}}}
\newcommand{\lentr}[1]{\ensuremath{\mathsf{brn}(#1)}}



% \newcommand{\ppdp}{} 
\newcommand{\arxivlink}{https://arxiv.org/abs/2107.12345}

\newcommand{\longversion}[2]{\ifx\ppdp\undefined#1\else#2\fi}

\newcommand{\appnote}{\ifx\ppdp\undefined 
% ARXIV  
      \noindent \emph{Note:}   
      Due to space limits, 
      omitted  material (definitions, proofs, additional examples) can be found in the appendices. 
  \else 
    % PPDP 
    \noindent \emph{Note:}   
    Due to space limits, omitted material (definitions, proofs, additional examples) can 
    be found at \url{\arxivlink}. 
\fi 
}

\newcommand{\appnoteEx}
{\ifx\ppdp\undefined 
% ARXIV  
      \noindent The breakdown of $B'$ is similar and given in 
      \appref{ex:ex1-decomp}.
  \else 
    % PPDP 
    \noindent The breakdown of $B'$ is similar. 
\fi 
}

==> macros/macros-pi3.tex <==


\newcommand{\colorpro}{VioletRed}
\newcommand{\colortyp}{JungleGreen}

% \newcommand{\B}[3]{\mathcal{B}^{#1}_{#2}\big(#3\big)}
\newcommand{\B}[3]{\textcolor{\colorpro}{\mathcal{B}^{\textcolor{black}{#1}}_{\textcolor{black}{#2}}\big(\textcolor{black}{#3}\big)}}
% \newcommand{\mB}[3]{\mathsf{B}^{#1}_{#2}\big(#3\big)}
\newcommand{\mB}[3]{\textcolor{\colorpro}{\mathsf{B}^{\textcolor{black}{#1}}_{}\big(\textcolor{black}{#3}\big)}}
%
% \newcommand{\V}[3]{\mathcal{V}^{#1}_{#2}\big(#3\big)}
\newcommand{\V}[3]{\textcolor{\colorpro}{\mathcal{V}^{}_{\textcolor{black}{#2}}\big(\textcolor{black}{#3}\big)}}

% \newcommand{\mV}[3]{\mathsf{V}^{#1}_{#2}\big(#3\big)}
\newcommand{\mV}[3]{\textcolor{\colorpro}{\mathsf{V}^{#1}_{#2}\big(\textcolor{black}{#3}\big)}}

% \newcommand{\Gt}[1]{\mathcal{G}(#1)}
\newcommand{\Gt}[1]{\textcolor{\colortyp}{\mathcal{G}(\textcolor{black}{#1})}}
\newcommand{\D}[1]{\textcolor{\colorpro}{\mathcal{D}(\textcolor{black}{#1})}}
\newcommand{\indT}[1]{\textcolor{\colortyp}{[\textcolor{black}{#1}\rangle}}
\newcommand{\indTaux}[2]{\textcolor{\colortyp}{[\textcolor{black}{#1}\rangle^{\star}_{\textcolor{black}{#2}}}}

\newcommand{\Rt}[1]{\textcolor{\colortyp}{\mathcal{R}(\textcolor{black}{#1})}}
\newcommand{\Rts}[3]{\textcolor{\colortyp}{\mathcal{R}^{\star}(\textcolor{black}{#3})}}
\newcommand{\envR}{\Delta_\mu}
\newcommand{\envPropR}{\Phi}
\newcommand{\mD}[1]{\textcolor{\colorpro}{\mathsf{D}(\textcolor{black}{#1})}}
\newcommand{\plen}[1]{\textcolor{\colorpro}{\lbag \textcolor{black}{#1}\rbag }}
\newcommand{\len}[1]{|#1|}
\newcommand{\incrname}[2]{\subst{#1_{#2+1}}{#1_#2}}
\newcommand{\eqprm}{\equiv_{p}}
\newcommand{\prop}{c}
\newcommand{\apropinp}[1]{\abinp{\prop_{#1}}}
\newcommand{\propinp}[1]{\binp{\prop_{#1}}}

\newcommand{\propinpv}[1]{\binp{\prop{#1}}}
\newcommand{\propoutv}[1]{\bout{\dual{\prop{#1}}}}
\newcommand{\apropinpv}[1]{\abinp{\prop{#1}}}
\newcommand{\apropoutv}[1]{\about{\dual{\prop{#1}}}}


\newcommand{\propinpx}[1]{\binp{x_{\prop_{#1}}}}
\newcommand{\propout}[1]{\bout{\dual{\prop_{#1}}}}
\newcommand{\propoutt}[1]{\boutt{\dual{\prop_{#1}}}}
\newcommand{\apropout}[1]{\about{\dual{\prop_{#1}}}}
\newcommand{\proprinp}[1]{\binp{\prop^{#1}}}
\newcommand{\proprout}[1]{\bout{\prop^{#1}}}
\newcommand{\aproprout}[1]{\about{\prop^{#1}}}
\newcommand{\propoutx}[1]{\bout{\dual{x_{\prop_{#1}}}}}
\newcommand{\propbout}[1]{\bbout{\dual{\prop_{#1}}}}


\newcommand{\apropbout}[1]{\abbout{\dual{\prop_{#1}}}}
\newcommand{\slhotup}[1]{{#1}^{\leadsto}}


\newcommand{\cpropinp}[2]{\textcolor{gray1}{\binp{\prop_{#1}}{#2}}}
\newcommand{\capropout}[2]{\textcolor{gray1}{\apropout{#1}{#2}}}

\newcommand{\cbpropinp}[2]{\textcolor{orange!40!gray}{\binp{\prop_{#1}}{#2}}}
\newcommand{\cbpropout}[2]{\textcolor{orange!40!gray}{\bout{\dual{\prop_{#1}}}{#2}}}

\newcommand{\cbapropout}[2]{\textcolor{orange!40!gray}{\apropout{#1}{#2}}}

\newcommand{\slhot}[1]{{#1} \leadsto \diamond}
\newcommand{\degree}{l}
\newcommand{\thunk}[1]{\{\!\{#1\}\!\}}
\newcommand{\appthunk}[1]{\mathtt{run}\,{#1}}
%\newcommand{\appendx}[1]{}


\newcommand{\tr}{\mathsf{tr}}


\newcommand{\appendx}[1]{#1}

\newcommand{\mugamma}{\gamma}
\newcommand{\misty}{\textsf{MISTY}\xspace}


\newcommand{\nextn}[1]{\ensuremath{\mathsf{next}(#1)}}



\newcommand{\recursf}[1]{\mathtt{recur}(#1)}
\newcommand{\ctype}{\mathsf{cType}}

\newcommand{\lin}[1]{\mathsf{lin}(#1)}
\newcommand{\sh}[1]{\mathsf{sh}(#1)}


\newcommand{\blue}[1]{\textcolor{blue}{#1}}


\newcommand{\fpn}[1]{\ensuremath{\mathsf{fpn}(#1)}}



\newcommand{\wtd}[1]{\widetilde{#1}}



% ------------------------------------------------------------------------------
% BISIMULATION PROOF COMMANDS BEGIN 
\newcommand{\hidejp}[1]{}

\newcommand{\jpair}[2]{\ensuremath{\textcolor{red}{#1}~,~\textcolor{blue}{#2}} }

\newcommand{\Dlet}{\mathcal{J}}

\newcommand{\Db}[3]{\Dlet^{#1}_{#2}\big(#3\big)}
\newcommand{\Dset}{\Dlet}

\newcommand{\Clet}{\mathcal{C}}
\newcommand{\Cset}{\Clet}

\newcommand{\Cb}[3]{\mathcal{C}^{#1}_{#2}\big(#3\big)}
\newcommand{\Cbs}[3]{\widehat{\mathcal{C}}^{#1}_{#2}\big(#3\big)}
\newcommand{\Vb}[3]{\mathcal{C}^{#1}_{#2}\big(#3\big)}



\newcommand{\Cbrec}[3]{\mathcal{C}^{#1}_{\mathsf{rec} \ #2}\big(#3\big)}

\newcommand{\Cbr}[3]{\mathcal{C}^{R \ #1}_{#2}\big(#3\big)}


\newcommand{\Dbrec}[3]{\Dlet^{#1}_{\mathsf{rec} \ #2}\big(#3\big)}



\newcommand{\ftriggert}[2]{#1 \Leftarrow_{\mathtt{C}} #2}
\newcommand{\psb}{\mathtt{\sessp^{sb}}}
\newcommand{\psr}{\mathtt{\sessp^{sr}}}

\newcommand{\Bsimple}[1]{\mathsf{B}(#1)}

\newcommand{\propsel}[2]{\bsel{\dual{\prop_{#1}}}{#2}}
\newcommand{\propbra}[2]{\bbra{\prop_{#1}}{#2}}

\newcommand{\fnb}[2]{\mathtt{fnb}(#1,#2)}

\newcommand{\mstpred}[1]{\textsf{m}(#1)}
\newcommand{\subl}[1]{\textsf{sub}(#1)}
\newcommand{\condpv}[2]{\textsf{cond}(#1,#2)}


\newcommand{\vrelate}{\boxtimes}
\newcommand{\valuesrelate}{\bowtie}

\newcommand{\valuesrelatev}{\bowtie_{\mathcal{C}}}

\newcommand{\iname}[1]{\ensuremath{\breve{#1}}}
\newcommand{\processrelate}{\diamond}

\newcommand{\rfni}[1]{\ensuremath{\mathsf{rfni}(#1)}}
% \newcommand{\fpn}[1]{\ensuremath{\mathsf{fpn}(#1)}}

\newcommand{\fcr}[1]{\ensuremath{\mathsf{cr}(#1)}}

\newcommand{\highlighta}[1]{\colorbox{lightgray!60}{\ensuremath{#1}}}


\newcommand{\highlightb}[1]{\colorbox{lightblue}{\ensuremath{#1}}}

\newcommand{\indices}[1]{\ensuremath{\mathsf{index}(#1)}}
\newcommand{\idp}[1]{\ensuremath{\mathcal{I}(#1)}}


\newcommand{\initname}[2]{\ensuremath{\subst{#1_{#2}}{#1}}}

\newcommand{\rulename}[2]{\langle \texttt{#1}#2 \rangle}

\newcommand{\Rb}[1]{\ensuremath{\mathcal{R}_{#1}}}





\newcommand{\Se}{\relS}

\newcommand{\mstb}{\approx^{\mathtt{M}}}
\newcommand{\hob}{\approx^{\mathtt{H}}}

\newcommand{\bbralts}[2]{#1 \& #2}
\newcommand{\bsellts}[2]{#1 \oplus #2}
\newcommand{\minnames}[2]{\langle #1 \rangle_{#2}}
\newcommand{\mapcharm}[2]{\langle #1 \rangle^{#2}}
\newcommand{\omapcharm}[1]{\langle #1 \rangle}

\newcommand{\mhby}[1]{\hby{#1}_{\texttt m}}
\newcommand{\Mhby}[1]{\Hby{#1}_{\texttt m}}

\newcommand{\horelm}[5]{#1 \proves #2 #3 #4 \proves #5}



\newcommand{\complho}{\ensuremath{\HO^{\texttt{c}}}\xspace}


% name passing syntactic sugar 
\newcommand{\namepass}[1]{\ulcorner #1 \urcorner}
\newcommand{\namepasstyp}[1]{\llceil #1 \rrceil}

\newcommand{\plscheck}[1]{\textcolor{red}{#1}}
\newcommand{\subsqn}[1]{\ensuremath{\mathsf{next}(#1)}}
% BISIMULATION PROOF COMMANDS END
% ------------------------------------------------------------------------------


\newcommand{\recprov}[3]{\binp{\prop^{#1}}{#2}\appl{#2}{#3}}
\newcommand{\recprovx}[3]{\binp{\prop^{#1}}{#2}\appl{#2}{#3}}
\newcommand{\recpvar}[1]{#1}


\newcommand{\revisionc}[1]{#1} 

\newcommand{\revisionrem}{}{}

\excludecomment{revisionrem}
\newcommand{\revisioncheck}[1]{\textcolor{orange}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% first order 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Possible options:
% ACMBlue, ACMYellow, ACMOrange, ACMRed, ACMLightBlue, ACMGreen, ACMPurple and ACMDarkBlue
% \newcommand{\deccolor}{ACMRed}
\newcommand{\deccolor}{red}
% \newcommand{\decoptcolor}{ACMDarkBlue}
\newcommand{\decoptcolor}{blue}

\newcommand{\jcheck}[1]{\textcolor{red}{#1}}
\newcommand{\acheck}[1]{\textcolor{blue}{#1}}
%% START Macros by Amelia
\newcommand{\Amelia}[3]{\textcolor{\deccolor}{\mathcal{A'}}^{#1}_{#2}\textcolor{\deccolor}{\big(}#3\textcolor{\deccolor}{\big)}}
\newcommand{\AmeliaMod}[3]{\textcolor{\deccolor}{\mathcal{A}}^{#1}_{#2}\textcolor{\deccolor}{\big(}#3\textcolor{\deccolor}{\big)}}
%\newcommand{\D}[1]{\mathcal{D}(#1)}
\newcommand{\F}[1]{\textcolor{\deccolor}{\mathcal{F}(}#1\textcolor{\deccolor}{)}}
\newcommand{\Do}[1]{\textcolor{\decoptcolor}{\mathcal{F}^\ast(}#1\textcolor{\decoptcolor}{)}}
\newcommand{\msessp}{\ensuremath{\mu\pi}\xspace}

% TODO: check this 
% \newcommand{\mGt}[1]{\mathcal{H}(#1)}
\newcommand{\mGt}[1]{\textcolor{\deccolor}{\mathcal{H}(}#1\textcolor{\deccolor}{)}}
\newcommand{\Gtopt}[1]{\textcolor{\decoptcolor}{\mathcal{H}}^{\textcolor{\decoptcolor}{*}}\textcolor{\decoptcolor}{(}#1\textcolor{\decoptcolor}{)}}

\newcommand{\mRt}[1]{\textcolor{\deccolor}{\mathcal{R'}(}#1\textcolor{\deccolor}{)}}
\newcommand{\mRts}[3]{\textcolor{\deccolor}{\mathcal{R'}^{\star}(}#3\textcolor{\deccolor}{)}}
% \newcommand{\envPropR}{\Phi}



% COMMANDS 

% \newcommand{\hidejp}[1]{}

% \newcommand{\mB}[3]{\mathsf{B}^{#1}_{#2}\big(#3\big)}
% \newcommand{\V}[3]{\mathcal{V}^{#1}_{#2}\big(#3\big)}
% \newcommand{\mV}[3]{\mathsf{V}^{#1}_{#2}\big(#3\big)}
% \newcommand{\Gt}[1]{\mathcal{G}(#1)}
% \newcommand{\Rt}[1]{\mathcal{R}(#1)}
% \newcommand{\Rts}[3]{\mathcal{R}^{\star}(#3)}
% \newcommand{\envR}{\Delta_\mu}
\newcommand{\thetaR}{\Theta_\mu}
\newcommand{\thetax}{\Theta_{\rvar{X}}}
% \newcommand{\envPropR}{\Phi}
% \newcommand{\D}[1]{\mathcal{D}(#1)}




% \newcommand{\mD}[1]{\mathsf{D}(#1)}
% \newcommand{\len}[1]{|#1|}
% \newcommand{\incrname}[2]{\subst{#1_{#2+1}}{#1_#2}}
% \newcommand{\eqprm}{\equiv_{p}}
% \newcommand{\prop}{c}
% \newcommand{\apropinp}[1]{\abinp{\prop_{#1}}}
% \newcommand{\propinp}[1]{\binp{\prop_{#1}}}
% \newcommand{\propinpx}[1]{\binp{x_{\prop_{#1}}}}
% \newcommand{\propout}[1]{\bout{\dual{\prop_{#1}}}}
% \newcommand{\apropout}[1]{\about{\dual{\prop_{#1}}}}
% \newcommand{\proprinp}[1]{\binp{\prop^{#1}}}
% \newcommand{\proprout}[1]{\bout{\prop^{#1}}}
% \newcommand{\proprinpk}[2]{\binp{\prop^{#1}_{#2}}}
\newcommand{\proproutk}[2]{\bout{\dual {\prop^{#1}_{#2}}}}
% \newcommand{\aproprout}[1]{\about{\prop^{#1}}}
% \newcommand{\propoutx}[1]{\bout{\dual{x_{\prop_{#1}}}}}
% \newcommand{\propbout}[1]{\bbout{\dual{\prop_{#1}}}}
% \newcommand{\apropbout}[1]{\abbout{\dual{\prop_{#1}}}}

\newcommand{\propinprec}[1]{\binp{\prop^r_{#1}}}
\newcommand{\apropinprec}[1]{\abinp{\prop^r_{#1}}}
\newcommand{\apropoutrec}[1]{\about{\dual{\prop^r_{#1}}}}
\newcommand{\propoutrec}[1]{\bout{\dual{\prop^r_{#1}}}}

% \newcommand{\propinprecsh}[1]{\binp{\prop^r_{#1}}}
% \newcommand{\apropinprecsh}[1]{\abinp{\prop^r_{#1}}}
\newcommand{\propoutrecsh}[1]{\bout{{\prop^r_{#1}}}}
\newcommand{\apropoutrecsh}[1]{\about{\prop^r_{#1}}}

% \newcommand{\psb}{\mathtt{\sessp^{sb}}}
% \newcommand{\psr}{\mathtt{\sessp^{sr}}}

\newcommand{\unaryint}[1]{\ensuremath{\textsf{odd}(#1)}}

% \newcommand{\Bsimple}[1]{\mathsf{B}(#1)}

% \newcommand{\lin}[1]{\mathtt{lin}(#1)}
% \newcommand{\sh}[1]{\mathtt{sh}(#1)}


% \newcommand{\propsel}[2]{\bsel{\dual{\prop_{#1}}}{#2}}
% \newcommand{\propbra}[2]{\bbra{\prop_{#1}}{#2}}

% \newcommand{\slhotup}[1]{{#1}^{\leadsto}}
% \newcommand{\slhot}[1]{{#1} \leadsto \diamond}
% \newcommand{\degree}{l}
% \newcommand{\thunk}[1]{\{\!\{#1\}\!\}}
% \newcommand{\appthunk}[1]{\mathtt{run}\,{#1}}
%\newcommand{\appendx}[1]{}
% \newcommand{\appendx}[1]{#1}

% \newcommand{\mugamma}{\gamma}
% \newcommand{\misty}{\textsf{MISTY}\xspace}




% \newcommand{\fnb}[2]{\mathtt{fnb}(#1,#2)}
\newcommand{\Brec}[3]{\textcolor{\decoptcolor}{\mathbb{A}}^{#1}_{\textcolor{\decoptcolor}{\mathtt{rec}}~#2}\textcolor{\decoptcolor}{\big(}#3\textcolor{\decoptcolor}{\big)}}
\newcommand{\Rrec}[3]{\mathcal{R}^{#1}_{\mathtt{rec}#2}\big(#3\big)}
\newcommand{\Bsb}[3]{\mathcal{B}^{#1}_{\mathtt{sb} \ #2}\big(#3\big)}

\newcommand{\Bopt}[3]{\textcolor{\decoptcolor}{\mathbb{A}}^{#1}_{#2}\textcolor{\decoptcolor}{\big(}#3\textcolor{\decoptcolor}{\big)}}


\newcommand{\Brecd}[4]{\mathcal{B}^{#1}_{\mathtt{rec}#2}\big(#3\big)^{#4}}

\newcommand{\rvardepth}[1]{\ensuremath{\mathsf{recd}(#1)}}
\newcommand{\rvardepthaux}[1]{\ensuremath{\mathsf{recd}'(#1)}}

\newcommand{\Bbra}[3]{\mathcal{L}^{#1}_{#2}\big(#3\big)}
% \newcommand{\Bbrafst}[3]{\mathcal{L}^{#1}_{#2}\big(#3\big)}
\newcommand{\Bbrasnd}[1]{\mathcal{R}(#1)}

% \newcommand{\blue}[1]{\textcolor{blue}{#1}}

% \newcommand{\wtd}[1]{\widetilde{#1}}
\newcommand{\li}[1]{\widetilde{#1}}

\newcommand{\pfmap}{\Sigma}
\newcommand{\pfmapsmall}{\sigma}

% \newcommand{\lenHO}[1]{\lfloor #1 \rceil}
\newcommand{\lenHO}[1]{\textcolor{\deccolor}{\lfloor} #1 \textcolor{\deccolor}{\rceil}}
\newcommand{\lenHOopt}[1]{\textcolor{\decoptcolor}{\lfloor} #1 \textcolor{\decoptcolor}{\rceil^*}}

%\usepackage{accents}
\newcommand{\dbtilde}[1]{\widehat{#1}}
%\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}
%\newcommand{\dbtilde}[1]{\tilde{\raisebox{0pt}[0.85\height]{$\tilde{#1}$}}}

\newcommand{\indexed}[3]{\mathtt{indexed}_{#3}(#1,#2)}



% NEW COMMANDS FOR BISIMULATION 
% \newcommand{\Cb}[3]{\mathcal{C}^{#1}_{#2}\big(#3\big)}
% \newcommand{\Cbs}[3]{\widehat{\mathcal{C}}^{#1}_{#2}\big(#3\big)}
% \newcommand{\Cbrec}[3]{\mathcal{C}^{#1}_{\mathsf{rec} \ #2}\big(#3\big)}
% \newcommand{\Cbs}[3]{\mathsf{C}^{#1}_{#2}\big(#3\big)}
\newcommand{\Cbsb}[3]{\mathcal{C}^{#1}_{\mathtt{sb} \ #2}\big(#3\big)}
% \newcommand{\Dlet}{\mathcal{J}}
% \newcommand{\Db}[3]{\Dlet^{#1}_{#2}\big(#3\big)}
% \newcommand{\Dbrec}[3]{\Dlet^{#1}_{\mathsf{rec} \ #2}\big(#3\big)}
% \newcommand{\Dset}{\Dlet}

\newcommand{\Dbsb}[3]{\Dlet^{#1}_{\mathtt{sb} \ #2}\big(#3\big)}

% \newcommand{\fpn}[1]{\ensuremath{\mathsf{fpn}(#1)}}
% \newcommand{\nextn}[1]{\ensuremath{\mathsf{next}(#1)}}

% \newcommand{\indices}[1]{\ensuremath{\mathsf{index}(#1)}}
\newcommand{\bname}[1]{\ensuremath{\mathsf{bn}(#1)}}

\newcommand{\mstindex}{\ensuremath{l}}

% \usepackage{accents}

% \newcommand{\ddbtilde}[1]{\accentset{\approx}{#1}}
% \newcommand{\vardbtilde}[1]{\wtd{\raisebox{0pt}[0.85\height]{$\wtd{#1}$}}}

% \newcommand{\bns}[1]{\ensuremath{\mathtt{m}(#1)}}
% \newcommand{\wbns}[1]{\ensuremath{\vardbtilde {#1}}}

% \newcommand{\bns}[1]{\ensuremath{\ddbtilde {#1}}}
% \newcommand{\wbns}[1]{\ensuremath{\vardbtilde {#1}}}

% \newcommand{\bns}[1]{\ensuremath{\ddbtilde {#1}}}
% \newcommand{\wbns}[1]{\ensuremath{\vardbtilde {#1}}}

% \newcommand{\bns}[1]{\ensuremath{\tilde {#1}_{m}}}
% \newcommand{\wbns}[1]{\ensuremath{\wtd {#1}_{m}}}


% \newcommand{\bns}[1]{\ensuremath{\tilde {#1#1}}}
% \newcommand{\wbns}[1]{\ensuremath{\Hat {#1}}}

\newcommand{\bns}[1]{\ensuremath{\tilde {#1_*}}}
\newcommand{\wbns}[1]{\ensuremath{\widetilde {#1_*}}}

% \newcommand{\bns}[1]{\ensuremath{\tilde {#1_#1}}}
% \newcommand{\wbns}[1]{\ensuremath{\widetilde {#1_#1}}}

% \newcommand{\iname}[1]{\ensuremath{\breve{#1}}}

% \newcommand{\vrelate}{\bowtie}
% \newcommand{\valuesrelate}{\bowtie_{\mathtt{c}}}

% \newcommand{\highlighta}[1]{\colorbox{lightgray}{\ensuremath{#1}}}


% \newcommand{\rfni}[#1]{\mathtt{rfni}(P)}

% \newcommand{\valuesrelatev}{\bowtie_{\mathcal{C}}}


% NEW COMMANDS 


% \newcommand{\horelm}[5]{#1 \proves #2 #3 #4 \proves #5}
% \newcommand{\mstb}{\approx^{\mathtt{M}}}

\newcommand{\numpropam}[1]{\textcolor{\deccolor}{\#(}#1\textcolor{\deccolor}{)}}
\newcommand{\numprop}[1]{\textcolor{\decoptcolor}{\#^*(}#1\textcolor{\decoptcolor}{)}}


% \newcommand{\bbralts}[2]{#1 \& #2}
% \newcommand{\bsellts}[2]{#1 \oplus #2}
% \newcommand{\minnames}[2]{\langle #1 \rangle_{#2}}
% \newcommand{\mapcharm}[2]{\langle #1 \rangle^{#2}}
% \newcommand{\omapcharm}[1]{\langle #1 \rangle_{\texttt{c}}}

% \newcommand{\Rt}[1]{\textcolor{\decoptcolor}{\mathcal{R}(}#1\textcolor{\decoptcolor}{)}}
% \newcommand{\Rts}[3]{\textcolor{\decoptcolor}{\mathcal{R}^{\star}(}#3\textcolor{\decoptcolor}{)}}

\newcommand{\Rtopt}[1]{\textcolor{\decoptcolor}{\mathcal{R}(}#1\textcolor{\decoptcolor}{)}}
\newcommand{\Rtsopt}[3]{\textcolor{\decoptcolor}{\mathcal{R}^{\star}(}#3\textcolor{\decoptcolor}{)}}

% \newcommand{\mhby}[1]{\hby{#1}_{\texttt m}}
% \newcommand{\Mhby}[1]{\Hby{#1}_{\texttt m}}

% \newcommand{\tr}{\mathsf{tr}}

% \newcommand{\initname}[2]{\ensuremath{\subst{#1_{#2}}{#1}}}

% \newcommand{\rulename}[2]{\langle \texttt{#1}#2 \rangle}

% \newcommand{\Rb}[1]{\ensuremath{\mathcal{R}_{#1}}}

% \newcommand{\mstpred}[1]{\textsf{m}(#1)}
% \newcommand{\subl}[1]{\textsf{sub}(#1)}
% \newcommand{\condpv}[2]{\textsf{cond}(#1,#2)}

\newcommand{\ftriggerm}[3]{#1 \Leftarrow_{\mathtt{m}} #2{\,:\,}#3}
\newcommand{\fotriggerm}[6]{\binp{#1}{#2} \newsp{#3}{\binp{#3}{\wtd y}  \mapcharm{#4}{y}_{#6} \Par \bout{\dual{#3}}{#5} \inact}}


% \newcommand{\processrelate}{\diamond}

\newcommand{\rhom}{\ensuremath{\rho_{\mathtt m}}}

\newcommand{\sigmav}{\ensuremath{\sigma_v}}

\newcommand{\empg}{{}}

%\newcommand{\recpx}[1]{\ensuremath{\mathtt{\mathsf{X}}(#1)}}
\newcommand{\recpx}[1]{\ensuremath{\mathsf{frv}(#1)}}

\newcommand{\lenrecpx}[1]{\ensuremath{\#_X(#1)}}

\newcommand{\specx}{\ensuremath{\gamma}}

\newcommand{\recdep}{\ensuremath{d}}

%\newcommand{\lentr}[1]{\ensuremath{\len{#1}_{{tr}}}}
\newcommand{\lentr}[1]{\ensuremath{\mathsf{brn}(#1)}}



% \newcommand{\ppdp}{} 
\newcommand{\arxivlink}{https://arxiv.org/abs/2107.12345}

\newcommand{\longversion}[2]{\ifx\ppdp\undefined#1\else#2\fi}

\newcommand{\appnote}{\ifx\ppdp\undefined 
% ARXIV  
      \noindent \emph{Note:}   
      Due to space limits, 
      omitted  material (definitions, proofs, additional examples) can be found in the appendices. 
  \else 
    % PPDP 
    \noindent \emph{Note:}   
    Due to space limits, omitted material (definitions, proofs, additional examples) can 
    be found at \url{\arxivlink}. 
\fi 
}

\newcommand{\appnoteEx}
{\ifx\ppdp\undefined 
% ARXIV  
      \noindent The breakdown of $B'$ is similar and given in 
      \appref{ex:ex1-decomp}.
  \else 
    % PPDP 
    \noindent The breakdown of $B'$ is similar. 
\fi 
}

==> sources/ameliatable.tex <==
  \begin{table*}[!ht]
\begin{tabular}{ |l|l|l|}
  \rowcolor{gray!25}
  \hline
  $P$ &
    \multicolumn{2}{l|}{
  \begin{tabular}{l}
    \noalign{\smallskip}
    $\AmeliaMod{k}{\tilde x}{P}_g$
    \smallskip
  \end{tabular}
}  \\
  \hline
%%% OUTPUT
$\bout{u_i}{w_j} Q$ &
      \begin{tabular}{l}
      \noalign{\smallskip}
      $\propinp{k}{\widetilde x} \news{a} \big(\bout{u_i}{a}
       \big( \apropout{k+3}{\widetilde x} \Par
          \AmeliaMod{k+3}{\tilde x}{Q \sigma}_g \Par$
        \\
        $\qquad \qquad \qquad \binp{a}{y} \binp{y}{z_1} \apropout{k+1}{z_1} \Par
        \propinp{k+1}{z_1} \binp{z_1}{x} \apropout{k+2}{x} \Par$
        \\
        $\qquad \qquad \qquad \qquad \propinp{k+2}{x} 
        \news{s} \big(\bout{x}{s} \about{ \dual{s} }{\widetilde{w}} \big) \big) \big)$
     \smallskip
  \end{tabular}
  &
  %side-conditions
  \begin{tabular}{l}
    \noalign{\smallskip}
    $w_j:C $ \\
    
    $\widetilde w = (w_j,\ldots,w_{j+\len{\mGt{C}}-1})$ \\
    % $\widetilde z = \fv{Q}$ \\
		% $\sigma = \linecondit{u_i:S}{\incrname{u}{i}}{\{\} }$
    $\sigma = \nextn{u_i}$
%		\begin{cases}
%		\incrname{u}{i} & \text{if } u_i:S \\
%		\{\} & \text{otherwise}
%		\end{cases}
		% $
		%$\sigma$
		% $$\sigma = \begin{cases}
		% \incrname{u}{i} & if \\
		% \{\} &
		% \end{cases}$$
    \smallskip
  \end{tabular}
  \\
%  \hline
%	$\bout{u_i}{y}Q$
%	&
%	\begin{tabular}{l}
%	\noalign{\smallskip}
%	$\propinp{k}{\widetilde x} \bout{u_i}{y}
%	\propout{k+1}{\widetilde x'} \inact \Par \B{k+1}{\tilde x'}{Q\sigma}$ \\
%
%	\smallskip
%\end{tabular}
%	&
%	\begin{tabular}{l}
%		\noalign{\smallskip}
%		%$\widetilde x \eqprm \widetilde z y$ \\
%%		$\widetilde x' = \begin{cases}
%%		\widetilde z y, & \text{if} \ y \in \fv{Q}  \\
%%		\widetilde z, & \text{otherwise}
%%		\end{cases}$ \\
%	$\widetilde x' = \fv{Q}$ \\
%	%$y \in \widetilde x$ \\
%	$\sigma = \begin{cases}
%	\incrname{u}{i} & \text{if } u_i:S \\
%	\{\} & \text{otherwise}
%	\end{cases}$
%	\smallskip
%\end{tabular}
\hline 

%%% INPUT
$\binp{u_i}{w}Q$
&

  \begin{tabular}{l}
      \noalign{\smallskip}
            $\propinp{k}{\widetilde x}\binp{u_i}{y} \apropout{k+1}{\widetilde x, y} \Par$ 
            \\
            $\qquad \news{s_1} \big(\propinp{k+1}{\widetilde x, y} 
            \propout{k+2}{y} \apropout{k+3}{\widetilde x} \Par$ 
            \\
            $\qquad \qquad \qquad \propinp{k+2}{y} \news{s} \big(\bout{y}{s} \about{\dual{s}}{s_1}   ) \Par$ 
            \\
            $\qquad \qquad \qquad\propinp{k+3}{\widetilde x} 
            \news{a}  \big(\bout{\dual{s_1}}{a} \big( 
              \apropout{k+l+4}{} \Par \propinp{k+l+4}{} \inact \Par \widehat{Q}_{\tilde{x}}~  \big) \big) \big)$
            %%%%
            \smallskip 
            \\
      where:\\
      $ \!\begin{aligned} 
        \widehat{Q}_{\tilde{x}} &= \binp{a}{y'} \binp{y'}
        {\widetilde{w}} \big( \apropout{k+4}{\widetilde x} \Par
        \AmeliaMod{k+4}{\widetilde x}{Q \subst{w_1}{w} \sigma }_g \big) 
      \end{aligned}$ 
%      \smallskip
%        \\
  \smallskip
  \end{tabular}
  &
  %side-conditions
  \begin{tabular}{l}
    \noalign{\smallskip}
%    	$\widetilde x' = \begin{cases}
%		\widetilde x y & \text{if } y \in \fv{Q} \\
%		\widetilde x & \text{otherwise}
%		\end{cases}$ \\
%    $w:\slhotup{C}$\\
    $w : C$\\
    $\widetilde w = (w_1, \ldots, w_{\len{\mGt{C}}}) $\\
% 	$\widetilde z = \fv{Q} $ \\
	$l = \lenHO{Q}$ \smallskip \\
		%$\sigma = \begin{cases}
		%\incrname{u}{i} & \text{if } u_i:S \\
		%\{\} & \text{otherwise}
		%\end{cases}$
    
    % $\widetilde{\prop} = \begin{cases} 
    %         \epsilon & \text{if} \ \leadsto = \multimap \\
    %      (\prop_k,\ldots,\prop_{k+\lenHO{P}-1}) & \text{if} \ \leadsto = \rightarrow
    %  \end{cases}$ \smallskip \\
     
    %  $\sigma = \linecondit{u_i:S}{\incrname{u}{i}}{\epsilon}$
     $\sigma = \nextn{u_i}$
%     \begin{cases}
%		\incrname{u}{i} & \text{if } u_i:S \\
%	    \epsilon & \text{otherwise}
%		\end{cases}

\smallskip
  \end{tabular}
    \\
  \hline

    %$\appl{V}{u_i}$ &
  %\begin{tabular}{l}
    %\noalign{\smallskip}
    %$\propinp{k}{\widetilde x}\appl{\V{k+1}{\tilde x}{V}}{\widetilde m}$
    %\smallskip
  %\end{tabular}
  %&
  %%side-conditions
  %\begin{tabular}{l}
  %	\noalign{\smallskip}
  %	$u_i:C$ \\
  %	$\widetilde x = \fv{V}$ \\
  %  $\widetilde{m} = (u_i,\ldots,u_{i+\len{\Gt{C}}-1})$
  %  \smallskip
  %\end{tabular}
  %\\
  %\hline


%  $\appl{y}{u_i}$ &
%  \begin{tabular}{l}
%    \noalign{\smallskip}
%    $\propinp{k}{\widetilde x}\appl{y}{\widetilde m}$
%    \smallskip
%  \end{tabular}
%  &
%  %side-conditions \\
%  \begin{tabular}{l}
%    \noalign{\smallskip}
%    $u_i:C$ \\
%    %$\widetilde x = y$ \\
%    $\widetilde m = (u_i,\ldots,u_{i+\len{\Gt{C}}-1})$
%    \smallskip
%  \end{tabular}
%\\

  
%%% INPUT WITH RECURSIVE NAME 
$\bout{r_i}{w_j} P$ &
\begin{tabular}{l}
  \noalign{\smallskip}
  $\propinp{k}{\widetilde x}
  \news{a_1}{}\proprout{r}{a_1}\big(\AmeliaMod{k+3}{\tilde x}{P}_g
  \Par \binp{a_1}{y_1}\binp{y_1}{\widetilde z}W \big)$ \\
  \text{where:} \\
  $W =  \news{a_2}\big(\bout{z_{f(S)}}{a_2} \big(\propout{k+3}{\widetilde x}\proprinp{r}{b}
        \news{s} \big(\bout{b}{s}\about{\dual{s}}{\widetilde z} \big) \Par$
         \\
        $ \qquad \qquad  \binp{a_2}{y_2}\binp{y_2}{z'_1}
        % \news{\widetilde \prop}
        \big(\apropout{k+1}{} \Par $ 
        \\ 
        $\qquad \qquad \propinp{k+1}{}\binp{z'_1}{x}\apropout{k+2}{x} 
        \Par \propinp{k+2}{x}\news{s'} \big(\bout{x}{s'}\about{\dual s'}{\widetilde w} \big) \big) \big) \big)$
 \smallskip
\end{tabular}
&
\begin{tabular}{l}
	\noalign{\smallskip}
   $r:S \wedge \mathsf{tr}(S)$ \\
   $\wtd z = (z_1,\ldots,z_{\len{\mRts{}{s}{S}}})$\\
   $\widetilde{c} = (c_{k+1}, c_{k+2})$ \\
  %  $\widetilde{y} = \fn{P}$ \\
   $w:C \wedge \wtd{w} = (w_j, \ldots, w_{j+ \len{\mGt{C}} - 1})$
\smallskip
\end{tabular}
  \\
  \hline
  $\binp{r_i}{w} P$ &
\begin{tabular}{l}
  \noalign{\smallskip}
    $\propinp{k}{\widetilde x}\news{a_1}\big(\proprout{r}{a_1}
    \big(\news{s_1}\big(\propinp{k+1}{y}\propout{k+2}{y}\apropout{k+3}{}
    \Par$
    \\
    $\qquad \propinp{k+2}{y}\news{s}\big(\bout{y}{s}\about{\dual s}{s_1}) \Par $
    \\
    $\qquad \propinp{k+3}{}\news{a_2} \big(\bout{s_1}{a_2}\big(
    \apropout{k+l+4}{} \Par \propinp{k+l+4}{}\inact \Par$
    \\
    $\qquad \qquad \qquad \qquad  \binp{a_2}{y_2}\binp{y_2}{\widetilde w}
    % \news{\widetilde \prop}
    \big(\apropout{k+4}{\widetilde x}
    \Par \AmeliaMod{k+4}{\tilde x}{P\subst{w_1}{w}}_g
    \big)\big)\big)  \Par$
    \\
   $
    \qquad \qquad \qquad \qquad \binp{a_1}{y_1}\binp{y_1}{\widetilde z}\binp{z_{f(S)}}{y}$
    \\
    $\qquad \qquad \qquad \qquad \qquad 
    \propout{k+1}{y}\proprinp{r}{b}
    \news{s'}\big(\bout{b}{s'}
    \about{\dual s'}{\widetilde z}\big)
    \big)\big) \big)$
 \smallskip
\end{tabular}
&
\begin{tabular}{l}
	\noalign{\smallskip}
   $r:S \wedge \mathsf{tr}(S)$ \\
   $\wtd z = (z_1,\ldots,z_{\len{\mRts{}{s}{S}}})$\\
  %  $\widetilde{x}' = \fn{P}$\\
   $l = \lenHO{P}$ \\
  %  $l = \begin{cases} 
  %           \lenHO{P} & \text{if} \ \leadsto = \multimap \\
  %        0 & \text{if} \ \leadsto = \rightarrow
  %    \end{cases}$\\
   $w:C \wedge \wtd{w} = (w_1, \ldots, w_{\len{\mGt{C}}})$
  %  $\wtd{\prop} =  (\prop_{k+4},\ldots,\prop_{k+\lenHO{P}+3})$ \\
  %  $\widetilde{\prop} = \begin{cases} 
  %           \epsilon & \text{if} \ \leadsto = \multimap \\
  %        (\prop_{k+4},\ldots,\prop_{k+\lenHO{P}+3}) & \text{if} \ \leadsto = \rightarrow
  %    \end{cases}$
\smallskip
\end{tabular}
  \\
  \hline
  %%% RESTRICTION
  $\news{s:C}{P'}$ &
  \begin{tabular}{l}
    \noalign{\smallskip}
 	$\news{\widetilde{s}:\mGt{C}}{\,\AmeliaMod{k}{\tilde x}
 			{P'\sigma}_g}$
    \smallskip
  \end{tabular}
  &
  %side-conditions
  \begin{tabular}{ll}
    \noalign{\smallskip}
    % $\widetilde x = \fv{P'}$ \\
    $\widetilde{s} = (s_1,\ldots,s_{\len{\mGt{C}}})$ &
    $\sigma = 	\subst{s_1 \dual{s_1}}{s \dual{s}}$
% 	$\sigma = \begin{cases}
% 				\subst{s_1 \dual{s_1}}{s \dual{s}} & \text{if} \ C = S \\
% 				\subst{s_1}{s} & \text{if} \ C = \chtype{U}
%             \end{cases}
% $
    \smallskip
  \end{tabular}
  \\
  \hline
   %%% RESTRICTION TAIL RECURSIVE 
   $\news{r:\trec{t}{S}}{P'}$ &
   \begin{tabular}{l}
     \noalign{\smallskip}
    $\news{\widetilde{r}:\mRt{S}}{\,
    \proprinp{r}{b}\news{s'}\big(\bout{b}{s'}\about{\dual s'}
        {\widetilde r}\big) \Par 
        \proprinp{\dual r}{b}\news{s'}\big(\bout{b}{s'}\about{\dual s'}
        {\widetilde {\dual r}}\big)
   \Par \AmeliaMod{k}{\tilde x}  
        {P'\sigma}_g}$
     \smallskip
   \end{tabular}
   &
   %side-conditions
   \begin{tabular}{ll}
     \noalign{\smallskip}
     % $\widetilde x = \fv{P'}$ \\
     $\tr(\trec{t}{S})$  & $\sigma = 	\subst{r_1 \dual{r_1}}{r \dual{r}}$ 
    \\
     $\widetilde{r} = (r_1,\ldots,r_{\len{\mRt{S}}})$ \\
     $\widetilde{\dual r} = (\dual r_1,\ldots,\dual r_{\len{\mRt{S}}})$
    %  $\sigma = 	\subst{s_1 \dual{s_1}}{s \dual{s}}$
 % 	$\sigma = \begin{cases}
 % 				\subst{s_1 \dual{s_1}}{s \dual{s}} & \text{if} \ C = S \\
 % 				\subst{s_1}{s} & \text{if} \ C = \chtype{U}
 %             \end{cases}
 % $
     \smallskip
   \end{tabular}
   \\
   \hline
%%% PARALLEL
  $Q_1 \Par Q_2$ &
  \begin{tabular}{l}
    \noalign{\smallskip}
    $\propinp{k}{\tilde x} \propout{k+1}{\tilde y}
    \apropout{k+\degree+1}{\tilde z}   \Par \AmeliaMod{k+1}{\tilde y}{Q_1}_g \Par \AmeliaMod{k+\degree+1}{\tilde z}{Q_2}_g$
    \smallskip
  \end{tabular}
  &
  %side-conditions
  \begin{tabular}{lll}
    \noalign{\smallskip}
    $\widetilde y  = \fv{Q_1}$ &
    $\widetilde z = \fv{Q_2}$ &
    $\degree = \lenHO{Q}$
    \smallskip
  \end{tabular}
      \\
  \hline

%%% INACTION
  $\inact$ &
\begin{tabular}{l}
  \noalign{\smallskip}
  $\propinp{k}{}\inact$
 \smallskip
\end{tabular}
&
\begin{tabular}{l}
	\noalign{\smallskip}
\smallskip
\end{tabular}
  \\
  % \hline
  \hline 
  %%%% RECURSIVE PROCESS
  $\recp{X}{P}$ &
\begin{tabular}{l}
  \noalign{\smallskip}
      $\news{s_1} \big(  \propinp{k}{\widetilde x}\propout{k+1}{\wtd x}
      \apropout{k+3}{\wtd x} \Par$ 
      \\
      $\qquad \quad \propinp{k+1}{\wtd x} \news{a_1}\big( \bout{s_1}{a_1} \big( \apropout{k+2}{}
      \Par \propinp{k+2}{}\inact \Par$
      \\
      $\qquad \qquad \qquad \qquad \qquad \propinp{k+3}{\widetilde x}\binp{s_1}{z_x}
      \apropout{k+4}{\wtd x, z_x} 
      \Par$
      \\
      $
      \qquad \qquad \qquad \qquad \qquad 
      \AmeliaMod{k+4}{\tilde x, z_x}{P}_{g, \{X \rightarrow {\tilde n}\}} \Par $\\
      $\qquad \qquad \qquad \qquad \qquad
      \repl\binp{a_1}{y'_1}
      \binp{y'_1}{\vmap{\widetilde n^1}, \ldots, \vmap{\widetilde n^m}, y_1}\widehat{P}\,\big)\big)\big)$ 
      \\
      \text{where:} 
      \\
     $\widehat{P} = \news{\widetilde \prop}\big( \prod_{0 < i \leq m}
        \proprinp{n_i}{b}\news{s'}\big(\bout{b}{s'}\about{\dual s'}
        {\vmap{\widetilde n^i}}\big)
        \Par \apropout{k+2}{\widetilde x}$ 
        \\
        $\quad \quad \quad \qquad \qquad \qquad  
        \propinp{k+2}{\widetilde x}\binp{y_1}{z_x}\apropout{k+3}{\widetilde x, z_x} 
        \Par   \auxmapp{ \AmeliaMod{k+3}{\tilde{x}, z_x}
        {P}_{g, \{X \rightarrow {\tilde n}\}}  }{{}}{{\tilde \prop, \tilde \prop_r}}\big)$
 \smallskip
\end{tabular}
&
\begin{tabular}{l}
	\noalign{\smallskip}
    $\wtd n = \fn{P}$ \\
    $m = \len{\wtd n}$ \\
    $\vmap{\widetilde n} = (\vmap{n_1}, \dots, \vmap{n_m})$ \\
    $i \in \{1,\ldots,m \}.$ \\
    $\qquad \vmap{n_i} : S_i$ \\
    $\qquad \vmap{\widetilde n^i} = (\vmap{n_1^i}, \dots, \vmap{n_{\len{\mGt{S_i}}}^i })$\\
    $\widetilde{\prop} =(\prop_{k+2},\ldots,
    \prop_{k+\lenHO{ \vmap{P}^1_{g, \{X \rightarrow \tilde n \}}{{}} }+1})$ \\
    $\wtd c_r = \bigcup_{v \in \wtd n} c^v$
\smallskip
\end{tabular}
\\
  \hline
  %%%% RECURSIVE VARIABLE
  $\rvar{X}$ &
\begin{tabular}{l}
  \noalign{\smallskip}
    $\news{s_1}\big( \propinp{k}{z_x}\propout{k+1}{z_x}\apropout{k+2}{z_x} 
    \Par $
    $\propinp{k+2}{z_x}\bout{\dual s_1}{z_x}\apropout{k+3}{} 
    \Par \propinp{k+3}{}\inact$ 
     \\ 
     $\qquad \qquad \propinp{k+1}{z_x}\news{a_1}
     \big( \proprout{n_1}{a_1}\big($
    %  \\
    $
    \binp{a_1}{y_1}\binp{y_1}{\widetilde z_1} \ldots \news{a_j}Q\big)\big)
    % \Par \propinp{k+2}{z_x}\bout{\dual s_1}{z_x}\apropout{k+3}{} 
    % \Par \propinp{k+3}{}\inact 
    \big)$ 
    \\ 
    \text{where:} 
    \\
    $Q = \big(\proprout{n_j}{a_j}\big(\binp{a_j}{y_j}\binp{y_j}{\widetilde z_j}
    \news{s'}\big(\bout{z_x}{s'}\about{\dual s'}{\widetilde z_1, \ldots, \widetilde z_j, s_1}\big)\big)\big)$
 \smallskip
\end{tabular}
&
\begin{tabular}{l}
	\noalign{\smallskip}
      $\wtd n = g(X)$ \\
      $\len{\widetilde n} = j$ \\
      $i \in \{1, \dots, j\}$ \\
      $\quad n_i : S \wedge \mathsf{tr}(S_i)$ \\
      $\quad \widetilde{z_i} = (z_1^i, \dots, z_{\len{\mRts{}{}{S_i}}}^i)$
\smallskip
\end{tabular}
% \\
%   \hline
%   $\inact$ &
% \begin{tabular}{l}
%   \noalign{\smallskip}
%   $\propinp{k}{}\inact$
%  \smallskip
% \end{tabular}
% &
% \begin{tabular}{l}
% 	\noalign{\smallskip}
% \smallskip
% \end{tabular}
  \\
  \hline
\end{tabular}
\caption{Decompose by composition: Breakdown function $\AmeliaMod{k}{\tilde x}{\cdot}_g$ for \sessp processes 
(cf. Definition~\ref{def:am-decomp}). \label{table:repo}}
\vspace{-4mm}
\end{table*}

==> sources/ameliatable1-backup.tex <==
  % \begin{table*}[!ht]
\begin{tabular}{ |l|l|l|}
  \rowcolor{gray!25}
  \hline
  $P$ &
    \multicolumn{2}{l|}{
  \begin{tabular}{l}
    \noalign{\smallskip}
    $\AmeliaMod{k}{\tilde x}{P}_g$
    \smallskip
  \end{tabular}
}  \\
  \hline
%%% OUTPUT
$\bout{u_i}{w_j} Q$ &
      \begin{tabular}{l}
      \noalign{\smallskip}
      $\propinp{k}{\widetilde x} \news{a} \big(\bout{u_i}{a}
       \big( \apropout{k+3}{\widetilde x} \Par
          \AmeliaMod{k+3}{\tilde x}{Q \sigma}_g \Par$
        \\
        $\qquad \qquad \qquad \binp{a}{y} \binp{y}{z_1} \apropout{k+1}{z_1} \Par
        \propinp{k+1}{z_1} \binp{z_1}{x} \apropout{k+2}{x} \Par$
        \\
        $\qquad \qquad \qquad \qquad \propinp{k+2}{x} 
        \news{s} \big(\bout{x}{s} \about{ \dual{s} }{\widetilde{w}} \big) \big) \big)$
     \smallskip
  \end{tabular}
  &
  %side-conditions
  \begin{tabular}{l}
    \noalign{\smallskip}
    $w_j:C $ \\
    
    $\widetilde w = (w_j,\ldots,w_{j+\len{\mGt{C}}-1})$ \\
    % $\widetilde z = \fv{Q}$ \\
		% $\sigma = \linecondit{u_i:S}{\incrname{u}{i}}{\{\} }$
    $\sigma = \nextn{u_i}$
%		\begin{cases}
%		\incrname{u}{i} & \text{if } u_i:S \\
%		\{\} & \text{otherwise}
%		\end{cases}
		% $
		%$\sigma$
		% $$\sigma = \begin{cases}
		% \incrname{u}{i} & if \\
		% \{\} &
		% \end{cases}$$
    \smallskip
  \end{tabular}
  \\
%  \hline
%	$\bout{u_i}{y}Q$
%	&
%	\begin{tabular}{l}
%	\noalign{\smallskip}
%	$\propinp{k}{\widetilde x} \bout{u_i}{y}
%	\propout{k+1}{\widetilde x'} \inact \Par \B{k+1}{\tilde x'}{Q\sigma}$ \\
%
%	\smallskip
%\end{tabular}
%	&
%	\begin{tabular}{l}
%		\noalign{\smallskip}
%		%$\widetilde x \eqprm \widetilde z y$ \\
%%		$\widetilde x' = \begin{cases}
%%		\widetilde z y, & \text{if} \ y \in \fv{Q}  \\
%%		\widetilde z, & \text{otherwise}
%%		\end{cases}$ \\
%	$\widetilde x' = \fv{Q}$ \\
%	%$y \in \widetilde x$ \\
%	$\sigma = \begin{cases}
%	\incrname{u}{i} & \text{if } u_i:S \\
%	\{\} & \text{otherwise}
%	\end{cases}$
%	\smallskip
%\end{tabular}
\hline 

%%% INPUT
$\binp{u_i}{w}Q$
&

  \begin{tabular}{l}
      \noalign{\smallskip}
            $\propinp{k}{\widetilde x}\binp{u_i}{y} \apropout{k+1}{\widetilde x, y} \Par$ 
            \\
            $\qquad \news{s_1} \big(\propinp{k+1}{\widetilde x, y} 
            \propout{k+2}{y} \apropout{k+3}{\widetilde x} \Par$ 
            \\
            $\qquad \qquad \qquad \propinp{k+2}{y} \news{s} \big(\bout{y}{s} \about{\dual{s}}{s_1}   ) \Par$ 
            \\
            $\qquad \qquad \qquad\propinp{k+3}{\widetilde x} 
            \news{a}  \big(\bout{\dual{s_1}}{a} \big( 
              \apropout{k+l+4}{} \Par \propinp{k+l+4}{} \inact \Par \widehat{Q}_{\tilde{x}}~  \big) \big) \big)$
            %%%%
            \smallskip 
            \\
      where:\\
      $ \!\begin{aligned} 
        \widehat{Q}_{\tilde{x}} &= \binp{a}{y'} \binp{y'}
        {\widetilde{w}} \big( \apropout{k+4}{\widetilde x} \Par
        \AmeliaMod{k+4}{\widetilde x}{Q \subst{w_1}{w} \sigma }_g \big) 
      \end{aligned}$ 
%      \smallskip
%        \\
  \smallskip
  \end{tabular}
  &
  %side-conditions
  \begin{tabular}{l}
    \noalign{\smallskip}
%    	$\widetilde x' = \begin{cases}
%		\widetilde x y & \text{if } y \in \fv{Q} \\
%		\widetilde x & \text{otherwise}
%		\end{cases}$ \\
%    $w:\slhotup{C}$\\
    $w : C$\\
    $\widetilde w = (w_1, \ldots, w_{\len{\mGt{C}}}) $\\
% 	$\widetilde z = \fv{Q} $ \\
	$l = \lenHO{Q}$ \smallskip \\
		%$\sigma = \begin{cases}
		%\incrname{u}{i} & \text{if } u_i:S \\
		%\{\} & \text{otherwise}
		%\end{cases}$
    
    % $\widetilde{\prop} = \begin{cases} 
    %         \epsilon & \text{if} \ \leadsto = \multimap \\
    %      (\prop_k,\ldots,\prop_{k+\lenHO{P}-1}) & \text{if} \ \leadsto = \rightarrow
    %  \end{cases}$ \smallskip \\
     
    %  $\sigma = \linecondit{u_i:S}{\incrname{u}{i}}{\epsilon}$
     $\sigma = \nextn{u_i}$
%     \begin{cases}
%		\incrname{u}{i} & \text{if } u_i:S \\
%	    \epsilon & \text{otherwise}
%		\end{cases}

\smallskip
  \end{tabular}
    \\
  \hline

    %$\appl{V}{u_i}$ &
  %\begin{tabular}{l}
    %\noalign{\smallskip}
    %$\propinp{k}{\widetilde x}\appl{\V{k+1}{\tilde x}{V}}{\widetilde m}$
    %\smallskip
  %\end{tabular}
  %&
  %%side-conditions
  %\begin{tabular}{l}
  %	\noalign{\smallskip}
  %	$u_i:C$ \\
  %	$\widetilde x = \fv{V}$ \\
  %  $\widetilde{m} = (u_i,\ldots,u_{i+\len{\Gt{C}}-1})$
  %  \smallskip
  %\end{tabular}
  %\\
  %\hline


%  $\appl{y}{u_i}$ &
%  \begin{tabular}{l}
%    \noalign{\smallskip}
%    $\propinp{k}{\widetilde x}\appl{y}{\widetilde m}$
%    \smallskip
%  \end{tabular}
%  &
%  %side-conditions \\
%  \begin{tabular}{l}
%    \noalign{\smallskip}
%    $u_i:C$ \\
%    %$\widetilde x = y$ \\
%    $\widetilde m = (u_i,\ldots,u_{i+\len{\Gt{C}}-1})$
%    \smallskip
%  \end{tabular}
%\\

  
%%% INPUT WITH RECURSIVE NAME 
$\bout{r_i}{w_j} P$ &
\begin{tabular}{l}
  \noalign{\smallskip}
  $\propinp{k}{\widetilde x}
  \news{a_1}{}\proprout{r}{a_1}\big(\AmeliaMod{k+3}{\tilde x}{P}_g
  \Par \binp{a_1}{y_1}\binp{y_1}{\widetilde z}W \big)$ \\
  \text{where:} \\
  $W =  \news{a_2}\big(\bout{z_{f(S)}}{a_2} \big(\propout{k+3}{\widetilde x}\proprinp{r}{b}
        \news{s} \big(\bout{b}{s}\about{\dual{s}}{\widetilde z} \big) \Par$
         \\
        $ \qquad \qquad  \binp{a_2}{y_2}\binp{y_2}{z'_1}
        % \news{\widetilde \prop}
        \big(\apropout{k+1}{} \Par $ 
        \\ 
        $\qquad \qquad \propinp{k+1}{}\binp{z'_1}{x}\apropout{k+2}{x} 
        \Par \propinp{k+2}{x}\news{s'} \big(\bout{x}{s'}\about{\dual s'}{\widetilde w} \big) \big) \big) \big)$
 \smallskip
\end{tabular}
&
\begin{tabular}{l}
	\noalign{\smallskip}
   $r:S \wedge \mathsf{tr}(S)$ \\
   $\wtd z = (z_1,\ldots,z_{\len{\mRts{}{s}{S}}})$\\
   $\widetilde{c} = (c_{k+1}, c_{k+2})$ \\
  %  $\widetilde{y} = \fn{P}$ \\
   $w:C \wedge \wtd{w} = (w_j, \ldots, w_{j+ \len{\mGt{C}} - 1})$
\smallskip
\end{tabular}
  \\
  \hline
  $\binp{r_i}{w} P$ &
\begin{tabular}{l}
  \noalign{\smallskip}
    $\propinp{k}{\widetilde x}\news{a_1}\big(\proprout{r}{a_1}
    \big(\news{s_1}\big(\propinp{k+1}{y}\propout{k+2}{y}\apropout{k+3}{}
    \Par$
    \\
    $\qquad \propinp{k+2}{y}\news{s}\big(\bout{y}{s}\about{\dual s}{s_1}) \Par $
    \\
    $\qquad \propinp{k+3}{}\news{a_2} \big(\bout{s_1}{a_2}\big(
    \apropout{k+l+4}{} \Par \propinp{k+l+4}{}\inact \Par$
    \\
    $\qquad \qquad \qquad \qquad  \binp{a_2}{y_2}\binp{y_2}{\widetilde w}
    % \news{\widetilde \prop}
    \big(\apropout{k+4}{\widetilde x}
    \Par \AmeliaMod{k+4}{\tilde x}{P\subst{w_1}{w}}_g
    \big)\big)\big)  \Par$
    \\
   $
    \qquad \qquad \qquad \qquad \binp{a_1}{y_1}\binp{y_1}{\widetilde z}\binp{z_{f(S)}}{y}$
    \\
    $\qquad \qquad \qquad \qquad \qquad 
    \propout{k+1}{y}\proprinp{r}{b}
    \news{s'}\big(\bout{b}{s'}
    \about{\dual s'}{\widetilde z}\big)
    \big)\big) \big)$
 \smallskip
\end{tabular}
&
\begin{tabular}{l}
	\noalign{\smallskip}
   $r:S \wedge \mathsf{tr}(S)$ \\
   $\wtd z = (z_1,\ldots,z_{\len{\mRts{}{s}{S}}})$\\
  %  $\widetilde{x}' = \fn{P}$\\
   $l = \lenHO{P}$ \\
  %  $l = \begin{cases} 
  %           \lenHO{P} & \text{if} \ \leadsto = \multimap \\
  %        0 & \text{if} \ \leadsto = \rightarrow
  %    \end{cases}$\\
   $w:C \wedge \wtd{w} = (w_1, \ldots, w_{\len{\mGt{C}}})$
  %  $\wtd{\prop} =  (\prop_{k+4},\ldots,\prop_{k+\lenHO{P}+3})$ \\
  %  $\widetilde{\prop} = \begin{cases} 
  %           \epsilon & \text{if} \ \leadsto = \multimap \\
  %        (\prop_{k+4},\ldots,\prop_{k+\lenHO{P}+3}) & \text{if} \ \leadsto = \rightarrow
  %    \end{cases}$
\smallskip
\end{tabular}
  \\
  \hline
\end{tabular} 
  %%% RESTRICTION
%   \begin{tabular} 
%   $\news{s:C}{P'}$ &
%   \begin{tabular}{l}
%     \noalign{\smallskip}
%  	$\news{\widetilde{s}:\mGt{C}}{\,\AmeliaMod{k}{\tilde x}
%  			{P'\sigma}_g}$
%     \smallskip
%   \end{tabular}
%   &
%   %side-conditions
%   \begin{tabular}{ll}
%     \noalign{\smallskip}
%     % $\widetilde x = \fv{P'}$ \\
%     $\widetilde{s} = (s_1,\ldots,s_{\len{\mGt{C}}})$ &
%     $\sigma = 	\subst{s_1 \dual{s_1}}{s \dual{s}}$
% % 	$\sigma = \begin{cases}
% % 				\subst{s_1 \dual{s_1}}{s \dual{s}} & \text{if} \ C = S \\
% % 				\subst{s_1}{s} & \text{if} \ C = \chtype{U}
% %             \end{cases}
% % $
%     \smallskip
%   \end{tabular}
%   \\
%   \hline
%    %%% RESTRICTION TAIL RECURSIVE 
%    $\news{r}{P'}$ &
%    \begin{tabular}{l}
%      \noalign{\smallskip}
%     $\news{\widetilde{r}:\mRt{S}}{\,
%     \proprinp{r}{b}\news{s'}\big(\bout{b}{s'}\about{\dual s'}
%         {\widetilde r}\big) \Par 
%         \proprinp{\dual r}{b}\news{s'}\big(\bout{b}{s'}\about{\dual s'}
%         {\widetilde {\dual r}}\big)
%    \Par \AmeliaMod{k}{\tilde x}  
%         {P'\sigma}_g}$
%      \smallskip
%    \end{tabular}
%    &
%    %side-conditions
%    \begin{tabular}{ll}
%      \noalign{\smallskip}
%      % $\widetilde x = \fv{P'}$ \\
%      $\trec{t}{S}$
%      \\ 
%      $\tr(\trec{t}{S})$  & $\sigma = 	\subst{r_1 \dual{r_1}}{r \dual{r}}$ 
%     \\
%      $\widetilde{r} = (r_1,\ldots,r_{\len{\mRt{S}}})$ \\
%      $\widetilde{\dual r} = (\dual r_1,\ldots,\dual r_{\len{\mRt{S}}})$
%     %  $\sigma = 	\subst{s_1 \dual{s_1}}{s \dual{s}}$
%  % 	$\sigma = \begin{cases}
%  % 				\subst{s_1 \dual{s_1}}{s \dual{s}} & \text{if} \ C = S \\
%  % 				\subst{s_1}{s} & \text{if} \ C = \chtype{U}
%  %             \end{cases}
%  % $
%      \smallskip
%    \end{tabular}
%    \\
%    \hline
% %%% PARALLEL
%   $Q_1 \Par Q_2$ &
%   \begin{tabular}{l}
%     \noalign{\smallskip}
%     $\propinp{k}{\tilde x} \propout{k+1}{\tilde y}
%     \apropout{k+\degree+1}{\tilde z}   \Par \AmeliaMod{k+1}{\tilde y}{Q_1}_g \Par \AmeliaMod{k+\degree+1}{\tilde z}{Q_2}_g$
%     \smallskip
%   \end{tabular}
%   &
%   %side-conditions
%   \begin{tabular}{lll}
%     \noalign{\smallskip}
%     $\widetilde y  = \fv{Q_1}$ &
%     $\widetilde z = \fv{Q_2}$ &
%     $\degree = \lenHO{Q}$
%     \smallskip
%   \end{tabular}
%       \\
%   \hline

% %%% INACTION
%   $\inact$ &
% \begin{tabular}{l}
%   \noalign{\smallskip}
%   $\propinp{k}{}\inact$
%  \smallskip
% \end{tabular}
% &
% \begin{tabular}{l}
% 	\noalign{\smallskip}
% \smallskip
% \end{tabular}
%   \\
%   % \hline
%   \hline 
%   %%%% RECURSIVE PROCESS
%   $\recp{X}{P}$ &
% \begin{tabular}{l}
%   \noalign{\smallskip}
%       $\news{s_1} \big(  \propinp{k}{\widetilde x}\propout{k+1}{\wtd x}
%       \apropout{k+3}{\wtd x} \Par$ 
%       \\
%       $\qquad \quad \propinp{k+1}{\wtd x} \news{a_1}\big( \bout{s_1}{a_1} \big( \apropout{k+2}{}
%       \Par \propinp{k+2}{}\inact \Par$
%       \\
%       $\qquad \qquad \qquad \qquad \qquad \propinp{k+3}{\widetilde x}\binp{s_1}{z_x}
%       \apropout{k+4}{\wtd x, z_x} 
%       \Par$
%       \\
%       $
%       \qquad \qquad \qquad \qquad \qquad 
%       \AmeliaMod{k+4}{\tilde x, z_x}{P}_{g, \{X \rightarrow {\tilde n}\}} \Par $\\
%       $\qquad \qquad \qquad \qquad \qquad
%       \repl\binp{a_1}{y'_1}
%       \binp{y'_1}{\vmap{\widetilde n^1}, \ldots, \vmap{\widetilde n^m}, y_1}\widehat{P}\,\big)\big)\big)$ 
%       \\
%       \text{where:} 
%       \\
%      $\widehat{P} = \news{\widetilde \prop}\big( \prod_{0 < i \leq m}
%         \proprinp{n_i}{b}\news{s'}\big(\bout{b}{s'}\about{\dual s'}
%         {\vmap{\widetilde n^i}}\big)
%         \Par \apropout{k+2}{\widetilde x}$ 
%         \\
%         $\quad \quad \quad \qquad \qquad \qquad  
%         \propinp{k+2}{\widetilde x}\binp{y_1}{z_x}\apropout{k+3}{\widetilde x, z_x} 
%         \Par   \auxmapp{ \AmeliaMod{k+3}{\tilde{x}, z_x}
%         {P}_{g, \{X \rightarrow {\tilde n}\}}  }{{}}{{\tilde \prop, \tilde \prop_r}}\big)$
%  \smallskip
% \end{tabular}
% &
% \begin{tabular}{l}
% 	\noalign{\smallskip}
%     $\wtd n = \fn{P}$ \\
%     $m = \len{\wtd n}$ \\
%     $\vmap{\widetilde n} = (\vmap{n_1}, \dots, \vmap{n_m})$ \\
%     $i \in \{1,\ldots,m \}.$ \\
%     $\qquad \vmap{n_i} : S_i$ \\
%     $\qquad \vmap{\widetilde n^i} = (\vmap{n_1^i}, \dots, \vmap{n_{\len{\mGt{S_i}}}^i })$\\
%     $\widetilde{\prop} =(\prop_{k+2},\ldots,
%     \prop_{k+\lenHO{ \vmap{P}^1_{g, \{X \rightarrow \tilde n \}}{{}} }+1})$ \\
%     $\wtd c_r = \bigcup_{v \in \wtd n} c^v$
% \smallskip
% \end{tabular}
% \\
%   \hline
%   %%%% RECURSIVE VARIABLE
%   $\rvar{X}$ &
% \begin{tabular}{l}
%   \noalign{\smallskip}
%     $\news{s_1}\big( \propinp{k}{z_x}\propout{k+1}{z_x}\apropout{k+2}{z_x} 
%     \Par $
%     $\propinp{k+2}{z_x}\bout{\dual s_1}{z_x}\apropout{k+3}{} 
%     \Par \propinp{k+3}{}\inact$ 
%      \\ 
%      $\qquad \qquad \propinp{k+1}{z_x}\news{a_1}
%      \big( \proprout{n_1}{a_1}\big($
%     %  \\
%     $
%     \binp{a_1}{y_1}\binp{y_1}{\widetilde z_1} \ldots \news{a_j}Q\big)\big)
%     % \Par \propinp{k+2}{z_x}\bout{\dual s_1}{z_x}\apropout{k+3}{} 
%     % \Par \propinp{k+3}{}\inact 
%     \big)$ 
%     \\ 
%     \text{where:} 
%     \\
%     $Q = \big(\proprout{n_j}{a_j}\big(\binp{a_j}{y_j}\binp{y_j}{\widetilde z_j}
%     \news{s'}\big(\bout{z_x}{s'}\about{\dual s'}{\widetilde z_1, \ldots, \widetilde z_j, s_1}\big)\big)\big)$
%  \smallskip
% \end{tabular}
% &
% \begin{tabular}{l}
% 	\noalign{\smallskip}
%       $\wtd n = g(X)$ \\
%       $\len{\widetilde n} = j$ \\
%       $i \in \{1, \dots, j\}$ \\
%       $\quad n_i : S \wedge \mathsf{tr}(S_i)$ \\
%       $\quad \widetilde{z_i} = (z_1^i, \dots, z_{\len{\mRts{}{}{S_i}}}^i)$
% \smallskip
% \end{tabular}
% % \\
% %   \hline
% %   $\inact$ &
% % \begin{tabular}{l}
% %   \noalign{\smallskip}
% %   $\propinp{k}{}\inact$
% %  \smallskip
% % \end{tabular}
% % &
% % \begin{tabular}{l}
% % 	\noalign{\smallskip}
% % \smallskip
% % \end{tabular}
%   \\
%   \hline
% \end{tabular}
% \caption{Decompose by composition: Breakdown function $\AmeliaMod{k}{\tilde x}{\cdot}_g$ for \sessp processes 
% (cf. Definition~\ref{def:am-decomp}). \label{table:repo}}
% \vspace{-4mm}
% \end{table*}

==> sources/c-table-rec-j.tex <==
\newcommand{\auxp}{B}
% \begin{figure*}

%     \begin{table}[H]
      \begin{tabular}{ |l|l|l|}
        \rowcolor{gray!25}
        \hline
        $P$ &
          \multicolumn{2}{l|}{
        \begin{tabular}{l}
          \noalign{\smallskip}
          $\Dbrecpi{k}{\tilde x, \rho}{P}^d_g$ $\text{ when } 
          g  \not= \es$
          \smallskip
        \end{tabular}
      } 
       \\
        \hline
               %%%%%%
      %% =======================
      %% =======================
      %%%%%%
      % $\Dbrecpi{k}{\tilde x, \rho}{\bout{u_i}{y_j}{Q}}^d_g$ & 
      $\bout{n_i}{y_j}{Q}$ &
      \begin{tabular}{l}
      \noalign{\smallskip}
      $\{\bout{n_l}{\wtd y\rho} \propoutrec{k+1}{\wtd z\rho}
      \recp{X}\binp{\prop^r_k}{\wtd x}
      \bout{n_l}{\wtd y} 
      \propoutrec{k+1}{\wtd z}\rvar{X}
    \Par$ 
     \\
    $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$ 
    \qquad \qquad \qquad 
    $\text{ if } \rvardepth{Q} = \recdep$
    \\
    \hdashline 
    \noalign{\smallskip}
    $N \cup \{\recp{X}\binp{\prop^r_k}{\wtd x}
      \bout{n_l}{\wtd y} 
      \propoutrec{k+1}{\wtd z}\rvar{X}
    \Par R$ 
     \\
    $: R \in \Dbrecpi{k+1}{\tilde z, \rho}{Q\sigma}^d_g\}$ 
    \qquad \qquad $\text{ otherwise }$
    \\
    % \hdashline 
    % \noalign{\smallskip}
    where: \\
    $ N = 
    \begin{cases}
    \{ \auxp
    %   \propoutrec{k+1}{\wtd z\rho}
    % \recp{X}\binp{\prop^r_k}{\wtd x}
    % \bout{n_l}{\wtd y} 
    % \propoutrec{k+1}{\wtd z}\rvar{X}
    \Par 
    % \\ 
    \Brecpi{k+1}{\tilde z}{Q\sigma}_g \} & \text{if } \rvardepth{Q} = \recdep + 1 \\ 
    \es & \text{otherwise}
    \end{cases} 
    $
    \\ 
    $ \auxp = \propoutrec{k+1}{\wtd z\rho}
    \recp{X}\binp{\prop^r_k}{\wtd x}
    \bout{n_l}{\wtd y} 
    \propoutrec{k+1}{\wtd z}\rvar{X}$
    %   \\
    %   $ \qquad N = \{\propoutrec{k+1}{\wtd z\rho}
    %   \recp{X}\binp{\prop^r_k}{\wtd x}
    %   \bout{n_l}{\wtd y} 
    %   \propoutrec{k+1}{\wtd z}\rvar{X}
    %  \Par$ 
    % $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$ $\text{ if } \rvardepth{Q} = \recdep + 1$  \\
    %   $\qquad N = \es$ $\texttt{ otherwise }$
    \smallskip
    \end{tabular} & 
    \begin{tabular}{l}
         \noalign{\smallskip}
         $y : T$ $\wedge (y_j,\ldots,y_{j+\len{\Gt{T}}-1})$ \\ 
      % $r:S \wedge \mathsf{tr}(S)$ \\
      $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
      $\wtd z = g(X) \cup \fnb{Q}{\wtd x \setminus \wtd w}$  \\
      $l = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
      $\sigma = \nextn{u_i}$
      \smallskip
    \end{tabular} 
    \\
    \hline 
    % $\Dbrecpi{k}{\tilde x}{\binp{u_i}{y}{Q}}^d_g$
    $\binp{n_i}{y}{Q}$
    &
    \begin{tabular}{l}
      \noalign{\smallskip}
       $\{\binp{n_l}{\wtd y} 
      \propoutrec{k+1}{\wtd z\rho}
      \recp{X}\binp{\prop^r_k}{\wtd x}
        \binp{n_l}{\wtd y} 
        \propoutrec{k+1}{\wtd z}
        \rvar{X}
       \Par$ 
       \\
      $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$ 
      \qquad \qquad \qquad 
      $\text{ if } \rvardepth{Q} = \recdep$
      \\
      \hdashline 
      \noalign{\smallskip}
      $N \cup \{\recp{X}\binp{\prop^r_k}{\widetilde x}
        \binp{n_l}{\widetilde y} 
        \propoutrec{k+1}{\wtd z}
        \rvar{X}
       \Par R$ 
       \\
      $: R \in \Dbrecpi{k+1}{\tilde z, \rho}{Q\sigma}^d_g\}$ 
      \qquad \qquad 
      $\text{otherwise}$
      \\
      where: 
      \\
      % \hdashline 
      % \noalign{\smallskip}
      $N = 
      \begin{cases} 
        \{ \auxp 
      %     \propoutrec{k+1}{\wtd z\rho}
      % \recp{X}\binp{\prop^r_k}{\wtd x}
      %   \binp{n_l}{\wtd y} 
      %   \propoutrec{k+1}{\wtd z}
      %   \rvar{X}
       \Par
      %  \\
      \Brecpi{k+1}{\tilde z}{Q\sigma}_g \} & \text{ if } \rvardepth{Q} = \recdep + 1 \\
      \es & \text{ otherwise }
      \end{cases}
      $
      \\ 
      $\auxp =   \propoutrec{k+1}{\wtd z\rho}
      \recp{X}\binp{\prop^r_k}{\wtd x}
        \binp{n_l}{\wtd y} 
        \propoutrec{k+1}{\wtd z}
        \rvar{X}$
      \smallskip 
    \end{tabular} & 
    \begin{tabular}{l}
         \noalign{\smallskip}
      % $r:S \wedge \mathsf{tr}(S)$ \\
      $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
      $\wtd z = g(X) \cup \fnb{Q}{\wtd x \wtd y \setminus \wtd w}$  \\
      $l = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
      $\sigma = \nextn{u_i} \cdot \subst{y_1}{y}$
      % $\wtd z = \fnb{Q}{\wtd x \wtd y}$  
      \smallskip
    \end{tabular} 
    \\
    \hline
    % $\Dbrecpi{k}{\tilde x,\rho}{Q_1 \Par Q_2}^d_g$
    $Q_1 \Par Q_2$
    & 
    \begin{tabular}{l}
      \noalign{\smallskip}
      $ N \cup \{\recp{X}\proprinpk{r}{k}{\wtd x}
      (\proproutk{r}{k+1}{\wtd y_1}\rvar{X}
      \Par \apropoutrecsh{k+\degree+1}{\wtd y_2}) 
       \Par$ 
       \\
      $R_1 \Par R_2 :$  \\
      $R_1 \in \Dbrecpi{k+1}{\tilde y_1, \rho}{Q_1}^d_{g_1}, 
      R_2 \in \Dbrecpi{k+\degree+1}{\tilde y_2, \rho}{Q_2}^d_{g_2}\}$ 
      % $\cup$ $N$
      \\
      % \hdashline 
      where: 
      \\ 
      % \noalign{\smallskip}
      $ N = 
      \begin{cases} 
     \{ \auxp 
      % \proproutk{r}{k+1}{\wtd y_1\rho}
      % \recp{X}\proprinpk{r}{k}{\wtd x} (\proproutk{r}{k+1}{\wtd y_1}\rvar{X}
      % \Par 
      % \apropoutrecsh{k+\degree+1}{\wtd y_2})
       \Par
      %  \\
       \Brecpi{k+1}{\tilde y_1}{Q_1}_{g_1} \Par 
       \\
      \Brecpi{k+\degree+1}{\tilde y_2}{Q_2}_{g_2}\} & \text{ if } \rvardepth{Q_1} = \recdep \\
      \es & \text{ otherwise }
      \end{cases}
      $
      \\ 
      $ \auxp = \proproutk{r}{k+1}{\wtd y_1\rho}
      \recp{X}\proprinpk{r}{k}{\wtd x} (\proproutk{r}{k+1}{\wtd y_1}\rvar{X}
      \Par$ 
      \\ 
      \qquad \qquad \qquad \qquad \qquad \qquad 
      $\apropoutrecsh{k+\degree+1}{\wtd y_2})$
      \smallskip 
    \smallskip
    \end{tabular} & 
    \begin{tabular}{l}
           \noalign{\smallskip}
           $\recpx{Q_1}$ \\
           $\wtd y_1  = g(X) \cup \fnb{Q_1}{\wtd x}$ \\
           $\wtd y_2  =  \fnb{Q_2}{\wtd x}$ \\
          %  $i \in \{1,2\}.$ \\
          %  $\quad \wtd y_i' = \linecondit{\recpx{Q_i}}{g(X)}{\epsilon}$ \\
          %  $\quad g_i = \linecondit{\recpx{Q_i}}{g_i}{\epsilon}$ \\
          %  $\quad \wtd y_i  = \wtd y_i' \cup \fnb{Q_i}{\wtd x}$ \\
           $\degree = \lenHOopt{Q_1}$
      \smallskip
    \end{tabular} 
    \\
    \hline
    % $\Dbrecpi{k}{\tilde x, \rho}{\news{s:C}{Q}}^d_g$ & 
    $\news{s}{Q}$ &
    \begin{tabular}{l}
      \noalign{\smallskip}
      $N \cup \{\recp{X}\news{\widetilde{s}:\Gt{C}}\propinp{k}{\wtd x}\propout{k+1}{\wtd z}X$
      $\Par$
      \\ 
      $R : R \in \Dbrecpi{k+1}{\tilde z, \rho}{Q \sigma }^d_g \}$
      \\
      \hdashline 
      \noalign{\smallskip}
      % $R = \propout{k+1}{\wtd z\rho}
      % \recp{X}\news{\wtd{s}:\Gt{C}}\propinp{k}{\wtd x}\propout{k+1}{\wtd z}X$ \\
      $ N = 
      \begin{cases}
      \{\news{\wtd{s}:\Gt{C}} B 
      \Par
      \\ 
      \Brecpi{k+1}{\tilde z}{Q\sigma}_g\} &  \text{ if } \rvardepth{Q_1} = \recdep \\
      \es & \text{ otherwise }
      \end{cases}
      $
      \\ 
       $B = \propout{k+1}{\wtd z\rho}
      \recp{X}\news{\wtd{s}:\Gt{C}}\propinp{k}{\wtd x}\propout{k+1}{\wtd z}X$ 
    \smallskip
    \end{tabular} & 
    \begin{tabular}{l}
      \noalign{\smallskip}
        %  $\mathsf{tr}(\trec{t}{S})$ \\
        $s : S$ \\ 
         $\widetilde{s} = (s_1,\ldots,s_{\len{\Gt{S}}})$ \\
         $\widetilde {\dual{s}} =  (\dual{s_1},\ldots,\dual{s_{\len{\Gt{S}}}})$ \\
         $\wtd n =
          \linecondit{\lin{s}}{\wtd n}{\epsilon}$ \\
    %        $\widetilde {\dual{s}} = \begin{cases}
    %         (\dual{s_1},\ldots,\dual{s_{\len{\Gt{S}}}}) & \text{if} \ C = S \\
    %         \epsilon & \text{if} \ C = \chtype{U}
    % \end{cases}
    % $\\
        %  $\widetilde {\dual{s}} = (\dual{s_1},\ldots,\dual{s_{\len{\Rtopt{S}}}})$ \\
         $\wtd z = \wtd x, \wtd s, \wtd n$ \\
         $\sigma = \subst{s_1 \dual{s_1}}{s \dual{s}} $
      \smallskip
    \end{tabular} 
    \\
    \hline
    % $\Brecpi{k}{\tilde x}{X}_g$ 
    $X$
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $\inact$
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    
    \\ 
        \rowcolor{gray!25}
        \hline
        $P$ &
          \multicolumn{2}{l|}{
        \begin{tabular}{l}
          \noalign{\smallskip}
          $\Dbrecpi{k}{\tilde x, \rho}{P}^d_g$ $\text{ when } g = \es$
          \smallskip
        \end{tabular}
      } 
       \\
        \hline
               %%%%%%
      %% =======================
      %% =======================
      %%%%%%
      $\bout{n_i}{y_j}{Q}$
      &  
      \begin{tabular}{l}
      \noalign{\smallskip}
      $ \{
      \bout{n_{\mstindex}}{\wtd y\rho} \apropoutrecsh{k+1}{\wtd z\rho} \Par  
      \recp{X}\propinprecsh{k}{\wtd x}
      (\bout{n_{\mstindex}}{\wtd y} \apropoutrecsh{k+1}{\wtd z}
      \Par \rvar{X}) 
     \Par$
     \\ 
    $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$
      \smallskip
      \end{tabular}
      & 
      \begin{tabular}{l}
             \noalign{\smallskip}
            %  $\wtd x = g(X)$
          \smallskip
      \end{tabular} 
    \\ \hline     
    $\binp{n_i}{y}{Q}$
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $
    \{\binp{n_{\mstindex}}{\wtd y} \apropoutrecsh{k+1}{\wtd z\rho}  \Par 
    \recp{X}\propinprecsh{k}{\wtd x}
    (\binp{n_{\mstindex}}{\wtd y} 
    \apropoutrecsh{k+1}{\wtd z} \Par \rvar{X}) 
    \Par$ 
     \\
    $\Brecpi{k+1}{\tilde z}{Q\sigma}_g\}$ 
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    \\ \hline    
    $Q_1 \Par Q_2$
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $
    \{\apropoutrecsh{k+1}{\wtd y_1\rho}
    \Par$ 
    \\ 
    $\apropoutrecsh{k+\degree+1}{\wtd y_2\rho} \Par 
    \recp{X}\proprinpk{r}{k}{\wtd x}(\apropoutrecsh{k+1}{\wtd y_1}
    \Par \apropoutrecsh{k+\degree+1}{\wtd y_2} \Par \rvar{X})
    \Par$ 
    \\
    $\Brecpi{k+1}{\tilde y_1}{Q_1}_{g_1} \Par 
    \Brecpi{k+\degree+1}{\tilde y_2}{Q_2}_{g_2}\}$ 
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    \\ \hline    
    $\news{s:C}{Q}$ 
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $
    \{\apropoutrecsh{k+1}{\wtd z\rho} \Par 
    \recp{X}\news{\wtd{s}:\Gt{C}}
    \propinp{k}{\wtd x}(\apropoutrecsh{k+1}{\wtd z} \Par X)$
    $\Par$
    \\
    $\Brecpi{k+1}{\tilde z}{Q}_g\}$
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    \\ \hline    
      \end{tabular}
    %   \caption{The extension of $\Cbpi{\tilde u}{\tilde x}{P}$ 
    %   and definition of $\Dbrecpi{k}{\tilde x, \rho}{P}^d_g$
    %   (recursion extension). Side conditions for 
    %   last four rows ($g = \es$) are the same as for corresponding 
    %   cases when $g \not = \es$. \label{pi:t:tablecd-rec}}
    %   \vspace{-2mm}
    %   \end{table}
    % \end{figure*}

==> sources/c-table-rec-j2_copy.tex <==
\newcommand{\auxp}{B}
% \begin{figure*}

%     \begin{table}[H]
      \begin{tabular}{ |l|l|l|}
    %     \rowcolor{gray!25}
    %     \hline
    %     $P$ &
    %       \multicolumn{2}{l|}{
    %     \begin{tabular}{l}
    %       \noalign{\smallskip}
    %       $\Dbrecpi{k}{\tilde x, \rho}{P}^d_g$ $\text{ when } 
    %       g  \not= \es$
    %       \smallskip
    %     \end{tabular}
    %   } 
    %    \\
    %     \hline
    %            %%%%%%
    %   %% =======================
    %   %% =======================
    %   %%%%%%
    %   % $\Dbrecpi{k}{\tilde x, \rho}{\bout{u_i}{y_j}{Q}}^d_g$ & 
    %   $\bout{n_i}{y_j}{Q}$ &
    %   \begin{tabular}{l}
    %   \noalign{\smallskip}
    %   $\{\bout{n_l}{\wtd y\rho} \propoutrec{k+1}{\wtd z\rho}
    %   \recp{X}\binp{\prop^r_k}{\wtd x}
    %   \bout{n_l}{\wtd y} 
    %   \propoutrec{k+1}{\wtd z}\rvar{X}
    % \Par$ 
    %  \\
    % $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$ 
    % \qquad \qquad \qquad 
    % $\text{ if } \rvardepth{Q} = \recdep$
    % \\
    % \hdashline 
    % \noalign{\smallskip}
    % $N \cup \{\recp{X}\binp{\prop^r_k}{\wtd x}
    %   \bout{n_l}{\wtd y} 
    %   \propoutrec{k+1}{\wtd z}\rvar{X}
    % \Par R$ 
    %  \\
    % $: R \in \Dbrecpi{k+1}{\tilde z, \rho}{Q\sigma}^d_g\}$ 
    % \qquad \qquad $\text{ otherwise }$
    % \\
    % % \hdashline 
    % % \noalign{\smallskip}
    % where: \\
    % $ N = 
    % \begin{cases}
    % \{ \auxp
    % %   \propoutrec{k+1}{\wtd z\rho}
    % % \recp{X}\binp{\prop^r_k}{\wtd x}
    % % \bout{n_l}{\wtd y} 
    % % \propoutrec{k+1}{\wtd z}\rvar{X}
    % \Par 
    % % \\ 
    % \Brecpi{k+1}{\tilde z}{Q\sigma}_g \} & \text{if } \rvardepth{Q} = \recdep + 1 \\ 
    % \es & \text{otherwise}
    % \end{cases} 
    % $
    % \\ 
    % $ \auxp = \propoutrec{k+1}{\wtd z\rho}
    % \recp{X}\binp{\prop^r_k}{\wtd x}
    % \bout{n_l}{\wtd y} 
    % \propoutrec{k+1}{\wtd z}\rvar{X}$
    % %   \\
    % %   $ \qquad N = \{\propoutrec{k+1}{\wtd z\rho}
    % %   \recp{X}\binp{\prop^r_k}{\wtd x}
    % %   \bout{n_l}{\wtd y} 
    % %   \propoutrec{k+1}{\wtd z}\rvar{X}
    % %  \Par$ 
    % % $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$ $\text{ if } \rvardepth{Q} = \recdep + 1$  \\
    % %   $\qquad N = \es$ $\texttt{ otherwise }$
    % \smallskip
    % \end{tabular} & 
    % \begin{tabular}{l}
    %      \noalign{\smallskip}
    %      $y : T$ $\wedge (y_j,\ldots,y_{j+\len{\Gt{T}}-1})$ \\ 
    %   % $r:S \wedge \mathsf{tr}(S)$ \\
    %   $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
    %   $\wtd z = g(X) \cup \fnb{Q}{\wtd x \setminus \wtd w}$  \\
    %   $l = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
    %   $\sigma = \nextn{u_i}$
    %   \smallskip
    % \end{tabular} 
    % \\
    % \hline 
    % % $\Dbrecpi{k}{\tilde x}{\binp{u_i}{y}{Q}}^d_g$
    % $\binp{n_i}{y}{Q}$
    % &
    % \begin{tabular}{l}
    %   \noalign{\smallskip}
    %    $\{\binp{n_l}{\wtd y} 
    %   \propoutrec{k+1}{\wtd z\rho}
    %   \recp{X}\binp{\prop^r_k}{\wtd x}
    %     \binp{n_l}{\wtd y} 
    %     \propoutrec{k+1}{\wtd z}
    %     \rvar{X}
    %    \Par$ 
    %    \\
    %   $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$ 
    %   \qquad \qquad \qquad 
    %   $\text{ if } \rvardepth{Q} = \recdep$
    %   \\
    %   \hdashline 
    %   \noalign{\smallskip}
    %   $N \cup \{\recp{X}\binp{\prop^r_k}{\widetilde x}
    %     \binp{n_l}{\widetilde y} 
    %     \propoutrec{k+1}{\wtd z}
    %     \rvar{X}
    %    \Par R$ 
    %    \\
    %   $: R \in \Dbrecpi{k+1}{\tilde z, \rho}{Q\sigma}^d_g\}$ 
    %   \qquad \qquad 
    %   $\text{otherwise}$
    %   \\
    %   where: 
    %   \\
    %   % \hdashline 
    %   % \noalign{\smallskip}
    %   $N = 
    %   \begin{cases} 
    %     \{ \auxp 
    %   %     \propoutrec{k+1}{\wtd z\rho}
    %   % \recp{X}\binp{\prop^r_k}{\wtd x}
    %   %   \binp{n_l}{\wtd y} 
    %   %   \propoutrec{k+1}{\wtd z}
    %   %   \rvar{X}
    %    \Par
    %   %  \\
    %   \Brecpi{k+1}{\tilde z}{Q\sigma}_g \} & \text{ if } \rvardepth{Q} = \recdep + 1 \\
    %   \es & \text{ otherwise }
    %   \end{cases}
    %   $
    %   \\ 
    %   $\auxp =   \propoutrec{k+1}{\wtd z\rho}
    %   \recp{X}\binp{\prop^r_k}{\wtd x}
    %     \binp{n_l}{\wtd y} 
    %     \propoutrec{k+1}{\wtd z}
    %     \rvar{X}$
    %   \smallskip 
    % \end{tabular} & 
    % \begin{tabular}{l}
    %      \noalign{\smallskip}
    %   % $r:S \wedge \mathsf{tr}(S)$ \\
    %   $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
    %   $\wtd z = g(X) \cup \fnb{Q}{\wtd x \wtd y \setminus \wtd w}$  \\
    %   $l = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
    %   $\sigma = \nextn{u_i} \cdot \subst{y_1}{y}$
    %   % $\wtd z = \fnb{Q}{\wtd x \wtd y}$  
    %   \smallskip
    % \end{tabular} 
    % \\
    % \hline
    % % $\Dbrecpi{k}{\tilde x,\rho}{Q_1 \Par Q_2}^d_g$
    % $Q_1 \Par Q_2$
    % & 
    % \begin{tabular}{l}
    %   \noalign{\smallskip}
    %   $ N \cup \{\recp{X}\proprinpk{r}{k}{\wtd x}
    %   (\proproutk{r}{k+1}{\wtd y_1}\rvar{X}
    %   \Par \apropoutrecsh{k+\degree+1}{\wtd y_2}) 
    %    \Par$ 
    %    \\
    %   $R_1 \Par R_2 :$  \\
    %   $R_1 \in \Dbrecpi{k+1}{\tilde y_1, \rho}{Q_1}^d_{g_1}, 
    %   R_2 \in \Dbrecpi{k+\degree+1}{\tilde y_2, \rho}{Q_2}^d_{g_2}\}$ 
    %   % $\cup$ $N$
    %   \\
    %   % \hdashline 
    %   where: 
    %   \\ 
    %   % \noalign{\smallskip}
    %   $ N = 
    %   \begin{cases} 
    %  \{ \auxp 
    %   % \proproutk{r}{k+1}{\wtd y_1\rho}
    %   % \recp{X}\proprinpk{r}{k}{\wtd x} (\proproutk{r}{k+1}{\wtd y_1}\rvar{X}
    %   % \Par 
    %   % \apropoutrecsh{k+\degree+1}{\wtd y_2})
    %    \Par
    %   %  \\
    %    \Brecpi{k+1}{\tilde y_1}{Q_1}_{g_1} \Par 
    %    \\
    %   \Brecpi{k+\degree+1}{\tilde y_2}{Q_2}_{g_2}\} & \text{ if } \rvardepth{Q_1} = \recdep \\
    %   \es & \text{ otherwise }
    %   \end{cases}
    %   $
    %   \\ 
    %   $ \auxp = \proproutk{r}{k+1}{\wtd y_1\rho}
    %   \recp{X}\proprinpk{r}{k}{\wtd x} (\proproutk{r}{k+1}{\wtd y_1}\rvar{X}
    %   \Par$ 
    %   \\ 
    %   \qquad \qquad \qquad \qquad \qquad \qquad 
    %   $\apropoutrecsh{k+\degree+1}{\wtd y_2})$
    %   \smallskip 
    % \smallskip
    % \end{tabular} & 
    % \begin{tabular}{l}
    %        \noalign{\smallskip}
    %        $\recpx{Q_1}$ \\
    %        $\wtd y_1  = g(X) \cup \fnb{Q_1}{\wtd x}$ \\
    %        $\wtd y_2  =  \fnb{Q_2}{\wtd x}$ \\
    %       %  $i \in \{1,2\}.$ \\
    %       %  $\quad \wtd y_i' = \linecondit{\recpx{Q_i}}{g(X)}{\epsilon}$ \\
    %       %  $\quad g_i = \linecondit{\recpx{Q_i}}{g_i}{\epsilon}$ \\
    %       %  $\quad \wtd y_i  = \wtd y_i' \cup \fnb{Q_i}{\wtd x}$ \\
    %        $\degree = \lenHOopt{Q_1}$
    %   \smallskip
    % \end{tabular} 
    % \\
    % \hline
    % % $\Dbrecpi{k}{\tilde x, \rho}{\news{s:C}{Q}}^d_g$ & 
    % $\news{s}{Q}$ &
    % \begin{tabular}{l}
    %   \noalign{\smallskip}
    %   $N \cup \{\recp{X}\news{\widetilde{s}:\Gt{C}}\propinp{k}{\wtd x}\propout{k+1}{\wtd z}X$
    %   $\Par$
    %   \\ 
    %   $R : R \in \Dbrecpi{k+1}{\tilde z, \rho}{Q \sigma }^d_g \}$
    %   \\
    %   \hdashline 
    %   \noalign{\smallskip}
    %   % $R = \propout{k+1}{\wtd z\rho}
    %   % \recp{X}\news{\wtd{s}:\Gt{C}}\propinp{k}{\wtd x}\propout{k+1}{\wtd z}X$ \\
    %   $ N = 
    %   \begin{cases}
    %   \{\news{\wtd{s}:\Gt{C}} B 
    %   \Par
    %   \\ 
    %   \Brecpi{k+1}{\tilde z}{Q\sigma}_g\} &  \text{ if } \rvardepth{Q_1} = \recdep \\
    %   \es & \text{ otherwise }
    %   \end{cases}
    %   $
    %   \\ 
    %    $B = \propout{k+1}{\wtd z\rho}
    %   \recp{X}\news{\wtd{s}:\Gt{C}}\propinp{k}{\wtd x}\propout{k+1}{\wtd z}X$ 
    % \smallskip
    % \end{tabular} & 
    % \begin{tabular}{l}
    %   \noalign{\smallskip}
    %     %  $\mathsf{tr}(\trec{t}{S})$ \\
    %     $s : S$ \\ 
    %      $\widetilde{s} = (s_1,\ldots,s_{\len{\Gt{S}}})$ \\
    %      $\widetilde {\dual{s}} =  (\dual{s_1},\ldots,\dual{s_{\len{\Gt{S}}}})$ \\
    %      $\wtd n =
    %       \linecondit{\lin{s}}{\wtd n}{\epsilon}$ \\
    % %        $\widetilde {\dual{s}} = \begin{cases}
    % %         (\dual{s_1},\ldots,\dual{s_{\len{\Gt{S}}}}) & \text{if} \ C = S \\
    % %         \epsilon & \text{if} \ C = \chtype{U}
    % % \end{cases}
    % % $\\
    %     %  $\widetilde {\dual{s}} = (\dual{s_1},\ldots,\dual{s_{\len{\Rtopt{S}}}})$ \\
    %      $\wtd z = \wtd x, \wtd s, \wtd n$ \\
    %      $\sigma = \subst{s_1 \dual{s_1}}{s \dual{s}} $
    %   \smallskip
    % \end{tabular} 
    % \\
    % \hline
    % % $\Brecpi{k}{\tilde x}{X}_g$ 
    % $X$
    % &  
    % \begin{tabular}{l}
    % \noalign{\smallskip}
    % $\inact$
    % \smallskip
    % \end{tabular}
    % & 
    % \begin{tabular}{l}
    %      \noalign{\smallskip}
    %     %  $\wtd x = g(X)$
    %   \smallskip
    % \end{tabular} 
    
    % \\ 
        \rowcolor{gray!25}
        \hline
        $P$ &
          \multicolumn{2}{l|}{
        \begin{tabular}{l}
          \noalign{\smallskip}
          $\Dbrecpi{k}{\tilde x, \rho}{P}^d_g$ $\text{ when } g = \es$
          \smallskip
        \end{tabular}
      } 
       \\
        \hline
               %%%%%%
      %% =======================
      %% =======================
      %%%%%%
      $\bout{n_i}{y_j}{Q}$
      &  
      \begin{tabular}{l}
      \noalign{\smallskip}
      $ \{
      \bout{n_{\mstindex}}{\wtd y\rho} \apropoutrecsh{k+1}{\wtd z\rho} \Par  
      \recp{X}\propinprecsh{k}{\wtd x}
      (\bout{n_{\mstindex}}{\wtd y} \apropoutrecsh{k+1}{\wtd z}
      \Par \rvar{X}) 
     \Par$
     \\ 
    $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$
      \smallskip
      \end{tabular}
      & 
      \begin{tabular}{l}
             \noalign{\smallskip}
            %  $\wtd x = g(X)$
          \smallskip
      \end{tabular} 
    \\ \hline     
    $\binp{n_i}{y}{Q}$
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $
    \{\binp{n_{\mstindex}}{\wtd y} \apropoutrecsh{k+1}{\wtd z\rho}  \Par 
    \recp{X}\propinprecsh{k}{\wtd x}
    (\binp{n_{\mstindex}}{\wtd y} 
    \apropoutrecsh{k+1}{\wtd z} \Par \rvar{X}) 
    \Par$ 
     \\
    $\Brecpi{k+1}{\tilde z}{Q\sigma}_g\}$ 
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    \\ \hline    
    $Q_1 \Par Q_2$
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $
    \{\apropoutrecsh{k+1}{\wtd y_1\rho}
    \Par$ 
    \\ 
    $\apropoutrecsh{k+\degree+1}{\wtd y_2\rho} \Par 
    \recp{X}\proprinpk{r}{k}{\wtd x}(\apropoutrecsh{k+1}{\wtd y_1}
    \Par \apropoutrecsh{k+\degree+1}{\wtd y_2} \Par \rvar{X})
    \Par$ 
    \\
    $\Brecpi{k+1}{\tilde y_1}{Q_1}_{g_1} \Par 
    \Brecpi{k+\degree+1}{\tilde y_2}{Q_2}_{g_2}\}$ 
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    \\ \hline    
    $\news{s:C}{Q}$ 
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $
    \{\apropoutrecsh{k+1}{\wtd z\rho} \Par 
    \recp{X}\news{\wtd{s}:\Gt{C}}
    \propinp{k}{\wtd x}(\apropoutrecsh{k+1}{\wtd z} \Par X)$
    $\Par$
    \\
    $\Brecpi{k+1}{\tilde z}{Q}_g\}$
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    \\ \hline    
      \end{tabular}
    %   \caption{The extension of $\Cb{\tilde u}{\tilde x}{P}$ 
    %   and definition of $\Dbrecpi{k}{\tilde x, \rho}{P}^d_g$
    %   (recursion extension). Side conditions for 
    %   last four rows ($g = \es$) are the same as for corresponding 
    %   cases when $g \not = \es$. \label{pi:t:tablecd-rec}}
    %   \vspace{-2mm}
    %   \end{table}
    % \end{figure*}

==> sources/c-table-rec.tex <==

% \begin{figure*}

%     \begin{table}[H]
      \begin{tabular}{ |l|l|l|}
        \rowcolor{gray!25}
    \hline
    $P$ &
      \multicolumn{2}{l|}{
    \begin{tabular}{l}
      \noalign{\smallskip}
      $\Cbpi{\tilde u}{\tilde x}{P}$
      \smallskip
    \end{tabular} 
    } 
    %   \\
    %   \hline
    % $Q_1 \parallel Q_2$ 
    % &
    %   \begin{tabular}{l}
    %   \noalign{\smallskip}
    %      $\{ R_1 \parallel R_2: 
    %      R_1 \in \Cbpi{\tilde u_1}{\tilde y}{Q_1}, 
    %      R_2 \in \Cbpi{\tilde u_2}{\tilde z}{Q_2}
    %      \}$
    %      \smallskip 
    %   \end{tabular}
    %   &
    %   %side-conditions
    %   \begin{tabular}{l}
    %     \noalign{\smallskip}
    %     $\wtd y = \fnb{Q_1}{\tilde x}$, $\wtd z = \fnb{Q_2}{\tilde x}$ \\
    %     $\subst{\tilde u}{\tilde x} = \subst{\tilde u_1}{\tilde y} \cdot \subst{\tilde u_2}{\tilde z}$ 
    %     \smallskip
    %   \end{tabular}
    %      \\
    %      \hline
    %      $\news{s:C}{Q}$ &
    %      \begin{tabular}{l}
    %        \noalign{\smallskip}
    %         $\{\news{\widetilde{s}:\Gt{C}}{\,R} : \Cbpi{\tilde u}{\tilde x}{Q\sigma} \}$
    %        \smallskip
    %      \end{tabular}
    %      &
    %      %side-conditions
    %      \begin{tabular}{l}
    %        \noalign{\smallskip}
    %        $\widetilde{s} = (s_1,\ldots,s_{\len{\Gt{C}}})$ \\
    %        $\sigma =  \subst{s_1 \dual{s_1}}{s \dual{s}}$
    %       %  $\sigma = \begin{cases}
    %       %              \subst{s_1 \dual{s_1}}{s \dual{s}} & \text{if} \ C = S \\
    %       %              \subst{s_1}{s} & \text{if} \ C = \chtype{U}
    %   %  \end{cases}
    %   %  $
    %        \smallskip
    %      \end{tabular}
    %      \\
    %      \hline
    %   $Q$
    %   &
    %   \begin{tabular}{l}
    %   \noalign{\smallskip}
    %      $\{  \news{\wtd \prop} R \,:\,  
    %   R = \apropout{k}{\wtd u} \Par \B{k}{\tilde x}{Q} \}$ 
    %   % \\
    %   $\cup~ \{ \news{\wtd \prop}R \,:\, R \in \Dbpi{\tilde u}{\tilde x}{Q}\}$
    %   \smallskip 
    %   \end{tabular}
    %   &
    %   %side-conditions
    %   \begin{tabular}{l}
    %     \noalign{\smallskip}
    %     $\wtd \prop = \fpn{R}$
    %     \smallskip
    %   \end{tabular} 
    %   \\
    %   \hline 
    %     $\inact$ &
    %   \begin{tabular}{l}
    %     \noalign{\smallskip}
    %     $\{\inact\}$
    %    \smallskip
    %   \end{tabular}
    %   &
    %   \begin{tabular}{l}
    %       \noalign{\smallskip}
    %   %$\widetilde x = \es$ 
    %   \smallskip
    %   \end{tabular}
    \\
       \hline
    $Q$
    &
    \begin{tabular}{l}
    \noalign{\smallskip}
    % $f$ \\
    $\Cbrecpi{\tilde u}{\tilde x}{\recp{X}Q^*}^d$
    $\text{ if } Q \equiv \alpha_d.\alpha_{d-1}. \ldots .\alpha_{d-p}.(P_X \Par R)$
    \\ 
    and $\recp{X}Q^*$ is a subprocess of $P_X$
    \smallskip 
    \\
    \hdashline 
    \noalign{\smallskip}
      % $\{  \news{\wtd \prop} R \,:\,  
      % R = \apropout{k}{\wtd u} \Par \B{k}{\tilde x}{Q} \}$ 
      $\{  \news{\wtd \prop} R \,:\,  
      R \in \{\apropout{k}{\wtd u} \Par \B{k}{\tilde x}{Q}, 
      \apropoutrecsh{k}{\wtd u}{} \Par \Brecpi{k}{\tilde x}{Q} \} \}$
      \\
      $\cup~ \{ \news{\wtd \prop}R \,:\, R \in 
      \Dbpi{\tilde u}{\tilde x}{Q} \cup \Dbrecpi{k}{\tilde x, \rho}{Q}^d_\es\}$ 
      $\text{ otherwise }$
    \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{l}
      \noalign{\smallskip}
      $\wtd \prop = \fpn{R}$ \\
      $\rho = \subst{\tilde u}{\tilde x}$
      \smallskip
    \end{tabular} 
    \\
    \hline 
    $\Cbrecpi{\tilde u}{\tilde x}{Q}^d$
    % $\recp{X}Q$
    &
    \begin{tabular}{l}
    \noalign{\smallskip}
    $ \{\news{\wtd \prop} (
      \recp{X}\binp{\prop^r_{X}}{\wtd y}
    \propoutrec{k+1}{\wtd y}X \Par R 
    \Par  
    \proprinpk{r}{k}{\wtd x}\propoutrecsh{\rvar{X}}{\wtd x}\rvar{X}:
     R \in \Dbrecpi{k}{\tilde x}{Q}^d_g \}$ $\cup N$ \\
     where: \\
     $M = 
     \begin{cases}
      \{  \news{\wtd \prop} (
      \recp{X}\binp{\prop^r_{X}}{\wtd y}
    \propoutrec{k+1}{\wtd y}X \Par R  \Par \\
    \propoutrecsh{\rvar{X}}{\wtd x\rho}
    \recp{X}\proprinpk{r}{k}{\wtd x}\propoutrecsh{\rvar{X}}{\wtd x}\rvar{X}
    )  \,:\, R \in \Dbrecpi{k}{\tilde x}{Q}^0_g \} & \text{ if } g \not= \es \\
    \{  \news{\wtd \prop} (
      \recp{X}\binp{\prop^r_{X}}{}
    \propoutrec{k+1}{}X \Par R  \Par  \\
    \apropoutrecsh{\rvar{X}}{} \Par 
    \recp{X}\proprinpk{r}{k}{}(\apropoutrecsh{\rvar{X}}{} \Par \rvar{X})
    )  \,:\, R \in \Dbrecpi{k}{\tilde x}{Q}^0_g \} & \text{ otherwise }
     \end{cases}$ 
     \\
    % $M_2 = \{  \news{\wtd \prop} (
    %   \recp{X}\binp{\prop^r_{X}}{\wtd y}
    % \propoutrec{k+1}{\wtd y}X \Par R$  \\
    % $\qquad \Par 
    % \proproutk{r}{\rvar{X}}{\wtd x\rho}
    % \recp{X}\proprinpk{r}{k}{\wtd x}\propoutrecsh{\rvar{X}}{\wtd x}\rvar{X}
    % )  \,:\, R \in \Dbrecpi{k}{\tilde x}{Q}^0_g \}$ \\
    $N =
    \begin{cases}
       \{  \news{\wtd \prop} (\propoutrec{k}{\wtd z\rho}
    \recp{X}\binp{\prop^r_{X}}{\wtd y}
    \propoutrec{k}{\wtd y}X \Par \Brecpi{k}{\tilde x}{Q}_g ) \}
    % \\
    \cup~ M & \text{ if } \recdep = 0 \\ 
    \emptyset & \text{otherwise}
    \end{cases}
    $
       \smallskip 
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{l}
      \noalign{\smallskip}
      % $\recdep = \rvardepth{Q}$
      $\wtd \prop = \fpn{R}$ \\
      $Q \equiv \recp{X} Q^*$ \\
      $\wtd x = \fs{Q^*}$ \\
      $g = \{ X \mapsto \wtd x\}$ \\
      $\rho = \subst{\tilde u}{\tilde x}$
      \smallskip
    \end{tabular}
    \\ 
        \rowcolor{gray!25}
        \hline
        $P$ &
          \multicolumn{2}{l|}{
        \begin{tabular}{l}
          \noalign{\smallskip}
          $\Dbrecpi{k}{\tilde x, \rho}{P}^d_g$ $\text{ when } 
          g  \not= \es$
          \smallskip
        \end{tabular}
      } 
       \\
        \hline
               %%%%%%
      %% =======================
      %% =======================
      %%%%%%
      % $\Dbrecpi{k}{\tilde x, \rho}{\bout{u_i}{y_j}{Q}}^d_g$ & 
      $\bout{n_i}{y_j}{Q}$ &
      \begin{tabular}{l}
      \noalign{\smallskip}
      $\{\bout{n_l}{\wtd y\rho} \propoutrec{k+1}{\wtd z\rho}
      \recp{X}\binp{\prop^r_k}{\wtd x}
      \bout{n_l}{\wtd y} 
      \propoutrec{k+1}{\wtd z}\rvar{X}
    \Par$ 
    %  \\
    $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$ $\text{ if } \rvardepth{Q} = \recdep$
    \\
    \hdashline 
    \noalign{\smallskip}
    $N \cup \{\recp{X}\binp{\prop^r_k}{\wtd x}
      \bout{n_l}{\wtd y} 
      \propoutrec{k+1}{\wtd z}\rvar{X}
    \Par$ 
    %  \\
    $R : R \in \Dbrecpi{k+1}{\tilde z, \rho}{Q\sigma}^d_g\}$ $\text{ otherwise }$
    \\
    % \hdashline 
    % \noalign{\smallskip}
    where: \\
    $ N = 
    \begin{cases}
    \{\propoutrec{k+1}{\wtd z\rho}
    \recp{X}\binp{\prop^r_k}{\wtd x}
    \bout{n_l}{\wtd y} 
    \propoutrec{k+1}{\wtd z}\rvar{X}
    \Par \Brecpi{k+1}{\tilde z}{Q\sigma}_g \} & \text{if } \rvardepth{Q} = \recdep + 1 \\ 
    \es & \text{otherwise}
    \end{cases} 
    $
    %   \\
    %   $ \qquad N = \{\propoutrec{k+1}{\wtd z\rho}
    %   \recp{X}\binp{\prop^r_k}{\wtd x}
    %   \bout{n_l}{\wtd y} 
    %   \propoutrec{k+1}{\wtd z}\rvar{X}
    %  \Par$ 
    % $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$ $\text{ if } \rvardepth{Q} = \recdep + 1$  \\
    %   $\qquad N = \es$ $\texttt{ otherwise }$
    \smallskip
    \end{tabular} & 
    \begin{tabular}{l}
         \noalign{\smallskip}
         $y : T$ $\wedge (y_j,\ldots,y_{j+\len{\Gt{T}}-1})$ \\ 
      % $r:S \wedge \mathsf{tr}(S)$ \\
      $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
      $\wtd z = g(X) \cup \fnb{Q}{\wtd x \setminus \wtd w}$  \\
      $l = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
      $\sigma = \nextn{u_i}$
      \smallskip
    \end{tabular} 
    \\
    \hline 
    % $\Dbrecpi{k}{\tilde x}{\binp{u_i}{y}{Q}}^d_g$
    $\binp{n_i}{y}{Q}$
    &
    \begin{tabular}{l}
      \noalign{\smallskip}
       $\{\binp{n_l}{\wtd y} 
      \propoutrec{k+1}{\wtd z\rho}
      \recp{X}\binp{\prop^r_k}{\wtd x}
        \binp{n_l}{\wtd y} 
        \propoutrec{k+1}{\wtd z}
        \rvar{X}
       \Par$ 
      %  \\
      $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$ $\text{ if } \rvardepth{Q} = \recdep$
      \\
      \hdashline 
      \noalign{\smallskip}
      $N \cup \{\recp{X}\binp{\prop^r_k}{\widetilde x}
        \binp{n_l}{\widetilde y} 
        \propoutrec{k+1}{\wtd z}
        \rvar{X}
       \Par$ 
      %  \\
      $R : R \in \Dbrecpi{k+1}{\tilde z, \rho}{Q\sigma}^d_g\}$
      \\
      % \hdashline 
      % \noalign{\smallskip}
      $N = 
      \begin{cases} 
        \{\propoutrec{k+1}{\wtd z\rho}
      \recp{X}\binp{\prop^r_k}{\wtd x}
        \binp{n_l}{\wtd y} 
        \propoutrec{k+1}{\wtd z}
        \rvar{X}
       \Par
      \Brecpi{k+1}{\tilde z}{Q\sigma}_g \} & \text{ if } \rvardepth{Q} = \recdep + 1 \\
      \es & \text{ otherwise }
      \end{cases}
      $
      \smallskip 
    \end{tabular} & 
    \begin{tabular}{l}
         \noalign{\smallskip}
      % $r:S \wedge \mathsf{tr}(S)$ \\
      $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
      $\wtd z = g(X) \cup \fnb{Q}{\wtd x \wtd y \setminus \wtd w}$  \\
      $l = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
      $\sigma = \nextn{u_i} \cdot \subst{y_1}{y}$
      % $\wtd z = \fnb{Q}{\wtd x \wtd y}$  
      \smallskip
    \end{tabular} 
    \\
    \hline
    % $\Dbrecpi{k}{\tilde x,\rho}{Q_1 \Par Q_2}^d_g$
    $Q_1 \Par Q_2$
    & 
    \begin{tabular}{l}
      \noalign{\smallskip}
      $ N \cup \{\recp{X}\proprinpk{r}{k}{\wtd x}
      (\proproutk{r}{k+1}{\wtd y_1}\rvar{X}
      \Par \apropoutrecsh{k+\degree+1}{\wtd y_2}) 
       \Par$ 
      %  \\
      $R_1 \Par R_2 :$  \\
      $R_1 \in \Dbrecpi{k+1}{\tilde y_1, \rho}{Q_1}^d_{g_1}, 
      R_2 \in \Dbrecpi{k+\degree+1}{\tilde y_2, \rho}{Q_2}^d_{g_2}\}$ 
      % $\cup$ $N$
      \\
      \hdashline 
      \noalign{\smallskip}
      $ N = 
      \begin{cases} 
     \{\proproutk{r}{k+1}{\wtd y_1\rho}
      \recp{X}\proprinpk{r}{k}{\wtd x} (\proproutk{r}{k+1}{\wtd y_1}\rvar{X}
      \Par 
      \apropoutrecsh{k+\degree+1}{\wtd y_2})
       \Par
      %  \\
      \\ \Brecpi{k+1}{\tilde y_1}{Q_1}_{g_1} \Par 
      \Brecpi{k+\degree+1}{\tilde y_2}{Q_2}_{g_2}\} & \text{ if } \rvardepth{Q_1} = \recdep \\
      \es & \text{ otherwise }
      \end{cases}
      $
      \smallskip 
    \smallskip
    \end{tabular} & 
    \begin{tabular}{l}
           \noalign{\smallskip}
           $\recpx{Q_1}$ \\
           $\wtd y_1  = g(X) \cup \fnb{Q_1}{\wtd x}$ \\
           $\wtd y_2  =  \fnb{Q_2}{\wtd x}$ \\
          %  $i \in \{1,2\}.$ \\
          %  $\quad \wtd y_i' = \linecondit{\recpx{Q_i}}{g(X)}{\epsilon}$ \\
          %  $\quad g_i = \linecondit{\recpx{Q_i}}{g_i}{\epsilon}$ \\
          %  $\quad \wtd y_i  = \wtd y_i' \cup \fnb{Q_i}{\wtd x}$ \\
           $\degree = \lenHOopt{Q_1}$
      \smallskip
    \end{tabular} 
    \\
    \hline
    % $\Dbrecpi{k}{\tilde x, \rho}{\news{s:C}{Q}}^d_g$ & 
    $\news{s:C}{Q}$ &
    \begin{tabular}{l}
      \noalign{\smallskip}
      $N \cup \{\recp{X}\news{\widetilde{s}:\Gt{C}}\propinp{k}{\wtd x}\propout{k+1}{\wtd z}X$
      $\Par$
      $R : R \in \Dbrecpi{k+1}{\tilde z, \rho}{Q \sigma }^d_g \}$
      \\
      \hdashline 
      \noalign{\smallskip}
      $R = \propout{k+1}{\wtd z\rho}
      \recp{X}\news{\wtd{s}:\Gt{C}}\propinp{k}{\wtd x}\propout{k+1}{\wtd z}X$ \\
      $ N = 
      \begin{cases}
      \{\news{\wtd{s}:\Gt{C}}R
      \Par
      \Brecpi{k+1}{\tilde z}{Q\sigma}_g\} &  \text{ if } \rvardepth{Q_1} = \recdep \\
      \es & \text{ otherwise }
      \end{cases}
      $
    \smallskip
    \end{tabular} & 
    \begin{tabular}{l}
      \noalign{\smallskip}
        %  $\mathsf{tr}(\trec{t}{S})$ \\
         $\widetilde{s} = (s_1,\ldots,s_{\len{\Gt{S}}})$ \\
         $\widetilde {\dual{s}} =  (\dual{s_1},\ldots,\dual{s_{\len{\Gt{S}}}})$ \\
         $\wtd n =
          \linecondit{\lin{s}}{\wtd n}{\epsilon}$ \\
    %        $\widetilde {\dual{s}} = \begin{cases}
    %         (\dual{s_1},\ldots,\dual{s_{\len{\Gt{S}}}}) & \text{if} \ C = S \\
    %         \epsilon & \text{if} \ C = \chtype{U}
    % \end{cases}
    % $\\
        %  $\widetilde {\dual{s}} = (\dual{s_1},\ldots,\dual{s_{\len{\Rtopt{S}}}})$ \\
         $\wtd z = \wtd x, \wtd s, \wtd n$ \\
         $\sigma = \subst{s_1 \dual{s_1}}{s \dual{s}} $
      \smallskip
    \end{tabular} 
    \\
    \hline
    % $\Brecpi{k}{\tilde x}{X}_g$ 
    $X$
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $\inact$
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    
    \\ 
        \rowcolor{gray!25}
        \hline
        $P$ &
          \multicolumn{2}{l|}{
        \begin{tabular}{l}
          \noalign{\smallskip}
          $\Dbrecpi{k}{\tilde x, \rho}{P}^d_g$ $\text{ when } g = \es$
          \smallskip
        \end{tabular}
      } 
       \\
        \hline
               %%%%%%
      %% =======================
      %% =======================
      %%%%%%
      $\bout{n_i}{y_j}{Q}$
      &  
      \begin{tabular}{l}
      \noalign{\smallskip}
      $ \{
      \bout{n_{\mstindex}}{\wtd y\rho} \apropoutrecsh{k+1}{\wtd z\rho} \Par  
      \recp{X}\propinprecsh{k}{\wtd x}
      (\bout{n_{\mstindex}}{\wtd y} \apropoutrecsh{k+1}{\wtd z}
      \Par \rvar{X}) 
     \Par$
    $\Brecpi{k+1}{\tilde z}{Q\sigma}_g \}$
      \smallskip
      \end{tabular}
      & 
      \begin{tabular}{l}
             \noalign{\smallskip}
            %  $\wtd x = g(X)$
          \smallskip
      \end{tabular} 
    \\ \hline     
    $\binp{n_i}{y}{Q}$
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $
    \{\binp{n_{\mstindex}}{\wtd y} \apropoutrecsh{k+1}{\wtd z\rho}  \Par 
    \recp{X}\propinprecsh{k}{\wtd x}
    (\binp{n_{\mstindex}}{\wtd y} 
    \apropoutrecsh{k+1}{\wtd z} \Par \rvar{X}) 
    \Par$ 
    %  \\
    $\Brecpi{k+1}{\tilde z}{Q\sigma}_g\}$ 
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    \\ \hline    
    $Q_1 \Par Q_2$
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $
    \{\apropoutrecsh{k+1}{\wtd y_1\rho}
    \Par \apropoutrecsh{k+\degree+1}{\wtd y_2\rho} \Par 
    \recp{X}\proprinpk{r}{k}{\wtd x}(\apropoutrecsh{k+1}{\wtd y_1}
    \Par \apropoutrecsh{k+\degree+1}{\wtd y_2} \Par \rvar{X})
    \Par$ 
    \\
    $\Brecpi{k+1}{\tilde y_1}{Q_1}_{g_1} \Par 
    \Brecpi{k+\degree+1}{\tilde y_2}{Q_2}_{g_2}\}$ 
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    \\ \hline    
    $\news{s:C}{Q}$ 
    &  
    \begin{tabular}{l}
    \noalign{\smallskip}
    $
    \{\apropoutrecsh{k+1}{\wtd z\rho} \Par 
    \recp{X}\news{\wtd{s}:\Gt{C}}
    \propinp{k}{\wtd x}(\apropoutrecsh{k+1}{\wtd z} \Par X)$
    $\Par$
    $\Brecpi{k+1}{\tilde z}{Q}_g\}$
    \smallskip
    \end{tabular}
    & 
    \begin{tabular}{l}
         \noalign{\smallskip}
        %  $\wtd x = g(X)$
      \smallskip
    \end{tabular} 
    \\ \hline    
      \end{tabular}
    %   \caption{The extension of $\Cbpi{\tilde u}{\tilde x}{P}$ 
    %   and definition of $\Dbrecpi{k}{\tilde x, \rho}{P}^d_g$
    %   (recursion extension). Side conditions for 
    %   last four rows ($g = \es$) are the same as for corresponding 
    %   cases when $g \not = \es$. \label{pi:t:tablecd-rec}}
    %   \vspace{-2mm}
    %   \end{table}
    % \end{figure*}

==> sources/minimality-result-full.tex <==

\section{Extension with Labeled Choices}
% \subsection{Minimality Result}

% \begin{align*}
%   \tau := \lto{\wtd \tau} \bnfbar \lti{\wtd \tau} 
%   \bnfbar \ltab{\wtd \tau} \bnfbar \ltend 
%   \bnfbar \ltc{\wtd \tau}
%   \bnfbar \ltbra  \bnfbar \texttt{Unit}
% \end{align*}

% \begin{align*}
%   P,Q, &:= \bout{x}{\tilde v}P \bnfbar 
%   \binp{x}{\tilde y}P \bnfbar \news{v}P
%   \bnfbar \inact \bnfbar P \Par Q 
%   \bnfbar \ltcase{v}{l_i}{x_i}{P_i}{i \in I} 
%   \\
%     v &:= x  \bnfbar \star \bnfbar l\_v
% \end{align*}

% \input{type_system_lt.tex}

% \begin{newaddenv}

%In this section, we address three intertwined aspects: (i)~the extension of our approach to support constructs for \emph{labeled choice} (branching and selection); (ii)~a detailed comparison with the CPS approach (Kobayashi, Dardha et al.) to deconstruct session-typed processes into linearly-typed processes; (iii)~a discussion on the notion of minimality enforced by \msts. 

%\subsection{Labelled Choices}
\begin{newaddenv}
In session-based concurrency, labeled choices are implemented via branching and selection constructs, denoted $\bbra{u_i}{l_j : P_j}_{j \in I}$ and $\bsel{u_i}{l_j}Q$, respectively. Intuitively, a branching construct specifies the offer of a finite number of alternative behaviors ($P_1, P_2, \ldots$), whereas a selection construct signals the choice of one of them. 
Put differently, branching and selection implement deterministic choices via the input and output of labels; 
they come with dedicated session types, denoted 
$\btbra{l_i : S_i}_{i \in I}$  and $\btsel{l_i : S_i}_{i \in I}$, respectively, for some finite index set $I$.
    
Here we illustrate how our decomposition strategy can be extended to account for labeled choice (and their types).
This entails the extension of the type decomposition function $\Gtopt{\cdot}$ (\Cref{pi:def:typesdecomp}) and of the breakdown function $\Bopt{k}{\tilde x}{P}$ (\Cref{pi:t:bdowncorec}); this latter extension will be denoted  $\Boptsb{k}{\tilde x}{\cdot}$.
For simplicity, we concentrate on the case of \emph{finite} processes,  without recursion / recursive session types. %; this will also facilitate comparisons with the CPS approach. 
We base our presentation on the corresponding breakdown for the case of the higher-order calculus \HO, as presented in~\cite{DBLP:journals/corr/abs-2301-05301}.

  Notice that in a branching type  $\btbra{l_i:S_i}_{i \in I}$ each
   $S_i$ can be different. 
   To uniformly handle these differences, we break down branching and selection types  as follows: 
\end{newaddenv}
\begin{definition}[Decomposing Types: Labeled Choices]
  \label{pi:d:typessb}
  We extend the type decomposition function $\Gtopt{\cdot}$ (\Cref{pi:def:typesdecomp}) as follows:
  \begin{align*}
    \Gtopt{\btbra{l_i : S_i}_{i \in I}} &= 
    \btbra{l_i :\, \btinp{\Gtopt{S_i}}\tinact}_{i \in I}  
    \\
    \Gtopt{\btsel{l_i : S_i}_{i \in I}} &=  
    \btsel{l_i :\, \btout{\Gtopt{S_i}}\tinact}_{i \in I} 
  \end{align*} 
\end{definition}
\begin{newaddenv}
  This decomposition follows the intuition that branching and selection correspond to the input and output of labels, respectively. 
  For example, in the case of branching, once a particular branch $l_i$ has been selected, we would like to input names on which to provide sessions from the branch $\Gtopt{S_i}$; the corresponding selection process 
  should provide the names for the chosen branch. 
  By binding names of selected branch, we account for the different 
  session types of the branches $S_i$. 

The decomposition of branching and selection processes is defined accordingly: 
\end{newaddenv}

\begin{definition}[Decomposing Processes: Labeled Choice] 
  \label{pi:d:processsb}
  % \begin{align*}
  %   \Bopt{k}{\tilde x}{
  %     \propinp{k}{\tilde x}\bbra{u_i}{l_j : P_j}_{j \in I}}  
  %   &= \bbra{u_i}{l_j : \binp{n_i}{\tilde y}\Bopt{}{}{P_i\subst{y_1}{x_i}}}_{j \in I} \\
  %   \Bopt{}{}{\bsel{x_i}{l_i}Q}  
  %   &= \bsel{x_i}{}
  % \end{align*}
  Given a $k \geq 0$ and a tuple of names $\tilde x$, the decomposition function $\Boptsb{k}{\tilde x}{\cdot}$ is defined as 
    \begin{align*}
      \Boptsb{k}{\tilde x}{
       \bbra{u_i}{l_j : P_j}_{j \in I}}  
      &= 
      \propinp{k}{\tilde x}
      \bbra{u_i}{l_j : \news{\tilde \prop_{j}}\binp{u_i}{\tilde y}\apropout{k+1}{\tilde x \tilde y} \Par 
      \Boptsb{k+1}{\tilde x \tilde y}{P_j\subst{y_1}{u_i}}}_{j \in I} 
      \\
      \Boptsb{k}{\tilde x}{\bsel{u_i}{l_j}Q}  
      &= 
      \propinp{k}{\tilde x}\bsel{u_i}{l_j}
      \news{\tilde u : \Gtopt{S_j}}\bout{u_i}{
        {\tilde{\dual u}}}
        \apropout{k+1}{\tilde x} \Par 
        \Boptsb{k+1}{\tilde x}{Q\subst{s_1}{u_i}}
      % \apropout{k+1}{\tilde x} \Par 
    \end{align*} 
    \noindent where $\widetilde u=(u_{i+1},\ldots,u_{i+\len{\Gtopt{S_j}}})$ 
    and $\widetilde {\dual {u}}=(\dual {u_{i+1}},\ldots,\dual 
    {u_{i+\len{\Gtopt{S_j}}}})$. 
    \begin{newaddenv}
      For the remaining constructs, $\Boptsb{k}{\tilde x}{\cdot}$ corresponds 
      to $\Boptsb{k}{\tilde x}{\cdot}$ (\Cref{pi:t:bdowncorec}). 
    \end{newaddenv} 
  \end{definition}
 % \Boptsb
  \begin{newaddenv}
    We illustrate the workings of $\Boptsb{k}{\tilde x}{\cdot}$ by means of 
    the following example, adapted from~\cite{DBLP:journals/corr/abs-2301-05301}: 
  \end{newaddenv}



\begin{example}
\label{pi:ex:server}
  Consider a mathematical server $Q$ that offers clients two operations: addition and negation of integers. 
  The server uses name $u$ to implement the following session type: 
    \begin{align*}
      S = \btbra{\textsf{add}: 
      \underbrace{\btinp{\textsf{int}} \btinp{\textsf{int}} 
      \btout{\textsf{int}} \tinact}_{S_{\textsf{add}}}
      ~,\ 
      \textsf{neg} : 
      \underbrace{\btinp{\textsf{int}} \btout{\textsf{int}} \tinact}_{S_{\textsf{neg}}} 
      }
    \end{align*}
    This way, the $\textsf{add}$ branch receives two integers and sends
    over their sum;  the $\textsf{neg}$ branch has a single input of an integer followed by an
    output of its negation. 
    
    Let us consider a possible implementation for the server $Q$ and for a client $R$ that {selects} the first branch to add integers 16 and 26:
    \begin{align*}
       Q & \defas \bbra{u}{\textsf{add} : 
      \underbrace{\binp{u}{a}\binp{u}{b}\boutt{u}{a+b} }_{Q_{\textsf{add}}},\ 
      \textsf{neg} : 
      \underbrace{\binp{u}{a}\boutt{u}{-a}}_{Q_{\textsf{neg}}}} 
      \\
      R & \defas \bsel{\dual{u}}{\textsf{add}} 
      \bout{\dual {u}}{\mathbf{16}} \bout{\dual u}{\mathbf{26}} \binpt{\dual u}{r} 
      \end{align*}

      \noindent 
      The composed process $P \defas \news{u}(Q \Par R)$ can reduce as follows: 
  \begin{align*}
    P & ~\red~ 
    \news{u} 
    (\binp{u}{a}\binp{u}{b}\about{u}{a+b} \Par 
    \bout{\dual {u}}{\mathbf{16}} \bout{\dual u}{\mathbf{26}} \binpt{\dual u}{r} ) \\
    & ~\red^2~ 
    \news{u} (\about{u}{\mathbf{16+26}}  \Par \binpt{\dual u}{r} )
    = P'
  \end{align*}
First, \newadd{following~\Cref{pi:d:typessb}}, the decomposition  of $S$ is the minimal session type $M$, defined as follows:
\begin{align*}
  M = \Gtopt{S} =
      \btbra{
        &\textsf{add}:
      \btinpt{{\big(\btinpt{\textsf{int}}, \btinpt{\textsf{int}}, \btoutt{\textsf{int}}  \big)}},
      \\ 
      &\textsf{neg}:
      \btinpt{{\big(\btinpt{\textsf{int}}, \btoutt{\textsf{int}} \big)}}} 
\end{align*}

Let us now discuss the decomposition of $P$. 
\newadd{Using~\Cref{pi:d:processsb}} we have: 
  \begin{align}
    D = \news{\prop_1, \ldots, \prop_7} (\propinp{1}{} \propout{2}{} \propoutt{3}{} 
    \Par 
    \Boptsb{2}{\epsilon}{Q\sigma_2} \Par 
    \Boptsb{3}{\epsilon}{R\sigma_2} )
    \label{pi:ex:dec}
  \end{align}
  \noindent where $\sigma_2=\subst{u_1\dual{u_1}}{u\dual u}$. 
  The breakdown of process $Q$  is as follows: 
\begin{align*}
  \Boptsb{2}{\epsilon}{Q\sigma_2} = 
  \propinp{2}{}
  \bbra{u_1}{
    &\textsf{add} : \news{\tilde \prop_{j}}
    \binp{u_1}{y_1, y_2, y_3}\apropout{1}{y_1,y_2,y_3} \Par 
  \Boptsb{1}{y_1, y_2, y_3}{Q_{\mathsf{add}}\subst{y_1}{u_1}}, 
  \\ 
  &\textsf{neg}: 
  \news{\tilde \prop_{j}}\binp{u_1}{\tilde y}\apropout{1}{y_1, y_2} \Par 
  \Boptsb{1}{\y_1, y_2}{Q_{\mathsf{neg}}\subst{y_1}{u_1}}
  }
\end{align*}
\noindent where 
\begin{align*}
  \Boptsb{1}{y_1, y_2, y_3}{Q_{\mathsf{add}}\subst{y_1}{u_1}} &= 
  \apropinp{1}{y_1, y_2, y_3} \Par \propinp{1}{y_1, y_2, y_3}
  \binp{y_1}{a}\apropout{2}{y_2,y_3,a} \Par 
  \\
  & \qquad 
  \propinp{2}{y_2,y_3,a}\binp{y_2}{b}\apropout{3}{y_3,a,b} \Par 
  \propinp{3}{y_3,a,b}\bout{y_3}{a+b}\apropinp{4}{} \Par 
  \apropinp{4}{} 
  \\ 
  \Boptsb{1}{y_1, y_2}{Q_{\mathsf{neg}}\subst{y_1}{u_1}} &= 
  \apropinp{1}{y_1, y_2} \Par \propinp{1}{y_1, y_2}
  \binp{y_1}{a}\apropout{2}{y_2,a} \Par 
  \\
  & \qquad 
  \propinp{2}{y_2,a}\bout{y_2}{-a}\apropout{3}{} \Par 
  % \propinp{3}{y_3,a,b}\bout{y_3}{a+b}\apropinp{4}{} \Par 
  \apropinp{3}{} 
\end{align*}
In process $\Boptsb{1}{y_1, y_2, y_3}{Q_{\mathsf{add}}\subst{y_1}{u_1}}$, name $u_1$ implements $M$. 
Following the common trio structure, the first prefix awaits activation on 
$\prop_2$. The next prefix mimics the
branching action of $Q$ on $u_1$. 
Then, each branch consists of the input of 
the breakdown of the continuation of channel $u$, that is 
$y_1,y_2,y_3$. This input does not have a counterpart in $Q$; 
it is meant to synchronize with process $\Boptsb{3}{\epsilon}{R\sigma_2}$, 
the breakdown of the corresponding selection process. 


In the bodies of the abstractions we break down $Q_{\textsf{add}}$ and $Q_{\textsf{neg}}$, but not before adjusting the names on which the broken down processes provide the sessions.
For this,  we substitute $u$ with $y_1$ in both processes, ensuring that the broken down names are bound by the input.
By binding decomposed names in the input we account for different 
session types of the original name in branches, while preserving typability: 
this way the decomposition of different branches can use (i)~the same names
but typed with different minimal types and (ii)~a different number of names, as it is the
case in this example. 



The decomposition of the client process $R$, which implements the selection, 
is as follows: 
\begin{align*}
  \Boptsb{3}{\epsilon}{R\sigma_2} &= 
  \propinp{3}{\epsilon}\bsel{\dual u_1}{\mathsf{add}}
  \news{u_2,u_3, u_4}\bout{\dual u_1}{ u_2,  u_3,  u_4}
  \apropout{4}{} \Par  \Boptsb{4}{\epsilon}{\bout{\dual u_2}{\mathbf{16}}\bout{\dual u_2}{\mathbf{26}} \binpt{\dual u_2}{r}}
  % \\
  % & 
  % \propinp{4}{} ... 
\end{align*}
\noindent where 
\begin{align*}
  \Boptsb{4}{\epsilon}{\bout{\dual u_2}{\mathbf{16}}\bout{\dual u_2}{\mathbf{26}} \binpt{\dual u_2}{r}} = 
  \propinp{4}{}\bout{\dual u_2}{\mathbf{16}}\apropout{5}{} \Par 
  \propinp{5}{}\bout{\dual u_3}{\mathbf{26}}\apropout{6}{} \Par 
  \propinp{6}{}\binp{\dual u_4}{r}\apropout{7}{} \Par 
  \apropinp{7}{} 
\end{align*}

After receiving the context on $\prop_3$ (empty in this case), the selection action on $u_1$ is mimicked; then, the breakdown of 
channel continuation, $ u_2,  u_3,  u_4$, that are locally bound, 
are sent along name $u_1$. 
The intention is to use these names to connect 
the selected branch and the continuation of a selection process: the subprocess encapsulated in the branch  will use
$(u_2,  u_3,  u_4)$, while the dual names $(\dual u_2, \dual u_3, \dual
u_4)$ are present in the breakdown of the continuation. 


Let us briefly examine the reductions of the decomposed process $D$ in (\ref{pi:ex:dec}).
First, $\prop_1$, $\prop_2$, and $\prop_3$ will synchronize. 
We have $D \red^4 D_1$, where
\begin{align*}
  D_1 = \news{\prop_4 \ldots \prop_7} 
  &\news{u_1} \big(
    \bbra{u_1}{
      \textsf{add} : \news{\tilde \prop_{j}}
      \binp{u_1}{y_1, y_2, y_3}\apropout{1}{\tilde y} \Par 
    \Boptsb{1}{y_1, y_2, y_3}{Q_{\mathsf{add}}\subst{y_1}{u_1}}, 
    \\ 
    & \qquad \qquad \qquad 
    \textsf{neg}: 
    \news{\tilde \prop_{j}}\binp{u_1}{\tilde y}\apropout{1}{y_1, y_2} \Par 
    \Boptsb{1}{\y_1, y_2}{Q_{\mathsf{neg}}\subst{y_1}{u_1}}
    }
  \\ 
    & \qquad \quad   \Par
    \bsel{\dual u_1}{\mathsf{add}}
    \news{u_2,u_3, u_4}\bout{\dual u_1}{ u_2,  u_3,  u_4}
    \apropout{4}{} \Par  \Boptsb{4}{\epsilon}{\bout{\dual u_2}{\mathbf{16}}\bout{\dual u_2}{\mathbf{26}} \binpt{\dual u_2}{r}}
    \big )
    \end{align*} 
 
    \noindent 
    Now, the processes chooses the label \textsf{add} 
    on $u_1$. The process $D_1$ will reduce further as 
    $D_1 \red D_2 \red^2 D_3$, where: 
    \begin{align*}
      D_2 =~ & \news{\tilde \prop_{j}}
      \binp{u_1}{y_1, y_2, y_3}\apropout{1}{\tilde y} \Par 
    \Boptsb{1}{y_1, y_2, y_3}{Q_{\mathsf{add}}\subst{y_1}{u_1}}
    \Par 
    \\ 
    & 
    \qquad  \news{u_2,u_3, u_4}\bout{\dual u_1}{ u_2,  u_3,  u_4}
    \apropout{4}{} \Par  \Boptsb{4}{\epsilon}{\bout{\dual u_2}{\mathbf{16}}\bout{\dual u_2}{\mathbf{26}} \binpt{\dual u_2}{r}} 
    \\
    D_3 =~ &
    \binp{\dual u_2}{a}\apropout{2}{ u_3, u_4,a} \Par  \propinp{2}{y_2, y_3,a}\binp{ y_2}{b}\apropout{3}{y_3,a,b} \Par 
    \\
    & \qquad  
    \propinp{3}{y_3,a,b}\bout{ y_3}{a+b}\apropout{4}{} \Par 
    \\ 
    & \qquad  
  \propinp{4}{} \bout{\dual u_2}{\mathbf{16}}\apropout{5}{} \Par 
  \propinp{5}{}\bout{\dual u_3}{\mathbf{26}}\apropout{6}{} \Par 
  \propinp{6}{}\binp{\dual u_4}{r}\apropout{7}{} \Par 
  \apropinp{7}{} 
    \end{align*}
Now, process $D_3$ can mimic the original 
transmission of the integer $16$ on channel $u_2$ as follows: 
\begin{align*}
  D_3 &\red 
  \apropout{2}{\dual u_3, \dual u_4, \mathbf{16}} \Par \propinp{2}{y_2, y_3,a}\binp{y_2}{b}\apropout{3}{y_3,a,b} \Par 
    \\
    & \qquad 
    \propinp{3}{y_3,a,b}\bout{y_3}{a+b}\apropout{4}{} \Par 
    \apropinp{4}{} 
    \Par 
    \\ 
    & \qquad 
  \apropout{5}{} \Par 
  \propinp{5}{}\bout{\dual u_3}{\mathbf{26}}\apropout{6}{} \Par 
  \propinp{6}{}\binp{\dual u_4}{r}\apropout{7}{} \Par 
  \apropinp{7}{} = D_4 
\end{align*}

Finally, $D_4$ reduces to $D_5$ as follows: 
\begin{align*}
  D_4 &\red^5 
  \bout{\dual u_4}{a+b}\apropout{4}{} \Par 
    \apropinp{4}{} 
    \Par 
    % \\ 
    % & \quad 
 \binp{ u_4}{r}\apropout{7}{} \Par 
  \apropinp{7}{} = D_5 
\end{align*}
This way, the steps from $D$ to $D_5$ correctly simulate the synchronizations of the process $P'$. 
\end{example}

  \subsection{Comparison with the CPS Approach}
  As mentioned in the Introduction, one advantage of investigating our approach to decomposition and \msts for \sessp is that it allows us to contrast it with the CPS approach that represents session-typed processes using linearly-typed processes, as proposed by Kobayashi and studied by Dardha et al~\cite{DBLP:journals/iandc/DardhaGS17}. In this sub-section we compare the two approaches, and establish formal connections between the two. In fact, we prove that \msts correspond to   linear $\pi$ types. 
  This result shows that \msts are indeed minimal. 

To substantiate our comparisons, we first introduce some selected notions for the linearly-typed $\pi$-calculus considered by Dardha et al.~(the reader is referred to~\cite{DBLP:journals/iandc/DardhaGS17} for a thorough description and technical results).
    \begin{definition}[Linearly-Typed $\pi$-calculus Processes~\cite{DBLP:journals/iandc/DardhaGS17}] 
    The syntax of processes $P, Q, \ldots$, values $v, v', \ldots$,  and of linear types $\tau, \tau', \ldots$ is as follows:
\begin{align*}
 \text{Processes~~}   P,Q, &:= \bout{x}{\tilde v}P \bnfbar 
  \binp{x}{\tilde y}P \bnfbar \news{v}P
  \bnfbar \inact \bnfbar P \Par Q 
  \bnfbar \ltcase{v}{l_i}{x_i}{P_i}{i \in I} 
  \\
   \text{Values~~}   v, v' &:= x  \bnfbar \star \bnfbar l\_v
   \\
    \text{Types~~}   \tau, \tau' & := \lto{\wtd \tau} \bnfbar \lti{\wtd \tau} 
  \bnfbar \ltab{\wtd \tau} \bnfbar \ltend 
  \bnfbar \ltc{\wtd \tau}
  \bnfbar \ltbra  \bnfbar \texttt{Unit}
\end{align*}
\end{definition} 
 
At the level of processes, the main difference with respect to the syntax of \HOp in \Cref{top:fig:syntax} is the case construct `$\ltcase{v}{l_i}{x_i}{P_i}{i \in I}$', which together with the variant value `$l\_v$' implement a form of deterministic choice. This choice is decoupled from a synchronization: indeed, the process $\ltcase{l_j\_v}{l_i}{x_i}{P_i}{i \in I}$ (with $j \in I$) autonomously reduces to $P_j\subst{v}{x_j}$.
	At the level of types, the grammar above first defines  types 
	$\lto{\wtd \tau}$, $ \lti{\wtd \tau}$, and  
$\ltab{\wtd \tau}$ 
	for the linear exchange messages of type $\widetilde{\tau}$: output, input, and both output and input, respectively. Then, the types $\ltend$ and $\ltc{\wtd \tau}$ are assigned to channels without any capabilities and with arbitrary capabilities, respectively. Finally, we have the variant type $\ltbra$ associated to the case construct  and the unit type $\texttt{Unit}$.
	
The typing rules for processes, given in~\Cref{top:fig:typeslinear}, should be self-explanatory; we omit definitions for contexts and their operations, which follow expected intuitions. The type system ensures the type preservation property (subject reduction).

\input{type_system_lt.tex}
	
As its name suggests, the key idea of the CPS approach is to represent  one message exchange using \emph{two} channels: one is the message itself, the other is a continuation for the next sequential action in the session. Rather than giving a formal definition, we illustrate this approach  by example.  
	
    \newcommand{\contc}{c}
  \begin{example}[The CPS Approach, By Example]
  Consider the session type $S$ and the processes $Q$ and $R$ from \Cref{pi:ex:server}. Under the CPS approach, the session type $S$ is represented as linear types as follows:
%    \begin{align*}
%      S = \btbra{\textsf{add}: 
%      \underbrace{\btinp{\textsf{int}} \btinp{\textsf{int}} 
%      \btout{\textsf{int}} \tinact}_{S_{\textsf{add}}}
%      ~,\ 
%      \textsf{neg} : 
%      \underbrace{\btinp{\textsf{int}} \btout{\textsf{int}} \tinact}_{S_{\textsf{neg}}} 
%      }
%    \end{align*}
    \begin{align*}
      \ltenc{S} &=
      \lti{\ltsel{\textsf{add}}{\ltenc{S_{\textsf{add}}},\ 
      \textsf{neg}: {\ltenc{S_{\textsf{neg}}}}}{}} 
      \\
      \ltenc{S_{\textsf{add}}} &= \lti{\textsf{int}, \lti{\textsf{int}, 
      \lto{\textsf{int}, \ltend}}}
      \\
      \ltenc{S_{\textsf{neg}}} &= \lti{\textsf{int}, \lto{\textsf{int},  \ltend}}
    \end{align*}
 This way, sequentiality in $S$ arises in  $\ltenc{S}$ as nesting of pairs---the later that an action appears in a session type, the deeper it will appear in the corresponding linear type.
 Accordingly, the encoding of $Q$ and $R$ as linear processes is as given below; the translation relies on a parameter that records continuations:
   \begin{align*}
    \ltenc{P}_{\emptyset} &= \news{u}\ltenc{Q \Par R}_{\emptyset} = 
    \news{u}\ltenc{Q}_{\emptyset} \Par \ltenc{R}_{\emptyset} \\
   \ltenc{Q}_{\emptyset} &=  
  %  \binp{u}{y}\ltcase{y}{l_i}{c}{\ltenc{P_i}}{}  
   \binp{u}{y}\ltcasep{y}{\textsf{add}\_c_1~\triangleright~\ltenc{Q_{\textsf{add}}}_{u \mapsto \contc_1},\ 
   \textsf{neg}\_c~\triangleright~\ltenc{Q_{\textsf{neg}}}_{u \mapsto \contc_1}} 
   \\
   \ltenc{Q_{\textsf{add}}}_{u \mapsto \contc_1} &= 
   \binp{\contc_1}{a, \contc_2}\binp{\contc_2}{b,\contc_3}\news{\contc_4}
   \bout{\contc_3}{a+b, \contc_4}\inact
   \\
   \ltenc{Q_{\textsf{neg}}}_{u \mapsto \contc_1} &= 
   \binp{\contc_1}{a, \contc_2}\news{\contc_3}
   \bout{\contc_2}{-a, \contc_3}\inact 
   \\ 
   \ltenc{R}_{\emptyset} &= 
   \news{\contc_1}\bout{u}{\textsf{add}\_\contc_1} 
   \news{\contc_2}\bout{\contc_1}{\textbf{16}, \contc_2}
   \news{\contc_3}\bout{\contc_2}{\textbf{26}, \contc_3}
   \binp{\contc_3}{r}\inact
   \end{align*}
   Observe how the branching construct in $Q$ is encoded using two constructs: an input prefix immediately followed by a case construct. 
   Also, notice the use of restrictions $\news{\contc_i}$ (with $i \in \{1,2,3\}$) in the encoding of output prefixes: this is crucial to avoid interferences and ensure that session communications are mimicked in the intended order.
  \end{example} 
  
  




% \end{newaddenv}

% \begin{align*}
%   \ltmap
% \end{align*}
% \todo[inline]{\msts}
\paragraph{Comparison}
Based on the above, we extract two sources of comparison between our decompositions into \msts and the CPS approach:
\begin{enumerate}
	\item At the level of types, there is a tight correspondence  between \msts and the class of linear types needed to encode session types in the CPS approach. 
	\item At the level of processes, both approaches use the same principle, namely to generate fresh names to encode the sequential structure of sessions. While the CPS approach follows a \emph{dynamic} discipline to generate such names (i.e., they are generated by the encoding of output-like actions), the decomposition approach follows a \emph{static discipline}, i.e., fresh names are generated based on the length of the source session types. 
\end{enumerate}

\paragraph*{Mutual encodings of \msts processes and linearly 
typed $\pi$-processes}
We provide the translation of \msts processes into linearly typed $\pi$ processes, 
denoted by $\ltenc{\text{-}}$, in
\Cref{pi:f:msttolst}. Importantly for our minimality reasoning, 
this translation is the simplification of the one given in~\cite{DBLP:journals/iandc/DardhaGS17} 
as we do not have to consider channel continuations 
when translating a process typed with \msts. 
This can be explicitly seen by the lack of parameter $f$  
 which is used in the original encoding to name a channel continuation. 
% as \msts does not have it. 
% allowed by taking \msts 
\begin{figure}[t]
  \begin{mdframed}[style=alttight]
        \begin{align*}
        C  & \bnfis		M  \bnfbar  {\chtype{M}}
    % \\
        % M  &\bnfis 	\tinact  \bnfbar  \btout{\widetilde{C}} \tinact \bnfbar \btinp{\widetilde{C}} \tinact
        \\ 
        \mugamma  &\bnfis \tinact \\ %\bnfbar \vart{t}  \\
      M  &\bnfis 	\mugamma  \bnfbar  \btout{\widetilde{C}} \mugamma \bnfbar \btinp{\widetilde{C}} \mugamma %\bnfbar \trec{t}{M }		
      \bnfbar \btbra{l_i : \btout{\wtd M_i}{\tinact}}_{i \in I} 
      \bnfbar \btsel{l_i : \btinp{\wtd M_i}{\tinact}}_{i \in I}
      % \\
      % M &\bnfis ...  
      \end{align*}
      \end{mdframed}
      \caption[Minimal Session Types for \sessp.]{Minimal Session Types for \sessp (finite fragment, modifies~\Cref{pi:d:mtypesi})}\label{pi:f:mtypesi2}
      % \vspace{-3mm}
   \end{figure}

   \begin{figure}[!t]
    \begin{mdframed}%[style=alttight]
      % \begin{tabular}{ll}
      % $\ltenc{\bbra{x}{l_i:P_i}_{i \in I}}_{f} 
      % \defeq 
      % \binp{x}{y}\ltcase{y}{l_i}{c}{\ltenc{P_i}_{f, \{x \mapsto c\}}}{i \in I}$ 
      % & 
      % $\ltenc{ \btbra{l_i : \btinp{\tilde M_i}{\tinact}}_{i \in I}} \defeq \lto{\lttcase{l_i}{\ltenc{\tilde M_i}}{i \in I}}$
      \noi{\bf Terms:}
    \begin{align*}
      % \ltenc{x} &\defeq f_x \\ 
      % \ltenc{\star}_f & \defeq \star \\ 
      \ltenc{\inact} &\defeq \inact \\ 
      \ltenc{\bout{x_i}{\wtd v}P} &\defeq \bout{x_i}{{\wtd v}}\ltenc{P}_{} \\ 
      \ltenc{\binp{x_i}{\wtd y}P} &\defeq \binp{x_i}{\wtd y}\ltenc{P}_{} \\ 
      \ltenc{\bsel{x}{l_j}\news{c}\bout{x}{\dual c}{P}} 
      &\defeq \news{c}\bout{f_x}{l_j\_c}\ltenc{P} \\
      % \ltenc{\bsel{x}{l_j}{P}}_f &\defeq \news{c}\bout{f_x}{l_j\_c}\ltenc{P}_{f,\{x \mapsto c\}} \\
      % \ltenc{\bbra{x}{l_i:P_i}_{i \in I}}_{f} 
      % &\defeq 
      % \binp{x}{y}\ltcase{y}{l_i}{c}{\ltenc{P_i}_{f, \{x \mapsto c\}}}{i \in I} \\
      \ltenc{\bbra{x}{l_i:\binp{x}{c}P_i}_{i \in I}}
      &\defeq 
      \binp{x}{y}\ltcase{y}{l_i}{c}{\ltenc{P_i}}{i \in I} \\
      \ltenc{P \Par Q} &\defeq \ltenc{P}_f \Par \ltenc{Q} \\ 
      \ltenc{\news{x}P} &\defeq \news{c}\ltenc{P} 
      % &~~~{\hbox to \textwidth{\leaders\hbox to 3pt{\hss . \hss}\hfil}}
      % \\
    % \end{align*}
    % %  \\ 
    %     ~~~{\hbox to \textwidth{\leaders\hbox to 3pt{\hss . \hss}\hfil}}
    %     \hspace*{-5cm}
    % \begin{align*}
      \\[1mm]
\noalign{\bf Types:}
      \ltenc{\chtype{M}} &\defeq \ltc{\ltenc{M}} 
    \\
      \ltenc{\tinact}{} &\defeq \ltend \\ 
      \ltenc{\btout{\tilde M}\tinact} &\defeq \lto{\ltenc{\tilde M}} \\
      \ltenc{\btinp{\tilde M}\tinact} &\defeq \lti{\ltenc{\tilde M}} \\
      \ltenc{\btsel{l_i : \btout{\tilde M_i}{\tinact}}_{i \in I}} &\defeq \lto{\lttcase{l_i}{\ltenc{\tilde M_i}}{i \in I}} \\
      \ltenc{ \btbra{l_i : \btinp{\tilde M_i}{\tinact}}_{i \in I}} &\defeq \lti{\lttcase{l_i}{\ltenc{\tilde M_i}}{i \in I}} 
      % \\
      \\[1mm]
\noalign{\bf Enviroments:}
      \ltenc{\Gamma, x : \chtype{\wtd M}} & \defeq 
  \ltenc{\Gamma}, x : \ltenc{\chtype{\wtd M}} 
  \\
  \ltenc{\Delta, x : M} & \defeq  
  \ltenc{\Delta}, x : \ltenc{M}  
  \\
  \ltenc{\emptyset} & \defeq \varnothing 
    \end{align*}
  % \end{tabular} 
  \end{mdframed}
  \caption{Typed encoding of \msts processes into linearly typed $\pi$ processes.
  \label{pi:f:msttolst}}
   \end{figure}


   \begin{figure}[!t]
    \begin{mdframed}%[style=alttight]
      % \begin{tabular}{ll}
      % $\ltenc{\bbra{x}{l_i:P_i}_{i \in I}}_{f} 
      % \defeq 
      % \binp{x}{y}\ltcase{y}{l_i}{c}{\ltenc{P_i}_{f, \{x \mapsto c\}}}{i \in I}$ 
      % & 
      % $\ltenc{ \btbra{l_i : \btinp{\tilde M_i}{\tinact}}_{i \in I}} \defeq \lto{\lttcase{l_i}{\ltenc{\tilde M_i}}{i \in I}}$
      \noi{\bf Terms:}
    \begin{align*}
      % \ltenc{x} &\defeq f_x \\ 
      % \ltenc{\star}_f & \defeq \star \\ 
      \ltencr{\bout{x_i}{{\wtd v}}{P}}
  &\defeq 
  \bout{x_i}{{\wtd v}}\ltencr{P} \\ 
  \ltencr{\binp{x_i}{{\wtd v}}{P}}
  &\defeq 
  \binp{x_i}{{\wtd v}}\ltencr{P} \\ 
  % \ltenc{\binp{x_i}{\wtd y}P}_f &\defeq \binp{x_i}{\wtd y}\ltenc{P}_{f} \\ 
  \ltencr{\news{c}\bout{f_x}{l_j\_c}{P}} 
  &\defeq
  {\news{c}\bsel{x}{l_j}\bout{x}{c}{P}}
   \\
  % \ltenc{\bsel{x}{l_j}{P}}_f &\defeq \news{c}\bout{f_x}{l_j\_c}\ltenc{P}_{f,\{x \mapsto c\}} \\
  % \ltenc{\bbra{x}{l_i:P_i}_{i \in I}}_{f} 
  % &\defeq 
  % \binp{x}{y}\ltcase{y}{l_i}{c}{\ltenc{P_i}_{f, \{x \mapsto c\}}}{i \in I} \\
  \ltencr{\binp{x}{y}\ltcase{y}{l_i}{c}{{P_i}}{i \in I}} 
  &\defeq 
  {\bbra{x}{l_i:\binp{x}{c}P_i}_{i \in I}}
   \\
  \ltencr{P \Par Q} &\defeq \ltencr{P} \Par \ltencr{Q} \\ 
  \ltencr{\news{x}P} &\defeq \news{x}\ltencr{P}
      % &~~~{\hbox to \textwidth{\leaders\hbox to 3pt{\hss . \hss}\hfil}}
      % \\
    % \end{align*}
    % %  \\ 
    %     ~~~{\hbox to \textwidth{\leaders\hbox to 3pt{\hss . \hss}\hfil}}
    %     \hspace*{-5cm}
    % \begin{align*}
      \\[1mm]
      \noalign{\bf Types:}
      \ltencr{\ltc{\tau}} &\defeq  {\chtype{\ltencr{\tau}}} 
\\
% \ltencr{\ltab{L}}  &\defeq
% \ltencr{\lto{L}}, \ltencr{\lti{L}}
% \\
\ltencr{\ltend} &\defeq \tinact   \\ 
\ltencr{\lto{L}} &\defeq \begin{cases}
  \btsel{l_i : \btout{\ltencr{\tilde \tau}\tinact}}_{i \in I} & \text{ if }  L = \lttcase{l_i}{\ltenc{\tilde \tau}}{i \in I}  \\
  \btout{\ltencr{\tilde \tau}}\tinact  & \text{ otherwise } L = \tilde \tau  
\end{cases}\\
\ltencr{\lti{L}} &\defeq 
\begin{cases}
  \btbra{l_i : \btinp{\ltencr{\tilde \tau}}\tinact}_{i \in I} & \text{ if }  L = \lttcase{l_i}{\ltenc{\tilde \tau}}{i \in I}  \\
  \btinp{\ltencr{\tilde \tau}}\tinact  & \text{ otherwise } L = \tilde \tau  
\end{cases}\\
% \ltencr{\lto{L}} &\defeq \begin{cases}
%   \btsel{l_i : \btout{\ltencr{\tilde \tau}\tinact}}_{i \in I} & \text{ if }  L = \lttcase{l_i}{\ltenc{\tilde \tau}}{i \in I}  \\
%   \btout{\ltencr{\tilde \tau}}\tinact  & \text{ otherwise } L = \tilde \tau  
% \end{cases}\\
\ltencr{\lttcase{l_i}{\tilde \tau}{u \in I}} &\defeq \tinact
      \\[1mm]
\noalign{\bf Enviroments:}
\ltencrlin{\Gamma \uplus x : \tau} & \defeq 
\begin{cases} 
  \ltencrlin{\Gamma}, x : \ltencr{\lti{\tilde \tau'}}, 
  \dual x : \ltencr{\lto{\tilde \tau'}}
  & \text{ if } 
  \tau \equiv \ltab{\tilde \tau'}
  \\ 
  \ltencrlin{\Gamma}, x : \ltencr{\tau} & 
  \text{ if } \lin{\tau} \text{ and } 
  \tau \not\equiv \ltab{\tilde \tau'}
  \\
  \ltencrlin{\Gamma} & \text{ otherwise }
\end{cases} 
\\ 
\ltencrun{\Gamma \uplus x : \tau} & \defeq  
\begin{cases} 
  \ltencrun{\Gamma}, x : \ltencr{\tau} & \text{ if } \un{\tau} 
  \\ 
  \ltencrun{\Gamma} & \text{ otherwise }
\end{cases} 
% \ltencr{\Gamma}, x : \ltencr{\tau} 
\\
\ltencrlin{\varnothing} & \defeq \emptyset 
\\
\ltencrun{\varnothing} & \defeq  \emptyset 
    \end{align*}
  % \end{tabular} 
  \end{mdframed}
  \caption{Typed encoding of linearly typed $\pi$ processes  into \msts processes.
  \label{pi:f:lsttomst}}
   \end{figure}


The translation in other direction is given in~\Cref{pi:f:lsttomst}. 
% Now, we provide translation in other direction: 
% from linear $\pi$ types into \msts: 



% \todo[inline]{TODO: translation from \msts to linear types}
\begin{restatable}[Minimality of \msts]{theorem}{mstminres}
    \label{pi:t:mstminres}
    We have the following 
      % Let $P$ be a \sessp process 
      % than we have
      \begin{enumerate}
        \item Let $P$ be a session typed \sessp-process 
        then 
         $\Gamma;\Delta \proves P \hastype \Proc \implies  
        \ltenc{\Gamma} \uplus \ltenc{\Delta}
        \proveslt \ltenc{P}$;
        \item Let $P$ be a linearly typed $\pi$-process 
        then  $\Gamma \proveslt P \implies  
        \ltencrun{\Gamma} ;  \ltencrlin{\Gamma}
        \proves \ltencr{P} \hastype \Proc$. 
      \end{enumerate}  
      % $$\Gamma;\Delta \proves P \iff
      % \ltenc{\Gamma}_{\emptyset}; \ltenc{\Delta}_{\emptyset} 
      % \proves \ltenc{P}_{\emptyset}
      % $$
      % such that 
      % $\Gamma;\Delta \proves P$. We have 
      % $$\horelm{\Gamma;\Delta}{P}{\ \mstb \ }
      % {\Gtopt{\Gamma};\Gtopt{\Delta}}{\Do{P}}$$ 
    \end{restatable} 

    \begin{proof}
      By induction on the structure of $P$ for both items 
      and definitions of  $\ltenc{\text{-}}$, 
      $\ltencrlin{\text{-}}$, $\ltencrun{\text{-}}$, 
      and $\ltencr{\text{-}}$. 
See~\Cref{pi:t:mstminres-proof} for details. 
    \end{proof}
  %  \input{mst-minimality-proof.tex}
% \todo[inline]{TODO: Minimality result}

==> sources/mst-minimality-proof.tex <==
\begin{proof}
  \label{pi:t:mstminres-proof}
    % By the induction on the structure of $P$. 
    We first consider Item~1. 
    \begin{enumerate}
      \item By the induction on the structure of $P$. 
      We consider Output, Selection, and Branching cases; 
      Input case is shown similarly to Output case. 
      \begin{enumerate}
      \item Case $P = \bout{u_i}{z_j}P'$. 
      Here by inversion of rule \textsc{Send} we have: 
      \begin{align}
        \label{pi:minlt:send:out-inv}
            \AxiomC{$\Gamma; \Delta 
            \proves P' \hastype \Proc 
            $} 
            \AxiomC{$\Gamma; \Delta_z \proves \tilde z_j \hastype \tilde C$} 
            \LeftLabel{\scriptsize \textsc{(PolySend)}}
            \BinaryInfC{$\Gamma; \Delta \cdot u_i:M 
            \cdot \Delta_z \proves \bout{u_i}{\tilde z_j}P' \hastype \Proc $} 
            \DisplayProof	
        \end{align}
        \noindent where $M = \btout{\tilde C}\tinact$. 
        We should show 
        \begin{align}
          \label{pi:minlt:send:goal}
          \ltenc{\Gamma} \uplus \ltenc{\Delta \cdot u_i:M \cdot \Delta_z} 
          \proves \ltenc{\bout{u_i}{\tilde z_j}P' } 
        \end{align}

        By IH on the first assumption of~\eqref{pi:minlt:send:out-inv} we have 

        \begin{align}
          \label{pi:minlt:send:out-inv-ih1}
          \ltenc{\Gamma} \uplus \ltenc{\Delta} 
          \proveslt \ltenc{P'}  
        \end{align}

        By the second assumption of~\eqref{pi:minlt:send:out-inv} 
        % and~\Cref{pi:f:msttolst} 
        we can infer the following  
        \begin{align} 
          \label{pi:minlt:send:out-inv-ih2}
        \ltenc{\Gamma} \uplus \ltenc{\Delta_z} 
              \proveslt \tilde z_j : \ltenc{\tilde C}
        \end{align} 

        Now, we can notice that by~\Cref{pi:f:msttolst} we have 
        $$\ltenc{M} = \ltenc{\btout{\tilde C}\tinact} 
        = \lto{\ltenc{\tilde C}}$$
        Further, we have
        \begin{align*}
          \ltenc{\Gamma} \uplus \ltenc{\Delta \cdot u_i:M \cdot \Delta_z} 
          = (\ltenc{\Gamma} \uplus \ltenc{u_i:{M}}) \uplus 
          ( \ltenc{\Gamma} \uplus \ltenc{\Delta_z} ) \uplus 
          (\ltenc{\Gamma} \uplus \ltenc{\Delta} )  
        \end{align*} 

        Thus,  the following tree proves this case:  
        \begin{align}
          \label{pi:pt:min:out-inv-goal}
              \AxiomC{$
              % \ltenc{\Gamma} \uplus 
              \ltenc{u_i:{M}} 
          \proveslt 
            u_i : \ltenc{M}
              $} 
              \AxiomC{$
              % \ltenc{\Gamma} \uplus \ltenc{\Delta_z} 
              % \proves \tilde z_j : \ltenc{\tilde C} 
              \eqref{pi:minlt:send:out-inv-ih2}
                $} 
              \LeftLabel{\scriptsize \textsc{(T$\pi$-Out)}}
              \AxiomC{$
              % \ltenc{\Gamma} \uplus \ltenc{\Delta} 
              % \proveslt \ltenc{P'}
              \eqref{pi:minlt:send:out-inv-ih1}
              $} 
              \TrinaryInfC{
                $
                \ltenc{\Gamma} \uplus \ltenc{\Delta \cdot u_i:M \cdot \Delta_z} 
                \proveslt {\bout{u_i}{\tilde z_j}\ltenc{P'} } 
              $} 
              \DisplayProof	
          \end{align}
          % \begin{align}
          %   \label{pi:pt:min:out-inv-goal}
          %       \AxiomC{$
          %       % \ltenc{\Gamma} \uplus 
          %       \ltenc{u_i:{M}} 
          %   \proveslt 
          %     u_i : \ltenc{M}
          %       $} 
          %       \AxiomC{$
          %       \ltenc{\Gamma} \uplus \ltenc{\Delta_z} 
          %       \proves \tilde z_j : \ltenc{\tilde C} 
          %         $} 
          %       \LeftLabel{\scriptsize \textsc{(T$\pi$-Out)}}
          %       \AxiomC{$
          %       \ltenc{\Gamma} \uplus \ltenc{\Delta} 
          %       \proveslt \ltenc{P'}
          %       $} 
          %       \TrinaryInfC{
          %         $
          %         \ltenc{\Gamma} \uplus \ltenc{\Delta \cdot u_i:M \cdot \Delta_z} 
          %         \proves {\bout{u_i}{\tilde z_j}\ltenc{P'} } 
          %       $} 
          %       \DisplayProof	
          %   \end{align}
          
        
      % \begin{align*}
      %   \AxiomC{$\bout{u_i}{z_j}P'$}
      %   \DisplayProof 
      % \end{align*} 
    

      \item Case $P= \bsel{u}{l_j}\news{c}\bout{u}{\dual c}{P'}$.  
      By inversion, we have the following typing derivation: 
    \begin{align}
      \label{pi:pt:min:sel1}
      \AxiomC{$
      \Gamma; 
      \Delta \cat  
      c : M_j \proves 
     {P'} \hastype \Proc 
      $}
      \AxiomC{$
      \Gamma; \dual c : \dual M_j \proves \dual c \hastype M_j 
      $}
      \LeftLabel{\scriptsize \textsc{Send}}    
      \BinaryInfC{
        $
        \Gamma; 
        \Delta  \cat u: \btout{\dual M_j}\tinact, 
        c : M_j, \dual c : \dual M_j \proves 
        \bout{u}{\dual c}{P'} \hastype \Proc 
        $
      }
      \DisplayProof 
    \end{align}
      \begin{align*}
        \AxiomC{
          \eqref{pi:pt:min:sel1}
          % $
          % \Gamma; 
          % \Delta  \cat u: \btout{\dual M_j}\tinact, 
          % c : M_j, \dual c : \dual M_j \proves 
          % \bout{u}{\dual c}{P'} \hastype \Proc 
          % $
        }
        \AxiomC{$M_j \dualof \dual M_j$}  
        \LeftLabel{\scriptsize \textsc{ResS}}         
         \BinaryInfC{$
        \Gamma; 
        \Delta  \cat u: \btout{\dual M_j}\tinact \proves 
        \news{c}\bout{u}{\dual c}{P'} \hastype \Proc 
        $} 
        \AxiomC{$
        j \in I
        $} 
        \LeftLabel{\scriptsize \textsc{Sel}}
        \BinaryInfC{$
          \Gamma; \Delta \cat 
          u:\btsel{l_i:\btout{\dual M_i}\tinact}_{i \in I} 
          \proves  
          \bsel{u}{l_j}\news{c}\bout{u}{\dual c}{P'} \hastype \Proc
          $} 
        \DisplayProof 
      \end{align*}
      % \begin{align*}
      %   \AxiomC{$
      %   \Gamma; \Lambda; \Delta \cat u: S_j  \proves P \hastype \Proc 
      %   $} 
      %   \AxiomC{$
      %   j \in I
      %   $} 
      %   \BinaryInfC{$
      %     \Gamma; \Lambda; \Delta \cat u:\btsel{l_i:S_i}_{i \in I} \proves \bsel{u}{l_j} P \hastype \Proc
      %     $} 
      %   \DisplayProof 
      % \end{align*}
        We should show the following 
        \begin{align}
          \ltenc{\Gamma}\uplus \ltenc{\Delta \cat 
          u:\btsel{l_i:\btout{\dual M_i}\tinact}_{i \in I}}  
          \proveslt 
          \ltenc{\bsel{u}{l_j}\news{c}\bout{u}{\dual c}{P'}} 
        \end{align}
        Here by~\Cref{pi:f:msttolst} we have 
        \begin{align*} 
        \ltenc{\btsel{l_i : \btout{\tilde M_i}{\tinact}}_{i \in I}} &\defeq 
        \lto{\lttcase{l_i}{\ltenc{\tilde M_i}}{i \in I}}
        \end{align*} 

        Further, by~\Cref{pi:f:msttolst} 
        and $M_j \dualof \dual M_j$, without loss of 
        generality, we can infer 
        \begin{align}
          \label{pi:minlt:sel-ih13}
          \ltenc{M_j} &= \lti{\tilde \tau'_j} \qquad  \qquad 
          \ltenc{\dual M_j} = \lto{\tilde \tau'_j}
        \end{align}

        % Thus, by this and~\eqref{pi:pt:min:sel1} 
        % we have 

        % \begin{align*}
        %   c : \lti{\tilde \tau'_j}
        % \end{align*}

        By~\Cref{pi:f:msttolst} we have 
        \begin{align*} 
        \ltenc{\bsel{u}{l_j}\news{c}\bout{u}{\dual c}{P'}} 
&\defeq \news{c}\bout{u}{l_j\_c}\ltenc{P'}
        \end{align*} 

        By IH on the first assumption of~\eqref{pi:pt:min:sel1} 
        we have 
        \begin{align}
          \label{pi:minlt:sel-ih1}
          \ltenc{\Gamma} \uplus 
          \ltenc{\Delta \cat  
          c : M_j} \proveslt  
         \ltenc{P'} 
        \end{align}

        By~\Cref{pi:f:msttolst} this is equivalent to 
        the following 
        \begin{align}
          \label{pi:minlt:sel-ih12}
          \ltenc{\Gamma} \uplus 
          \ltenc{\Delta} \cat  
          c : \ltenc{M_j} \proveslt  
         \ltenc{P'} 
        \end{align}
      
  %       \begin{align*}
  %         \inferrule[(T$\pi$-Out)]{
      % \Gamma_1 \proveslt x : \lto{\wtd \tau}
      % \qquad 
      % \wtd \Gamma_2 \proveslt \tilde v : \wtd \tau 
      % \quad 
      % \Gamma_3  \proveslt P}
      % {\Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3 
      % \proveslt \bout{x}{\tilde v}P}
  %       \end{align*}

  The following tree proves this case:  
        \begin{align}
          \label{pi:minlt:sel-1}
          \AxiomC{$
          \ltenc{\Gamma}, 
          % c : \ltenc{M_j} 
          c : \lto{\tilde \tau'_j} 
          \proveslt 
          % c : \ltenc{M_j}
          c : \lto{\tilde \tau'_j} 
          $} 
          \AxiomC{$j \in I$} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-LVal)}}
          \BinaryInfC{
            $
            \ltenc{\Gamma}, 
            % c : \ltenc{M_j}  
            c : \lto{\tilde \tau'_j}  
            \proveslt \ltvar{l_j}{c} : 
            \lttcase{l_i}{\ltenc{M_i}}{i \in I} 
            $
          } 
          \DisplayProof 
        \end{align}

        We may notice that the left-hand side of above derivation tree 
        follows by~\eqref{pi:minlt:sel-ih13}. 

        \begin{align*}
          \AxiomC{} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Var)}}
          \UnaryInfC{$
          u: \lto{\lttcase{l_i}{\ltenc{M_i}}{i \in I}}
          \proveslt 
          u: \lto{\lttcase{l_i}{\ltenc{M_i}}{i \in I}}
          $}
          \AxiomC{
            \eqref{pi:minlt:sel-1}
          } 
          \AxiomC{\eqref{pi:minlt:sel-ih12}} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Out)}}
          \TrinaryInfC{
            $
            \ltenc{\Gamma}\uplus \ltenc{\Delta} \cat
            % \ltenc{ 
            % u:\btsel{l_i:\btout{\dual M_i}\tinact}_{i \in I}} 
            u: \lto{\lttcase{l_i}{\ltenc{M_i}}{i \in I}}, 
            % c : \ltenc{M_j}  
             c : \ltab{\tilde \tau'_j}    
            \proveslt 
            \bout{u}{l_j\_c}\ltenc{P'}
            $
          } 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-res1)}}
          \UnaryInfC{$
            \ltenc{\Gamma}\uplus \ltenc{\Delta \cat 
            u:\btsel{l_i:\btout{\dual M_i}\tinact}_{i \in I}}  
            \proveslt 
            \news{c}\bout{u}{l_j\_c}\ltenc{P'}
          $} 
          \DisplayProof 
        \end{align*}
       
        This concludes Selection case.  

        \item Case $P = \bbra{u}{l_i:\binp{u}{c}P_i}_{i \in I}$. 
        By inversion, we have the following derivation tree 
        \begin{align}
          \label{pi:minlt:bra1}
          \AxiomC{$
          \Gamma; \Delta \cat c: M_i 
          \proves 
         P_i \hastype \Proc
          $} 
          \AxiomC{$
          \Gamma; c: M_j \proves c \hastype M_j 
          $} 
          \LeftLabel{\scriptsize \textsc{(Rcv)}}
          \BinaryInfC{$
          \Gamma; \Delta \cat 
          u:\btinp{M_i}\tinact \proves 
          \binp{u}{c}P_i \hastype \Proc
          $}
          \DisplayProof 
        \end{align}
        \begin{align}
          \label{pi:minlt:bra2}
          \AxiomC{$
          \forall i \in I
          $}
          \AxiomC{\eqref{pi:minlt:bra1}} 
        %   \AxiomC{$
        %   \Gamma; \Delta \cat c: M_i 
        %   \proves 
        %  P_i \hastype \Proc
        %   $} 
        %   \AxiomC{$
        %   \Gamma; c: M_j \proves c \hastype M_j 
        %   $} 
        %   \LeftLabel{\scriptsize \textsc{(Rcv)}}
        %   \BinaryInfC{$
        %   \Gamma; \Delta \cat 
        %   u:\btinp{M_i}\tinact \proves 
        %   \binp{u}{c}P_i \hastype \Proc
        %   $}
          \LeftLabel{\scriptsize \textsc{(Bra)}}
          \BinaryInfC{
            $
            \Gamma; \Delta \cat u: 
            \btbra{l_i:\btinp{M_i}\tinact}_{i \in I} \proves \bbra{u}{l_i:P_i}_{i \in I}\hastype \Proc
            $
          }
          \DisplayProof  
        \end{align}
        We should show the following 
        \begin{align} 
         \ltenc{\Gamma} \uplus 
         \ltenc{\Delta \cat u: 
            \btbra{l_i:\btinp{M_i}\tinact}_{i \in I}} 
            \proveslt \ltenc{\bbra{u}{l_i:P_i}_{i \in I}}
        \end{align} 
        
        Here, by~\Cref{pi:f:msttolst} we have 
        \begin{align*}
          \ltenc{
          \btbra{l_i:\btinp{M_i}\tinact}_{i \in I}}  = 
          \lti{\lttcase{l_i}{\ltenc{M_i}}{i \in I}}
        \end{align*}

        By IH on the first assumption on~\eqref{pi:minlt:bra1}
        we have 
        \begin{align} 
          \ltenc{\Gamma} \uplus 
          \ltenc{\Delta, c : M_i} \proveslt 
          \ltenc{P_i}
        \end{align} 

        By~\Cref{pi:f:msttolst} this is equivalent to the following 
        \begin{align} 
          \label{pi:minlt:bra-ih122}
          \ltenc{\Gamma_1} \uplus  \ltenc{\Delta}, 
          c:\ltenc{M_i} 
          \proveslt \ltenc{P_i}
        \end{align} 

        % ... 

        The following tree proves this case: 
        \begin{align} 
          \label{pi:minlt:bra-1}
          \AxiomC{} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Var)}}
          \UnaryInfC{$
          y :  \lttcase{l_i}{\ltenc{M_i}}{i \in I} \proveslt y :  \lttcase{l_i}{\ltenc{M_i}}{i \in I}
        $} 
        \AxiomC{
          \eqref{pi:minlt:bra-ih122}
          % $
          % \ltenc{\Gamma_1} \uplus  \ltenc{\Delta}, 
          % c:\ltenc{M_i} 
          % \proveslt \ltenc{P_i}
          % $
        } 
        \AxiomC{$
          \forall i \in I
        $}
        \LeftLabel{\scriptsize \textsc{(T$\pi$-Case)}}
        \TrinaryInfC{$
        \ltenc{\Gamma_1} \uplus  \ltenc{\Delta} \cat 
        y :  \lttcase{l_i}{\ltenc{M_i}}{i \in I}
        \proveslt 
\ltcase{y}{l_i}{c}{P_i}{i \in I}
        $} 
        \DisplayProof 
        \end{align} 

        \begin{align} 
          \AxiomC{} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Var)}}
          \UnaryInfC{$
          u : \lti{\lttcase{l_i}{\ltenc{M_i}}{i \in I}}  \proveslt u : 
            \lti{\lttcase{l_i}{\ltenc{M_i}}{i \in I}}$} 
          % \AxiomC{$
          %   \Gamma_1 \proveslt y :  \lttcase{l_i}{\ltenc{M_i}}{i \in I}
          % $} 
          \AxiomC{\eqref{pi:minlt:bra-1}} 
  %         \AxiomC{
  %           $
  %           \Gamma_2, c:\ltenc{M_i} \proveslt P_i
  %           $
  %         } 
  %         \AxiomC{$
  %           \forall i \in I
  %         $}
  %         \LeftLabel{\scriptsize \textsc{(T$\pi$-Case)}}
  %         \TrinaryInfC{$
  %         \Gamma_1 \uplus \Gamma_2 \proveslt 
      % \ltcase{y}{l_i}{c}{P_i}{i \in I}
  %         $} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Inp)}}
          \BinaryInfC{$
            \ltenc{\Gamma} \uplus 
            \ltenc{\Delta} 
            \cat 
            u : \lti{\lttcase{l_i}{\ltenc{M_i}}{i \in I}} 
            % \ltenc{u: 
            %  \btbra{l_i:\btinp{M_i}\tinact}_{i \in I}} 
            \proveslt 
            \binp{u}{y}\ltcase{y}{l_i}{c}{\ltenc{P_i}}{i \in I}
          $} 
          \DisplayProof 
        \end{align} 
        
        This concludes Branching case. 
      
    \end{enumerate}
    \item Now, we consider Item~2. By the induction on the structure of $P$.
   We consider Output, Selection, and Branching cases; 
    the Input case is shown similarly to Output case.  
    \begin{enumerate}
      \item Case $P = \bout{u_i}{z_j}P'$. 
      By inversion of rule \textsc{(T$\pi$-Out)} we have 
      \begin{align}
        \label{pi:minlt:send:ltmst:out-inv}
        \AxiomC{$\Gamma_1 \proveslt u_i : \lto{\wtd \tau}$} 
        \AxiomC{$\wtd \Gamma_2 \proveslt \tilde z_j : \wtd \tau $} 
        \AxiomC{$	\Gamma_3  \proveslt P'$} 
        \LeftLabel{\scriptsize \textsc{(T$\pi$-Out)}}
        \TrinaryInfC{
          $
          \Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3 
      \proveslt \bout{u_i}{\tilde z_j}P'
          $
        } 
        \DisplayProof 
      \end{align}

      We should show the following: 
      \begin{align}
        \label{pi:minlt:send:ltmst:goal}
        \ltencrun{\Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3} 
        ; 
        \ltencrlin{\Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3} 
      \proves \ltencr{\bout{u_i}{\tilde z_j}P'} 
      \end{align}

      By the first assumption of~\eqref{pi:minlt:send:ltmst:out-inv} 
      we have the following 
      \begin{align}
        \label{pi:minlt:send:ltmst:out-inv-ih1} 
        \ltencrun{\Gamma_1} ; 
        \ltencrlin{\Gamma_1}
         \proves u_i \hastype \ltencr{\lto{\tilde \tau}}
      \end{align} 

      Here by~\Cref{pi:f:lsttomst} we have 
      \begin{align*}
        \ltencr{\lto{\tilde \tau}} = 
        \btout{\ltencr{\tilde \tau}}\tinact 
      \end{align*}

      % \noindent From this we can infer the following 
      By the second assumption of~\eqref{pi:minlt:send:ltmst:out-inv} 
      we have the following 
      \begin{align}
        \label{pi:minlt:send:ltmst:out-inv-ih2} 
        \ltencrun{\wtd \Gamma_2} ; \ltencrlin{\wtd \Gamma_2} \proves 
        \tilde z_j \hastype \ltencr{\tilde \tau} 
      \end{align} 

      By IH on the third assumption of~\eqref{pi:minlt:send:ltmst:out-inv} 
      we have 
      \begin{align} 
        \label{pi:minlt:send:ltmst:out-inv-ih3} 
        \ltencrun{\Gamma_3}; 
        \ltencrlin{\Gamma_3}
        \proves \ltencr{P'} \hastype \Proc 
      \end{align} 

      By~\Cref{pi:f:lsttomst} we have the following 
      \begin{align*}
        % \ltencrun{\Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3} 
        % ; 
        \ltencrun{\Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3} 
        &= \ltencrun{\Gamma_1}, \ltencrun{\wtd \Gamma_2}, 
        \ltencrun{\Gamma_3} \\ 
        \ltencrlin{\Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3} 
        &= \ltencrlin{\Gamma_1}, \ltencrlin{\wtd \Gamma_2}, 
        \ltencrlin{\Gamma_3}
      \end{align*}

      The following tree proves this case:  
      \begin{align*}
        \AxiomC{
          % \eqref{pi:minlt:send:ltmst:out-inv-ih3}
          $ \ltencrun{\Gamma_3}; 
          \ltencrlin{\Gamma_3}
          \proves \ltencr{P'} \hastype \Proc  $
          } 
        \AxiomC{
          % \label{pi:minlt:send:ltmst:out-inv-ih2} 
          $\ltencrun{\wtd \Gamma_2} ; \ltencrlin{\wtd \Gamma_2} \proves 
          \tilde z_j \hastype \ltencr{\tilde \tau}$ 
        } 
        \LeftLabel{\scriptsize \textsc{(PolySend)}}
        \BinaryInfC{
          $\ltencrun{\Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3} 
        ; 
        \ltencrlin{\Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3} 
      \proves \ltencr{\bout{u_i}{\tilde z_j}P'} $
        } 
        \DisplayProof 
      \end{align*}
      This concludes Output case. 
      
      \item Case $P = \news{c}\bout{u}{l_j\_c}{P'}$. 
      We have the following derivation tree 
       \begin{align}
          \label{pi:minlt:lt:sel-1}
          \AxiomC{$
         c :  \lto{\tilde \tau'_j} 
          \proveslt c :  \lto{\tilde \tau'_j}
          $} 
          \AxiomC{$j \in I$} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-LVal)}}
          \BinaryInfC{
            $
            c: \lto{\tilde \tau'_j} \proveslt \ltvar{l_j}{c} : 
            \lttcase{l_i}{\tau_i}{i \in I} 
            $
          } 
          \DisplayProof 
        \end{align}
        \begin{align}
          \label{pi:minlt:lt:sel-2}
          \AxiomC{}
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Var)}}
          \UnaryInfC{$
          u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}
          \proveslt 
          u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}
          $}
          \AxiomC{
            \eqref{pi:minlt:lt:sel-1}
          } 
          \AxiomC{
            % \eqref{pi:minlt:sel-ih1}
            $\Gamma, c: \lti{\tilde \tau'_j} \proveslt P'$ 
            } 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Out)}}
          \TrinaryInfC{
            $
            \Gamma, 
            u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}, 
            c : \ltab{\tilde \tau'_j}
            \proveslt 
            \bout{u}{l_j\_c}{P'}
            $
          } 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-res1)}}
          \UnaryInfC{$
            % \ltenc{\Gamma}\uplus \ltenc{\Delta \cat 
            % u:\btsel{l_i:\btout{\dual M_i}\tinact}_{i \in I}}  
            \Gamma, 
            u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}
            \proveslt 
            \news{c}\bout{u}{l_j\_c}{P'}
          $} 
          \DisplayProof 
        \end{align}

        We should show the following 
        \begin{align}
          \ltencrun{\Gamma, 
          u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}; 
          \ltencrlin{\Gamma, 
          u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
          \proves 
          \ltencr{\news{c}\bout{u}{l_j\_c}{P'}} 
        \end{align}

        % From the typing rule in~\eqref{pi:minlt:lt:sel-1}
        % we infer the following  
        % \begin{align*}
        %   \tau_j = \ltab{\tilde \tau'_j}
        % \end{align*}

        By~\Cref{pi:f:lsttomst} and the first assumption 
        of~\eqref{pi:minlt:lt:sel-2}
        we have 
        \begin{align*}
          \ltencr{\lto{\lttcase{l_i}{{\tau_i}}{i \in I}}} 
          = 
          \btsel{l_i : \btout{\ltencr{\tau_i}}\tinact}_{i \in I}
        \end{align*} 

        By IH on the third assumption of~\eqref{pi:minlt:lt:sel-2} 
        we have 
        % \Gamma, c: \lti{\tilde \tau'_j} \proveslt P'
        \begin{align}
          \label{pi:minlt:lt:sel-ih1}
          \ltencrun{\Gamma, c: \lti{\tilde \tau'_j} }; 
          \ltencrlin{\Gamma, c: \lti{\tilde \tau'_j} } \proves 
            \ltencr{P'}
            \hastype \Proc 
        \end{align} 
        \noindent By~\Cref{pi:f:lsttomst} this judgment is equivalent to 
        \begin{align}
          \label{pi:minlt:lt:sel-ih2} 
          \ltencrun{\Gamma}; \ltencrlin{\Gamma}  
          % \ltencrlin{ u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
          % u :  \btout{\ltencr{\tau_j}}\tinact
          % \cat c : \ltencr{\ltab{\tilde \tau'_j}} 
          \cat c : \ltencr{\lti{\tilde \tau'_j}}
          % \cat \dual c : \ltencr{\lto{\tilde \tau'_j}}
          \proves 
          {\ltencr{P'}}
          \hastype \Proc 
        \end{align}
        Further, we have 
        \begin{align*}
          \ltencr{\news{c}\bout{f_x}{l_j\_c}{P}} 
= 
{\news{c}\bsel{x}{l_j}\bout{x}{c}{\ltencr{P}}}
        \end{align*}
        and 
        \begin{align*}
          &\ltencrun{\Gamma, 
          u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}; 
          \ltencrlin{\Gamma, 
          u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}} 
          = \\
           &\ltencrun{\Gamma}; \ltencrlin{\Gamma} \cat 
          \ltencrlin{ u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
          = \\
           &\ltencrun{\Gamma}; \ltencrlin{\Gamma} \cat 
          % \ltencrlin{ u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
          u : \btsel{l_i : \btout{\ltencr{\tau_i}}\tinact}_{i \in I}
        \end{align*}

        The following tree proves this case:  
        \begin{align}
          \label{pi:min:lt:sel-1}
          \AxiomC{
            \eqref{pi:minlt:lt:sel-ih2}
            % $
            % \ltencrun{\Gamma}; \ltencrlin{\Gamma}  
            % % \ltencrlin{ u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
            % % u :  \btout{\ltencr{\tau_j}}\tinact
            % % \cat c : \ltencr{\ltab{\tilde \tau'_j}} 
            % \cat c : \ltencr{\lti{\tilde \tau'_j}}
            % \proves 
            % {\ltencr{P'}}
            % \hastype \Proc 
            % $
          } 
          \AxiomC{}
          \LeftLabel{\scriptsize \textsc{(Sess)}}
          \UnaryInfC{$
            \ltencrun{\Gamma}; 
            % \ltencrlin{ u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
            % u :  \btout{\ltencr{\tau_j}}\tinact
            % \cat c : \ltencr{\ltab{\tilde \tau'_j}} 
            % \cat c : \ltencr{\lti{\tilde \tau'_j}}
             \dual c : \ltencr{\lto{\tilde \tau'_j}}
            \proves 
            {\dual c}
            \hastype \ltencr{\lto{\tilde \tau'_j}}
          $} 
          % \AxiomC{} 
          \LeftLabel{\scriptsize \textsc{(Send)}}
          \BinaryInfC{
          \begin{tabular}{l}  
          $
            \ltencrun{\Gamma}; \ltencrlin{\Gamma} \cat 
            % \ltencrlin{ u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
            u :  \btout{\ltencr{\tau_j}}\tinact
            % \cat c : \ltencr{\ltab{\tilde \tau'_j}} 
            \cat c : \ltencr{\lti{\tilde \tau'_j}}
            \cat \dual c : \ltencr{\lto{\tilde \tau'_j}}
            \proves$  \\
            $\bout{u}{\dual c}{\ltencr{P'}}
            \hastype \Proc 
          $
          \end{tabular}} 
          \AxiomC{$j \in I$} 
          \LeftLabel{\scriptsize \textsc{(Sel)}}
          \BinaryInfC{
          \begin{tabular}{l}  
          $
          \ltencrun{\Gamma}; \ltencrlin{\Gamma} \cat 
          % \ltencrlin{ u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
          u : \btsel{l_i : \btout{\ltencr{\tau_i}}\tinact}_{i \in I}
          % \cat c : \ltencr{\ltab{\tilde \tau'_j}} 
          \cat c : \ltencr{\lti{\tilde \tau'_j}}
          \cat \dual c : \ltencr{\lto{\tilde \tau'_j}}
          \proves$ \\ $ 
          \bsel{u}{l_j}\bout{u}{\dual c}{\ltencr{P'}}
          \hastype \Proc 
          $
          \end{tabular}} 
          \DisplayProof 
        \end{align}
        \begin{align*}
          \AxiomC{
            \eqref{pi:min:lt:sel-1}
          %   $
          % \ltencrun{\Gamma}; \ltencrlin{\Gamma} \cat 
          % % \ltencrlin{ u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
          % u : \btsel{l_i : \btout{\ltencr{\tau_i}}\tinact}_{i \in I}
          % % \cat c : \ltencr{\ltab{\tilde \tau'_j}} 
          % \cat c : \ltencr{\lti{\tilde \tau'_j}}
          % \cat \dual c : \ltencr{\lto{\tilde \tau'_j}}
          % \proves 
          % \bsel{u}{l_j}\bout{u}{\dual c}{\ltencr{P'}}
          % \hastype \Proc 
          % $
          } 
          \AxiomC{$\ltencr{\lti{\tilde \tau'_j}} \dualof \ltencr{\lto{\tilde \tau'_j}}$} 
          \LeftLabel{\scriptsize \textsc{(ResS)}}
          \BinaryInfC{$
          \ltencrun{\Gamma}; \ltencrlin{\Gamma} \cat 
          % \ltencrlin{ u : \lto{\lttcase{l_i}{{\tau_i}}{i \in I}}}
          u : \btsel{l_i : \btout{\ltencr{\tau_i}}\tinact}_{i \in I}
          \proves 
          \news{c}\bsel{u}{l_j}\bout{u}{\dual c}{\ltencr{P'}}
          \hastype \Proc 
          $} 
          \DisplayProof 
        \end{align*}
        This concludes Selection case. 

        \item Case $P = \binp{u}{y}\ltcase{y}{l_i}{c}{{P_i}}{i \in I}$. 
        By inversion we have the following derivation tree 
        \begin{align} 
          \label{pi:minlt:lt:bra-1}
          \AxiomC{} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Var)}}
          \UnaryInfC{$
          y :  \lttcase{l_i}{\tau_i}{i \in I} \proveslt y :  \lttcase{l_i}{\tau_i}{i \in I}
        $} 
        \AxiomC{
          % \eqref{pi:minlt:bra-ih122}
          $
          \Gamma_1 \uplus 
          c:\tau_i  
          \proveslt {P_i}
          $
        } 
        \AxiomC{$
          \forall i \in I
        $}
        \LeftLabel{\scriptsize \textsc{(T$\pi$-Case)}}
        \TrinaryInfC{$
          \Gamma_1 \uplus
          y :  \lttcase{l_i}{\tau_i}{i \in I}
          \proveslt 
  \ltcase{y}{l_i}{c}{P_i}{i \in I}
        $} 
        \DisplayProof 
        \end{align} 

        \begin{align} 
          \AxiomC{} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Var)}}
          \UnaryInfC{$
          u : \lti{\lttcase{l_i}{\tau_i}{i \in I}}  \proveslt u : 
            \lti{\lttcase{l_i}{\tau_i}{i \in I}}$} 
          \AxiomC{\eqref{pi:minlt:lt:bra-1}} 
          \LeftLabel{\scriptsize \textsc{(T$\pi$-Inp)}}
          \BinaryInfC{$
            % \ltenc{\Gamma} \uplus 
            % \ltenc{\Delta} 
            \Gamma_1 
            \uplus  
            u : \lti{\lttcase{l_i}{\tau_i}{i \in I}} 
            % \ltenc{u: 
            %  \btbra{l_i:\btinp{M_i}\tinact}_{i \in I}} 
            \proveslt 
            \binp{u}{y}\ltcase{y}{l_i}{c}{{P_i}}{i \in I}
          $} 
          \DisplayProof 
        \end{align} 

        We should show the following 
       \begin{align}
        \begin{tabular}{l}
       $\ltencrun{\Gamma_1 
        \uplus  
        u : \lti{\lttcase{l_i}{\tau_i}{i \in I}}}; 
        \ltencrlin{\Gamma_1 
        \uplus  
        u : \lti{\lttcase{l_i}{\tau_i}{i \in I}}} 
        % \ltenc{u: 
        %  \btbra{l_i:\btinp{M_i}\tinact}_{i \in I}} 
        \proveslt$ 
        \\ 
        $\ltencr{\binp{u}{y}\ltcase{y}{l_i}{c}{{P_i}}{i \in I}} $
        \end{tabular}
       \end{align}

       Here by~\Cref{pi:f:lsttomst} we have 
       \begin{align*}
        \ltencr{\lti{\lttcase{l_i}{\tau_i}{i \in I}}} 
        = 
        \btbra{l_i : \btinp{\ltencr{\tau_i}}\tinact}_{i \in I}
       \end{align*}

       By IH on the second assumption of~\eqref{pi:minlt:lt:bra-1}
       we have 
       \begin{align}
        \ltencrun{\Gamma_1 \uplus 
        c:\tau_i}; 
        \ltencrlin{\Gamma_1 \uplus 
        c:\tau_i}
        \proveslt 
        \ltencr{P_i}
       \end{align}
       By~\Cref{pi:f:lsttomst} this is equivalent
      to the following 
      \begin{align}
        \label{pi:minlt:lt:bra-ih1}
        \ltencrun{\Gamma_1}; 
        \ltencrlin{\Gamma_1} \cat 
        c:\ltencr{\tau_i} 
        \proveslt 
        \ltencr{P_i}
       \end{align}  

       The following tree proves this case 
       \begin{align}
        \label{pi:minlt:ltmst:bra1}
        \AxiomC{\eqref{pi:minlt:lt:bra-ih1}}
      %   \AxiomC{$
      %   \ltencrun{\Gamma_1}; 
      %     \ltencrlin{\Gamma_1} \cat c:\ltencr{\tau_i} 
      %   \proves 
      %  P_i \hastype \Proc
      %   $} 
      \AxiomC{} 
      \LeftLabel{\scriptsize \textsc{(Sess)}}
        \UnaryInfC{$
        \ltencrun{\Gamma_1};  c: \ltencr{\tau_i} 
        \proves c \hastype \ltencr{\tau_i} 
        $} 
        \LeftLabel{\scriptsize \textsc{(Rcv)}}
        \BinaryInfC{$
          \ltencrun{\Gamma_1}; 
          \ltencrlin{\Gamma_1} \cat 
          u:\btinp{\ltencr{\tau_i}}\tinact \proves 
          \binp{u}{c}P_i \hastype \Proc
        $}
        \DisplayProof 
      \end{align}
      \begin{align}
        \label{pi:minlt:ltmst:bra2}
        \AxiomC{$
        \forall i \in I
        $}
        \AxiomC{\eqref{pi:minlt:ltmst:bra1}} 
        \LeftLabel{\scriptsize \textsc{(Bra)}}
        \BinaryInfC{
          $
          \ltencrun{\Gamma_1}; 
          \ltencrlin{\Gamma_1}
          \cat 
          % \ltencrlin{
          % u : \lti{\lttcase{l_i}{\tau_i}{i \in I}}} 
          u : \btbra{l_i : \btinp{\ltencr{\tau_i}}\tinact}_{i \in I}
          % \Gamma; \Delta \cat u: 
          % \btbra{l_i:\btinp{M_i}\tinact}_{i \in I} 
          \proves \bbra{u}{l_i: \binp{u}{c}P_i}_{i \in I}\hastype \Proc
          $
        }
        \DisplayProof  
      \end{align}
      This concludes Branching case. 

      
    \end{enumerate}
    \end{enumerate}


  \end{proof}

==> sources/optimtable.tex <==
\begin{table*}
  \begin{tabular}{ |l|l|l|l|}
    \rowcolor{gray!25}
    \hline
     & $P$ &
      \multicolumn{2}{l|}{
    \begin{tabular}{l}
      \noalign{\smallskip}
      $\Bopt{k}{\tilde x}{P}$
      \smallskip
    \end{tabular}
  }  \\
    \hline
    1 & $\binp{u_i}{y}Q$
  & 
    \begin{tabular}{l}
        \noalign{\smallskip}
        $\propinp{k}{\wtd x}\binp{u_{\mstindex}}{\wtd y} \apropout{k+1}{\wtd z}
       \Par \Bopt{k+1}{\tilde z}{Q\sigma}$
        \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{l}
      \noalign{\smallskip}
    $y_j:S$ $\wedge$ $\widetilde y = (y_1,\ldots,y_{\len{S}})$ \\
    $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
  %   $\wtd w = \begin{cases}
  %  \{ u_i \} & \text{if} \ \lin{u_i} \\
  %  \epsilon & \text{otherwise} 	
  %  \end{cases}
  % $ \\ 
      $\widetilde z = \fnb{Q}{\widetilde x \widetilde y \setminus \wtd w}$\\
      $\mstindex = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
      $\sigma = \nextn{u_i} \cdot \subst{y_1}{y}$
      \smallskip
    \end{tabular}
      \\
    \hline
    
    2 & $\bout{u_i}{y_j}{Q}$ &
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\propinp{k}{\widetilde x}
        \bbout{u_{\mstindex}}{\widetilde y}
        \apropout{k+1}{\widetilde z}  \Par \Bopt{k+1}{\tilde z}{Q\sigma}$
       \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{ll}
      \noalign{\smallskip}
  $y_j : S \wedge \wtd y = (y_j, \ldots,y_{j+\len{\Gtopt{S}}-1})$ \\
  % $\wtd w = \begin{cases}
  %  \{ u_i \} & \text{if} \ \lin{u_i} \\
  %  \epsilon & \text{otherwise} 	
  %  \end{cases}
  % $ \\ 
  $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
       $\wtd z = \fnb{Q}{\wtd x \setminus \wtd w}$\\
       $\mstindex = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
      $\sigma = \nextn{u_i}$ 
      \smallskip
    \end{tabular}
    \\
  \hline 
  3 &  $\news{s:C}{Q}$ &
    \begin{tabular}{l}
      \noalign{\smallskip}
     $\news{\widetilde{s}:\Gtopt{C}}{\,\Bopt{k}{\tilde x}
         {Q\sigma}}$
      \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{l}
      \noalign{\smallskip}
      $\widetilde{s} = (s_1,\ldots,s_{\len{\Gtopt{C}}})$ \\
      $\sigma = \subst{s_1 \dual{s_1}}{s \dual{s}} $
  %   $\sigma = \begin{cases}
  %         \subst{s_1 \dual{s_1}}{s \dual{s}} & \text{if} \ C = S \\
  %         \subst{s_1}{s} & \text{if} \ C = \chtype{U}
  % \end{cases}
  % $
      \smallskip
    \end{tabular}
    \\
    \hline
    4 &    $\news{s:\trec{t}{S}}{Q}$
       &
        \begin{tabular}{l}
            \noalign{\smallskip}
             $\news{\widetilde{s}:\Rtopt{S}}$ 
         $\big(\propinp{k}{\wtd x}\propout{k+1}{\wtd z}\inact \Par \Bopt{k+1}{\tilde z}{Q}\big)$
        \smallskip
        \end{tabular} & 
        \begin{tabular}{ll}
            \noalign{\smallskip}
            $\mathsf{tr}(\trec{t}{S})$ &
            $\widetilde{s} = (s_1,\ldots,s_{\len{\Rtopt{S}}})$ 
            \\
            $\wtd z = \wtd x, \wtd s, \wtd {\dual s}$ &             $\widetilde {\dual{s}} = (\dual{s_1},\ldots,\dual{s_{\len{\Rtopt{S}}}})$ 
        \smallskip
        \end{tabular} \\
      \hline 

      5 & $Q_1 \Par Q_2$ &
    \begin{tabular}{l}
      \noalign{\smallskip}
      $\propinp{k}{\widetilde x} \propout{k+1}{\widetilde y}
      \apropout{k+\degree+1}{\widetilde z}  
       \Par \Bopt{k+1}{\tilde y}{Q_1} \Par \Bopt{k+\degree+1}{\tilde z}{Q_2}$
      \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{lll}
      \noalign{\smallskip}
      $\widetilde y  = \fnb{Q_1}{\widetilde x}$
      %  \\
      % &
      $\quad$
      $\widetilde z = \fnb{Q_2}{\widetilde x}$ \\
      
      $\degree = \len{Q_1}$
      \smallskip
    \end{tabular}
        \\
    \hline
    6 & $\inact$ &
  \begin{tabular}{l}
    \noalign{\smallskip}
    $\propinp{k}{}\inact$
   \smallskip
  \end{tabular}
  &
  \begin{tabular}{l}
    \noalign{\smallskip}
  \smallskip
  \end{tabular}
    \\
    \hline %\hline
    %%%%%%
    %% =======================
    %%%%%%
      % $\B{k}{\tilde x}{\bout{r}{y_j}{Q}}$ & 
    %   $\bout{r}{y_j}{Q}$ &
    %     \begin{tabular}{l}
    %         \noalign{\smallskip}
    %         $\propinp{k}{\widetilde x}
    %           \bbout{r_{f(S)}}{\widetilde y} 
    %           \apropout{k+1}{\widetilde z}
    %          \Par$ 
    %         %  \\
    %         $\B{k+1}{\tilde z}{Q}$
    %       \smallskip
    %     \end{tabular} & 
    %     \begin{tabular}{l}
    %            \noalign{\smallskip}
    %            $y : T$ $\wedge  \wtd y = (y_j,\ldots,y_{j + \len{\Gt{T}}-1})$\\
    %         $r:S \wedge \mathsf{tr}(S)$ \\
    %         $\wtd z = \fnb{Q}{\wtd x}$ 
    %         % \\
    %         % $(r_1,\ldots,r_{\len{\Gt{S}}}) \subseteq \wtd x$ % 
    %         \smallskip
    %     \end{tabular} 
    %     \\
    %   \hline     
    % % $\B{k}{\tilde x}{\binp{r}{y}Q}$
    % $\binp{r}{y}Q$
    % &
    %     \begin{tabular}{l}
    %       \noalign{\smallskip}
    %       $\propinp{k}{\widetilde x}
    %           \binp{r_{f(S)}}{\widetilde y}
    %           \apropout{k+1}{\widetilde z}
    %             \Par$ 
    %             % \\
    %         $\B{k+1}{\tilde z}{Q}$
    %       \smallskip
    %     \end{tabular} & 
    %     \begin{tabular}{l}
    %         \noalign{\smallskip}
    %         $r:S \wedge \mathsf{tr}(S)$ \\
    % $\wtd z = \fnb{Q}{\wtd x\wtd y}$  
    % % \\
    % % $(r_1,\ldots,r_{\len{\Gt{S}}}) \subseteq \wtd x$
    %   \smallskip
    %     \end{tabular} 
      %   \\
      % \hline 
      %  $\B{k}{\tilde x}{\news{s:\trec{t}{S}}{Q}}$
      % $\B{k}{\tilde x}{\recp{X}P}$
      7 & $\recp{X}P$
      &
        \begin{tabular}{l}
            \noalign{\smallskip}
            $\news{\prop^r_X}(\propinp{k}{\wtd x}
                \propoutrec{k+1}{\wtd z}
              \recp{X}\binp{\prop^r_{X}}{\wtd y}
        \propoutrec{k+1}{\wtd y}X
            \Par \Brec{k+1}{\tilde z}{P}_{g})$
         \smallskip
        \end{tabular} & 
        \begin{tabular}{ll}
               \noalign{\smallskip}
                %  $\len{\wtd y} = \len{\wtd x}$ \\
                %  $\wtd n = \fn{P}$ &
                 $\wtd n = \fs{P}$ &
                 $\wtd n : \wtd C$ $\wedge$ $\wtd z = \bname{\wtd n : \wtd C}$ \\
                %  $\wtd z = \wtd m$, 
                 $\len{\wtd z} = \len{\wtd y}$ &
                 $g = \{X \mapsto \wtd z\}$
            \smallskip
        \end{tabular} \\
        \hline 
      % \end{tabular} 
        
      % \begin{tabular} 
        \hline
            %%%%%%
    %% =======================
    %% =======================
    %%%%%%
    \rowcolor{gray!25}
    %\hline
     & $P$ &
      \multicolumn{2}{l|}{
    \begin{tabular}{l}
      \noalign{\smallskip}
      $\Brec{k}{\tilde x}{P}_g$
      \smallskip
    \end{tabular}
  }  \\
    \hline
    8 & $\bout{u_i}{y_j}{Q}$ & 
      \begin{tabular}{ll}
      \noalign{\smallskip}
      $\recp{X}\binp{\prop^r_k}{\widetilde x}
        \bout{u_l}{\widetilde y} 
        \propoutrec{k+1}{\wtd z}\rvar{X}
%      		\bout{\prop^r_{k+1}}{\widetilde z}X
       \Par\Brec{k+1}{\tilde z}{Q\sigma}_g$ 
       & $(\text{if } g \neq  \es)$  
      \smallskip
      \\
      \hdashline 
      \noalign{\smallskip}
      % \noalign{\hbox to \textwidth{\leaders\hbox to 3pt{\hss . \hss}\hfil}}
      $\recp{X}\propinprecsh{k}{\wtd x}
      \big(\bout{u_{\mstindex}}{\wtd y} 
        \apropoutrecsh{k+1}{\wtd z} \Par \rvar{X}\big) 
%      		\bout{\prop^r_{k+1}}{\widetilde z}X
       \Par$ 
      %  \\
      $\Brec{k+1}{\tilde z}{Q\sigma}_g 
      $ &  $(\text{if } g = \es)$
    \smallskip
  \end{tabular} & 
  \begin{tabular}{l}
         \noalign{\smallskip}
         $y : T$ $\wedge (y_j,\ldots,y_{j+\len{\Gtopt{T}}-1})$ \\ 
      % $r:S \wedge \mathsf{tr}(S)$ \\
      $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
      $\wtd z = g(X) \cup \fnb{Q}{\wtd x \setminus \wtd w}$  \\
      $l = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
      $\sigma = \nextn{u_i}$
      \smallskip
  \end{tabular} 
  \\
\hline 
  9 & $\binp{u_i}{y}{Q}$
  &
  \begin{tabular}{ll}
      \noalign{\smallskip}
      $\recp{X}\binp{\prop^r_k}{\widetilde x}
        \binp{u_l}{\widetilde y} 
        \propoutrec{k+1}{\wtd z}
        \rvar{X}
       \Par \Brec{k+1}{\tilde z}{Q\sigma}_g$
       & $(\text{if } g \neq  \es)$  
      % \small
       \smallskip
      \\
      \hdashline 
      \noalign{\smallskip}
      % \noalign{\hbox to \textwidth{\leaders\hbox to 3pt{\hss . \hss}\hfil}}
      $\recp{X}\propinprecsh{k}{\wtd x}
      \big(\binp{u_{\mstindex}}{\wtd y} 
        \apropoutrecsh{k+1}{\wtd z} \Par \rvar{X}\big) 
%      		\bout{\prop^r_{k+1}}{\widetilde z}X
       \Par \Brec{k+1}{\tilde z}{Q\sigma}_g$ 
       &
       $(\text{if } g = \es)$
      \smallskip 
  \end{tabular} & 
  \begin{tabular}{l}
         \noalign{\smallskip}
      % $r:S \wedge \mathsf{tr}(S)$ \\
      $\wtd w = \linecondit{\lin{u_i}}{\{ u_i \}}{\epsilon}$ \\
      $\wtd z = g(X) \cup \fnb{Q}{\wtd x \wtd y \setminus \wtd w}$  \\
      $l = \linecondit{\mathtt{tr}(u_i)}{f(S)}{i}$ \\
      $\sigma = \nextn{u_i} \cdot \subst{y_1}{y}$
      % $\wtd z = \fnb{Q}{\wtd x \wtd y}$  
      \smallskip
  \end{tabular} 
  \\
\hline
10 & $Q_1 \Par Q_2$
& 
\begin{tabular}{ll}
      \noalign{\smallskip}
      $\recp{X}\proprinpk{r}{k}{\wtd x}\big(\proproutk{r}{k+1}{\wtd y_1}\rvar{X}
      \Par \apropoutrecsh{k+\degree+1}{\wtd y_2}\big)
       \Par$
      & 
       $(\text{if } g \neq  \es)$  
    \smallskip
    \\
      \qquad \qquad $\Brec{k+1}{\tilde y_1}{Q_1}_{g} \Par 
      \Brec{k+\degree+1}{\tilde y_2}{Q_2}_{\es}$
      &   
    \smallskip
    \\
      \hdashline 
      \noalign{\smallskip}
      $\recp{X}\proprinpk{r}{k}{\wtd x}\big(\apropoutrecsh{k+1}{\wtd y_1}
      \Par \apropoutrecsh{k+\degree+1}{\wtd y_2} \Par \rvar{X}\big)
       \Par$ 
       \smallskip
       \\
      \qquad \qquad  $\Brec{k+1}{\tilde y_1}{Q_1}_{\es} \Par 
      \Brec{k+\degree+1}{\tilde y_2}{Q_2}_{\es}$ &
      $(\text{if  $g = \es$})$
      \smallskip
  \end{tabular} & 
  \begin{tabular}{l}
         \noalign{\smallskip}
         $\recpx{Q_1}$ \\
         $\wtd y_1  = g(X) \cup \fnb{Q_1}{\wtd x}$ \\
         $\wtd y_2  =  \fnb{Q_2}{\wtd x}$ \\
        %  $i \in \{1,2\}.$ \\
        %  $\quad \wtd y_i' = \linecondit{\recpx{Q_i}}{g(X)}{\epsilon}$ \\
        %  $\quad g_i = \linecondit{\recpx{Q_i}}{g_i}{\epsilon}$ \\
        %  $\quad \wtd y_i  = \wtd y_i' \cup \fnb{Q_i}{\wtd x}$ \\
         $\degree = \len{Q_1}$
      \smallskip
  \end{tabular} 
  \\
  \hline
  11 & ${\news{s:C}{Q}}$ & 
  \begin{tabular}{ll}
      \noalign{\smallskip}
      % $\news{\widetilde{s}:\Gt{C}}$ 
      $\recp{X}\news{\widetilde{s}:\Gtopt{C}}\proprinpk{r}{k}{\wtd x}\proproutk{r}{k+1}{\wtd z}X
      \Par
      \Brec{k+1}{\tilde z}{Q\sigma}_g$
      & $(\text{if } g \neq \es)$
      \smallskip
      \\
      \hdashline 
      \noalign{\smallskip}
      $\recp{X}\news{\wtd{s}:\Gtopt{C}}
      \proprinpk{r}{k}{\wtd x}\big(\apropoutrecsh{k+1}{\wtd z} \Par X\big)
      \Par
      \Brec{k+1}{\tilde z}{Q\sigma}_g$ 
      & $(\text{if } g = \es)$
  %  \smallskip
  \end{tabular} & 
  \begin{tabular}{l}
      \noalign{\smallskip}
        %  $\mathsf{tr}(\trec{t}{S})$ \\
         $\widetilde{s} = (s_1,\ldots,s_{\len{\Gtopt{S}}})$ \\
         $\widetilde {\dual{s}} =
          \linecondit{\lin{S}}{(\dual{s_1},\ldots,\dual{s_{\len{\Gtopt{S}}}})}{\epsilon}$ \\
  %        $\widetilde {\dual{s}} = \begin{cases}
  %         (\dual{s_1},\ldots,\dual{s_{\len{\Gt{S}}}}) & \text{if} \ C = S \\
  %         \epsilon & \text{if} \ C = \chtype{U}
  % \end{cases}
  % $\\
        %  $\widetilde {\dual{s}} = (\dual{s_1},\ldots,\dual{s_{\len{\Rtopt{S}}}})$ \\
         $\wtd z = \wtd x, \wtd s, \wtd {\dual s}$ \qquad
         $\sigma = \subst{s_1 \dual{s_1}}{s \dual{s}} $
      \smallskip
  \end{tabular} 
  \\
\hline
12 & $X$ 
 &  
 \begin{tabular}{ll}
  \noalign{\smallskip}
 $\recp{X}\proprinpk{r}{k}{\wtd x}\apropoutrecsh{\rvar{X}}{\wtd x}\rvar{X}$
 & $(\text{if } g \not= \es)$
%  \qquad 
\smallskip
\\
\hdashline 
\noalign{\smallskip}
 $\recp{X}\proprinpk{r}{k}{}\big(\apropoutrecsh{\rvar{X}}{} \Par X\big)$
 & $(\text{if } g = \es)$
 \smallskip
 \end{tabular}
 & 
%  \begin{tabular}{l}
%         \noalign{\smallskip}
%         $\wtd x = g(X)$
%      \smallskip
%  \end{tabular} 
  \\
\hline
13 &  $\inact$ &
  \begin{tabular}{l}
    \noalign{\smallskip}
    $\proprinpk{r}{k}{}\inact$
   \smallskip
  \end{tabular}
  &
  \begin{tabular}{l}
    \noalign{\smallskip}
  \smallskip
  \end{tabular}
  \\
    \hline
\end{tabular}
  \caption{Optimized breakdown function  $\Bopt{k}{\tilde x}{\cdot}$ for processes, and auxiliary function for recursive processes $\Brec{k}{\tilde x}{\cdot}_g$. \label{pi:t:bdowncorec}}
  \vspace{-3mm}
  \end{table*}

==> sources/preliminaries-backup.tex <==

We are concerned with \sessp, which is one of the sub-languages of \HOp~\cite{KouzapasPY17,DBLP:journals/iandc/KouzapasPY19}, for which we recall its syntax, semantics, and session type system. 
We also recall the mutual encodings between \sessp and
  \HO, the other relevant sub-language of \HOp~\cite{DBLP:conf/esop/KouzapasPY16,DBLP:journals/iandc/KouzapasPY19}. 
 Finally, we briefly discuss \msts for \HO and the minimality result in~\cite{APV19}. 

\subsection{\HOp (and its Sub-languages \HO and \sessp)}
%\noindent For the purpose of keeping this subsection as a short overview, we introduce the details defining \HOp, as they include both \HO and \sessp-calculus. The syntax and operational semantics %and the type systemare identical to those defined in \cite{MinimalSessionTypes}. We proceed by borrowing the presented information.\\


	\begin{figure}[!t]
	\begin{mdframed}[style=alttight]
				\begin{align*}
			n   \bnfis &  a,b \bnfbar s, \dual{s} 
			\\
			u,w   \bnfis & n \bnfbar x,y,z 
			\\
			V,W   \bnfis &\nonhosyntax{u} \bnfbar \nonpisyntax{\abs{x}{P}} \sbnfbar \nonpisyntax{x,y,z}
			\\[1mm]
			P,Q
			  \bnfis &
			\bout{u}{V}{P}  \sbnfbar  \binp{u}{x}{P} %\sbnfbar			\bsel{u}{l} P \sbnfbar \bbra{u}{l_i:P_i}_{i \in I}  
%			\\[1mm]
			  \sbnfbar  
			  \nonpisyntax{\appl{V}{u}} \sbnfbar  P\Par Q \sbnfbar \news{n} P 
			\sbnfbar \inact \sbnfbar \nonhosyntax{\rvar{X} \sbnfbar \recp{X}{P}}
%			\\%[1mm]
%			 \bnfbar &
%			\nonhosyntax{\rvar{X} \bnfbar \recp{X}{P}}
		\end{align*}
			\end{mdframed}
	\caption{\newjb{Syntax of \HOp. The sub-language \sessp lacks \nonpisyntax{\text{boxed}} constructs, while \HO lacks \nonhosyntax{\text{shaded}} constructs.}}
	\label{top:fig:syntax}
%	\vspace{-1mm}
%	\Hlinefig
%\vspace{-3mm}
\end{figure}
%We start by presenting the \textbf{syntax} of \HOp and its sub-languages \HO and \sessp, as studied in~\cite{DBLP:journals/iandc/KouzapasPY19,KouzapasPY17}. 
\paragraph{Syntax}
\Cref{top:fig:syntax} gives the  {syntax} of processes $P, Q, \dots$, values $V, W, \ldots$, and conventions for names.  Identifiers $a, b, c, \dots$ denote \emph{shared names}, while $s, \dual{s}, \dots $ are used for \emph{session names}. Duality is defined only on session names; this way, $\dual{\dual{s}} = s$, but $\dual{a} = a$. \emph{Names} (shared or sessions) are denoted by $m, n \dots$, and $x, y, z, \dots$ range over variables. 

We write $\widetilde x$ to denote a tuple $(x_1, \dots, x_n)$, and use $\epsilon$ to denote the empty tuple. Given a tuple  $\widetilde x$, we use $|\widetilde x|$ to denote its length. 

%The notations presented so far are common for both \sessp and \HO. Values are simply channel names in \sessp, while in \HO  they can be abstractions and variables. 
An abstraction $\abs{x}{P}$ binds $x$ to its body $P$. In processes, sequencing is specified via prefixes. The \emph{output} prefix, $\bbout{u}{V}P$, sends value $V$ on name $u$, then continues as $P$. Its dual is the \emph{input} prefix, $\binp{u}{x}P$, in which variable $x$ is bound. %Labelled (deterministic) choice consists of \emph{selection} and \emph{branching}, denoted as $\bsel{u}{l}P$ and $\bbra{u}{l_i:P_i}_{i \in I}$.
In the following we shall consider \emph{polyadic} communication, and so we have output and input prefixes of the form $\bbout{u}{\widetilde{V}}P$ and $\binp{u}{\widetilde{x}}P$, respectively.
Parallel composition, $P \Par Q$, reflects the combined behaviour of two processes running simultaneously. Restriction $\news{n}P$ binds the endpoints $n, \dual{n}$ in process $P$. 
Process $\inact$ denotes inaction. 
Recursive variables and recursive processes are denoted $\rvar{X} $ and $\recp{X}{P}$, respectively. 
Replication is denoted by the shorthand notation~$\repl{P}$, which stands for $\recp{X}(P \Par X)$.

%Although not specifically mentioned before, the process calculi used for the scope of this paper are considered polyadic.

The sets of free variables, sessions, and names of a process are denoted $\fv{P}$, $\fs{P}$,  and $\fn{P}$. A process $P$ is \emph{closed} if  $\fv{P} = \emptyset$.
We write  $\bbout{u}{}P$ and $\binp{u}{}P$ when the communication objects are not relevant. Also, we omit trailing occurrences of  $\inact$.


As \Cref{top:fig:syntax} details, the  {sub-languages} \sessp and \HO of \HOp differ as follows:
application $V u$ is only present in \HO; constructs for recursion $\recp{X}{P}$ are present in \sessp but not in \HO. 


\begin{figure}[!t]
\begin{mdframed}[style=alttight]
%\[
%	\begin{array}{rcllcrcll}
	\begin{align*}
		\appl{(\abs{x}{P})}{u}   & \red  P \subst{u}{x} 
		& \orule{App} &
		\\[1mm]
		\bout{n}{V} P \Par \binp{\dual{n}}{x} Q & \red  P \Par Q \subst{V}{x} 
		& \orule{Pass} &
		\\[1mm]
%		\bsel{n}{l_j} Q \Par \bbra{\dual{n}}{l_i : P_i}_{i \in I} & \red  Q \Par P_j ~~(j \in I)~~ 
%		& \orule{Sel} & 
%		\\[1mm]
%		&&
		P \red P'\Rightarrow  \news{n} P   & \red    \news{n} P' 
		& \orule{Res} & 
		\\[1mm]
		P \red P'  \Rightarrow    P \Par Q  & \red   P' \Par Q  
		& \orule{Par} & 
		\\[1mm]
%		&&
		P \scong Q \red Q' \scong P'  \Rightarrow  P  & \red  P'
		& \orule{Cong} &
	\end{align*}
%\]
	\begin{align*}
	&	
		P_1 \Par P_2 \scong P_2 \Par P_1
		\quad
		P_1 \Par (P_2 \Par P_3) \scong (P_1 \Par P_2) \Par P_3
		\\[1mm]
	&	P \Par \inact \scong P
		\quad 
		P \Par \news{n} Q \scong \news{n}(P \Par Q)
		~~ (n \notin \fn{P})
		\\[1mm] 
	&	\news{n} \inact \scong \inact
		\qquad  
		\recp{X}{P} \scong P\subst{\recp{X}{P}}{\rvar{X}}
		\qquad
		P \scong Q \textrm{ if } P \scong_\alpha Q
	\end{align*}
%\vspace{-3mm}
\end{mdframed}
\caption{Reduction Semantics of $\HOp$. 
\vspace{-3mm}
\label{fig:reduction}}
%\Hlinefig
\end{figure}

\paragraph{Reduction Semantics}
  The  {operational semantics} of \HOp, enclosed in \Cref{fig:reduction}, is expressed through a \emph{reduction relation}, denoted $\red$. 
Reduction is closed under \emph{structural congruence}, $\scong$, which identifies equivalent processes from a structural perspective. 
 We write $P\subst{V}{x}$ to denote the capture-avoiding substitution of variable $x$ with value $V$ in $P$. 
 We write `$\{ \}$'     to denote the empty substitution. 
In~\Cref{fig:reduction}, Rule~$\orule{App}$ denotes application, which only concerns names.
Rule~$\orule{Pass}$ defines a shared or session interaction on channel $n$'s endpoints. %Labelled (deterministic) choice is defined by Rule~$\orule{Sel}$. 
The remaining rules are standard.

\thesisalt{
  \paragraph{Labelled Transition System (LTS)}
  \label{top:ss:lts}
  % \subimport{sources/}{untyped-lts.tex}
  \input{untyped-lts.tex}
}{}

\subsection{Session Types for \HOp}
	\begin{figure}[!t]
	\begin{mdframed}%[style=alttight]
				\begin{align*}
						%\textrm{(value)} &
			U \bnfis & C \bnfbar L
			& %\\[1mm]
			%\textrm{(name)} & 
			C \bnfis & S \bnfbar \chtype{S} \bnfbar \chtype{L}
			\\%[1mm]
			%\textrm{(abstractions)}~~ & 
			L \bnfis & \shot{U} \bnfbar \lhot{U}
			& %\\[1mm]		
			%\textrm{(session)} & 
			S \bnfis &  \btout{U} S \bnfbar \btinp{U} S  
			\bnfbar  							
			 \trec{t}{S} \bnfbar \vart{t}  \bnfbar \tinact
			\\%[1mm]					
			% \bnfbar &  \btsel{l_i:S_i}_{i \in I}  \bnfbar \btbra{l_i:S_i}_{i \in I}
			%\\
	%	\end{align*}
%		      \vspace{1em}
      \noalign{\hbox to \textwidth{\leaders\hbox to 3pt{\hss . \hss}\hfil}}
%		      \vspace{1em}
%	\begin{align*}
U  \bnfis	&	\shot{\widetilde{C}} \bnfbar \lhot{\widetilde{C}}
		&
		C   \bnfis &		M  \bnfbar  {\chtype{U}}
\\
		% M  \bnfis  & 
    	% \tinact  \bnfbar  \btout{\widetilde{U}} \tinact \bnfbar 
    % \btinp{\widetilde{U}} \tinact \qquad \qquad  
    % \\
        \mugamma  \bnfis & \tinact \bnfbar \vart{t}
&
    M \bnfis & \mugamma  \bnfbar  \btout{\widetilde{U}} \mugamma 		
    	\bnfbar \btinp{\widetilde{U}} \mugamma \bnfbar \trec{t}{M }	
	%	\\
   % &  \bnfbar \btsel{l_i:M_i}_{i \in I}					\bnfbar \btbra{l_i:M_i}_{i \in I} \\
	\end{align*}
			\end{mdframed}
		\caption{STs for \HOp (top) and MSTs for \HO (bottom). \label{top:f:sts}}
		%\vspace{-5mm}
	\end{figure}
	\Cref{top:f:sts} (top) gives the syntax of types.
Value types $U$ include
the first-order types $C$ and the higher-order
types $L$. Session types are denoted with $S$ and
shared types with $\chtype{S}$ and $\chtype{L}$.
\newc{We write $\Proc$ to denote the \emph{process type}.}
%Note that we dissallow type $\chtype{U}$, thus
%in the type discipline shared names cannot carry shared names.
%In name types, $\chtype{U}$ is shared name types 
%which are sent via shared names. 
\newc{The functional} types $\shot{U}$ and $\lhot{U}$ denote
{\em shared} and {\em linear} higher-order 
%\jpc{functional}
types, respectively.
The {\em output type}
$\btout{U} S$ is assigned to a name that 
first sends a value of
type $U$ and then follows the type described by $S$.  
Dually, $\btinp{U} S$ denotes an {\em input type}. 
%The {\em selection type}
%$\btsel{l_i:S_i}_{i \in I}$ 
%and the 
%{\em branching type}
%$\btbra{l_i:S_i}_{i \in I}$ 
%define labelled choice, \newc{implemented at the level of processes by internal and external choice mechanisms, respectively.}
Type $\tinact$ is the termination type. 
We assume the {\em recursive type} $\trec{t}{S}$ is guarded,
i.e., the type variable $\vart{t}$ only appears under prefixes. 
This way, types such as, 
e.g.,  the type $\trec{t}{\vart{t}}$ are not allowed. 
The sets of free/bound variables of a   type $S$ are defined as usual; 
the sole binder is $\trec{t}{S}$.
Closed session types do not have free type variables.

Session types for \sessp exclude  $L$ from value types $U$ and $\chtype{L}$ from  $C$; session types for \HO exclude $C$ from value types $U$.

We write $S_1 \dualof S_2$ if 
$S_1$ is the \emph{dual} of $S_2$.   
Intuitively, 
duality
converts $!$ into $?$ %and $\oplus$ into $\&$ 
(and vice-versa).
This intuitive definition is enough for our purposes; the formal definition is co-inductive, see~\cite{DBLP:journals/iandc/KouzapasPY19,KouzapasPY17}.
Typing \emph{environments} are defined below:
%\[
\begin{align*}
	\Gamma  & \bnfis  \emptyset \bnfbar \Gamma \cat \varp{x}: \shot{U} \bnfbar \Gamma \cat u: \chtype{S} \bnfbar \Gamma \cat u: \chtype{L} 
        \bnfbar \Gamma \cat \rvar{X}: \Delta 
        \\
	\Lambda &\bnfis  \emptyset \bnfbar \Lambda \cat \AT{x}{\lhot{U}} 
	%\\
	\qquad\qquad
	%\hfill 
	\Delta   \bnfis   \emptyset \bnfbar \Delta \cat \AT{u}{S}
\end{align*}
%]
 $\Gamma$, $\Lambda$, and $\Delta$ satisfy different structural principles.
%Intuitively, the \emph{exchange} principle indicates that the ordering of type assignments does not matter. 
%\emph{Weakening} says that type assignments need not be used. 
%Finally, \emph{contraction}  says that type assignments may be duplicated.}
 $\Gamma$ maps variables and shared names to value types, and recursive 
variables to session environments;  
it admits weakening, contraction, and exchange principles.
While  $\Lambda$ maps variables to 
%the
 linear %functional 
higher-order
types, $\Delta$ maps
session names to session types. 
Both $\Lambda$ and $\Delta$ %behave linearly: they 
are
only subject to exchange.  
%We require that t
The domains of $\Gamma$,
$\Lambda$ and $\Delta$ 
(denoted $\dom{\Gamma}$, $\dom{\Lambda}$, and  $\dom{\Delta}$)
are assumed pairwise distinct. 


Given $\Gamma$, we write $\Gamma \backslash x$ to denote the environment obtained from 
 $\Gamma$ by removing the assignment $x:\shot{U}$, for some $U$.
This notation applies similarly to $\Delta$ and $\Lambda$; 
we write $\Delta \backslash \Delta'$ (and $\Lambda \backslash \Lambda'$) with the expected meaning.
Notation
$\Delta_1\cdot \Delta_2$ means 
the disjoint union of $\Delta_1$ and $\Delta_2$.  
We define \emph{typing judgements} for values $V$
and processes $P$:
%\begin{center}
%\begin{tabular}{c}
	$$\Gamma; \Lambda; \Delta \proves V \hastype U \qquad \qquad \qquad \qquad \qquad \Gamma; \Lambda; \Delta \proves P \hastype \Proc$$
%\end{tabular}
%\end{center}
The judgement on the left
says that under environments $\Gamma$, $\Lambda$, and $\Delta$ value $V$
has type $U$; the  judgement on the right says that under
environments $\Gamma$, $\Lambda$, and $\Delta$ process $P$ has the process type~$\Proc$.
\longversion{The typing rules are presented in Appendix~\ref{top:app:typing}.}{
  The typing rules are presented in \cite{AAP21-full}. 
}


Type soundness   for \HOp  
relies on two auxiliary notions: 
%that contain dual endpoints typed with dual types.
%The following definition ensures two session endpoints 
%are dual each other. 

%\smallskip

\begin{definition}[Session Environments: Balanced/Reduction]\label{top:d:wtenvred}%\rm
	Let $\Delta$ be a session environment.
	\begin{enumerate}[$\bullet$]
	\item  $\Delta$ is {\em balanced} if whenever
	$s: S_1, \dual{s}: S_2 \in \Delta$ then $S_1 \dualof S_2$.
	\item We define  reduction  $\red$ on session environments as: %\\ %[-2mm]
\begin{align*}
	\Delta \cat s: \btout{U} S_1 \cat \dual{s}: \btinp{U} S_2  & \red  
	\Delta \cat s: S_1 \cat \dual{s}: S_2  
%	\\
%	\Delta \cat s: \btsel{l_i: S_i}_{i \in I} \cat \dual{s}: \btbra{l_i: S_i'}_{i \in I} &\red \Delta \cat s: S_k \cat \dual{s}: S_k' \ (k \in I)
\end{align*}
\end{enumerate}
\end{definition}

%We state the type soundness result.
\begin{theorem}[Type Soundness~\cite{KouzapasPY17}]\label{t:sr}%\rm
			Suppose $\Gamma; \es; \Delta \proves P \hastype \Proc$
			with
			$\Delta$ balanced. 
			Then $P \red P'$ implies $\Gamma; \es; \Delta'  \proves P' \hastype \Proc$
			and $\Delta = \Delta'$ or $\Delta \red \Delta'$
			with $\Delta'$ balanced. 
\end{theorem}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \noindent We introduce the type systems of the aforementioned process calculi. We address each session type syntax separately, but provide the set of typing judgements that includes both cases.

% \begin{description}
%     \item[Session Types in \sessp-calculus]
% \end{description}
% \noindent We begin by presenting the notions for \sessp-calculus in Figure~\ref{fig:pi_sess}. A first-order \emph{channel type} $C$ can be a \emph{session} or a \emph{shared type}, denoted $S$ and $\chtype{S}$. The \emph{output type} $\btout{C} S$ sends a channel of type $C$, then proceeds as type $S$. The input type $\btinp{C} S$ is its dual. The \emph{selection} and \emph{branching types} are defined as $\btsel{l_i:S_i}_{i \in I}$ and $ \btbra{l_i:S_i}_{i \in I}$. \emph{Termination} is represented by type $\tinact$. A \emph{recursive type} $\trec{t}{S}$ is required to be guarded, i.e. types of the form $\trec{t}{t}$ are not allowed.\\
% \begin{figure}[!t]
% 	\begin{align*}
% 		C  & \bnfis		S \bnfbar \chtype{S} 
% 		\\ 
% 		S & \bnfis 	\btout{C} S \bnfbar \btinp{C} S \bnfbar \btsel{l_i:S_i}_{i \in I}
% 						\bnfbar \btbra{l_i:S_i}_{i \in I} \bnfbar  \trec{t}{S} \bnfbar \vart{t}  \bnfbar \tinact
% 	\end{align*}
% 	\caption{Syntax of session types for \sessp-calculus.\label{fig:pi_sess}}
% \end{figure}

% \noindent \emph{Environments} represent maps from identifiers to types. In \sessp- calculus, we distinguish between the \emph{shared} environment, $\Gamma$, and the \emph{session} environment, $\Delta$. They are defined as follows:
% $$
% 		\Gamma   \bnfis  \emptyset \bnfbar \Gamma \cat u: \chtype{S} \bnfbar \Gamma, \AT{X}{\Delta}
% 		 \qquad
% 		\Delta  \bnfis   \emptyset \bnfbar \Delta \cat \AT{u}{S}
% $$
% $\Gamma$ maps shared names to shared types and recursive variables to session environments, while $\Delta$ maps session names to session types. The domains of the environments, i.e. $\dom{\Gamma}$ and $\dom{\Delta}$, are assumed to be pairwise distinct. The disjoint union of $\Delta_1$ and $\Delta_2$ is denoted by $\Delta_1, \Delta_2$. The notation $\Gamma\backslash x$ refers to the environment obtained after removing the assignment $x:\chtype{S}$. A similar interpretation follows for $\Gamma \backslash \widetilde x$ and $\Delta \backslash u$. The session environment $\Delta$ is considered \emph{balanced} if whenever $s : S_1, \ \dual{s} : S_2$, then $S_1$ and $S_2$ are dual types. The formal definition of type duality can be found in \cite{HO}. The \emph{typing judgements} for names and processes are the following:  $$\Gamma; \Delta \proves u \hastype C \qquad \text{and} \qquad\Gamma; \Delta \proves P \hastype \Proc$$

% \noindent The first judgement states that name $u$ has type $C$ under environments $\Gamma; \Delta$. The second one is interpreted in the same manner, with $\Proc$ representing a process type.

% \begin{description}
%     \item[Minimal Session Types in \HO calculus]
% \end{description}
% \noindent Although $\HO$ calculus has a more extended type system, our interest lies solely on minimal session types. This is due to the outcome of our decomposition function, i.e. minimally-typed $\HO$ processes. Thus, addressing other information is redundant. \\

% \noindent Figure~\ref{f:MST_HO} contains the syntax of minimal session types, defined in \cite{MinimalSessionTypes}. We comment on the additional notations. The value type $U$ includes the \emph{shared} and \emph{linear higher-order types}, $\shot{\widetilde{C}}$ and $\lhot{\widetilde{C}}$, where $\widetilde C$ denotes a tuple. The \emph{first-order type} $C$ can be either a minimal session type $M$, or a shared value type $\chtype{U}$.
% Remark that the session types in $M$ do not contain sequencing; termination occurs immediately after a tuple is sent or received.
% \begin{figure}[ht]
% 	\begin{align*}
% U & \bnfis		\shot{\widetilde{C}} \bnfbar \lhot{\widetilde{C}}
% 		\\
% 		C  & \bnfis		M  \bnfbar  {\chtype{U}}
% \\
% 		M & \bnfis 	\tinact  \bnfbar  \btout{\widetilde{U}} \tinact \bnfbar \btinp{\widetilde{U}} \tinact \bnfbar \btsel{l_i:M_i}_{i \in I}
% 						\bnfbar \btbra{l_i:M_i}_{i \in I}
% 	\end{align*}
% 	\caption{Syntax of minimal session types for \HO.\label{f:MST_HO}}
% \end{figure}

% \noindent The type system of \HO calculus also involves a \emph{linear} environment: $\Lambda$ maps variables to linear higher-order types. While the $\Delta$ remains unchanged, the $\Gamma$ differs from the shared environment presented above. Variables $x$ and names $n$ are now mapped to shared higher-order and value types, respectively. Here are the environment definitions:
% \begin{align*}
% 		\Gamma  & \bnfis  \emptyset \bnfbar \Gamma \cat \varp{x}: \shot{C} 
% 		%\bnfbar \Gamma \cat u: \chtype{S} 
% 		\bnfbar \Gamma \cat u: \chtype{U}
% 		%\bnfbar \Gamma \cat \rvar{X}: \Delta
% \qquad
% 		\Lambda  \bnfis  \emptyset \bnfbar \Lambda \cat \AT{x}{\lhot{C}}
% 		 \\
% 		\Delta    & \bnfis   \emptyset \bnfbar \Delta \cat \AT{u}{S}
% \end{align*}

% \noindent The set of \emph{typing rules} for both process calculi are presented in Appendix~\ref{appendix}. For their interpretation, the reader should refer to \cite{HO}.

\subsection{Mutual Encodings between \sessp and \HO}
\label{s:encoding}
The encodings $\map{\cdot}^1_g: \sessp \to \HO$
and  $\map{\cdot}^2:  \HO\to\sessp $ are \emph{typed}: each consists of a translation on processes and a translation on types. 
This way, $\tmap{\cdot}{1}$ translates   types for first-order processes into   types for higher-order processes, while $\tmap{\cdot}{2}$ operates in the opposite direction---see Figures~\ref{top:f:enc:hopi_to_ho}
and~\ref{top:f:enc:ho_to_sessp}, respectively.
{Remarkably, these translations on processes and types do not alter their sequentiality.} 
%We briefly discuss these encodings.

% The first encoding is $\map{\cdot}^1: \sessp \to \HO$, presented in Figure~\ref{f:enc:hopi_to_ho}. Its opposing counterpart, the second encoding, is denoted by $\map{\cdot}^2$ and depicted in Figure
% ~\ref{top:f:enc:ho_to_sessp}. Both figures contain the respective type mappings as well, which are used to cast session types into the desired process calculi. So, $\tmap{\cdot}{1}$ maps a first-order session type into a higher-order session type, while $\tmap{\cdot}{2}$ achieves the opposite result. Remarkably, these mappings do not alter the sequentiality property of a process' type; they \emph{preserve minimality}. 
% Hence, by combining them with the type decomposition function defined in \cite{MinimalSessionTypes}, we can obtain a method which translates a first-order process into a minimally-typed first-order process. Let us briefly discuss each figure. \\



\paragraph{From \sessp to \HO}
To mimic the sending of name $w$, the encoding $\map{\cdot}^1_g$  encloses $w$
within the body of an input-guarded abstraction. The corresponding input process
receives this higher-order value, applies it on a restricted session, and sends
the encoded continuation through the session's dual.

Several auxiliary notions are used to encode recursive processes; we describe
them intuitively (see \cite{DBLP:journals/iandc/KouzapasPY19} for full details).
The key idea is to encode recursive processes in \sessp using a ``duplicator''
process in \HO, circumventing linearity by replacing free names with variables.
The parameter $g$ is a map from process variables to sequences of name
variables. Also, $\vmap{{\cdot}}$ maps sequences of session names into sequences
of variables, and $\auxmapp{\cdot}{{}}{\es}$ maps processes with free names to
processes without free names (but with free variables instead).


The encoding \tmap{\cdot}{1} depends on the auxiliary function
$\vtmap{\cdot}{1}$, defined on value types. Following the encoding on processes,
this mapping on values takes a first-order value type and encodes it into a
linear higher-order value type, which encloses an input type that expects to
receive another higher-order type. Notice how the innermost higher-order value
type is either shared or linear, following the nature of the given type. 



\begin{figure}[!t]
\begin{mdframed}%[style=alttight]
\noi{\bf Terms:} 
\begin{align*}
	\map{\bout{u}{w} P}^{1}_ {g}	&\defeq	\!\bout{u}{ \abs{z}{\,\binp{z}{x} (\appl{x}{w})} } \map{P}^{1}_{g}
	\\
	\map{\binp{u}{\AT{x}{C}} Q}^{1}_{g}	&\defeq	\!\binp{u}{y} \newsp{s}{\appl{y}{s} \!\Par\! \bout{\dual{s}}{\abs{x}{\map{Q}^{1}_{g}}} \inact}
	\\
%		\map{\bsel{u}{l} P}^{1}_{g} &\defeq \bsel{u}{l} \map{P}^{1}_{g}
%	\\
%	\map{\bbra{u}{l_i{:}P_i}_{i \in I}}^{1}_{g} &\defeq \!\bbra{u}{l_i: \map{P_i}^{1}_{g}}_{i \in I}
%	\\
		\map{P \Par Q}^{1}_{g} & \defeq \map{P}^{1}_{g} \Par \map{Q}^{1}_{g}
	\\
	\map{\news{n} P}^{1}_{g} &\defeq \!\news{n} \map{P}^{1}_{g}
		\\
	\map{\inact}^{1}_{g} &\defeq \inact \\
  \map{\recp{X}{P}}^{1}_{g} &\defeq
		\newsp{s}{\bbout{\dual{s}}{V} \inact  \Par  \binp{s}{z_\X} \map{P}^{1}_{{g,\{\rvar{X}\to \tilde{n}\}}}}
		\\
    & \qquad  \text{where } (\tilde{n} = \fn{P}) \\
    & \qquad V = \abs{(\vmap{\tilde{n}}, y)} \,{\binp{y}{z_\X} 
    \auxmapp{\map{P}^{1}_{{g,\{\rvar{X}\to \tilde{n}\}}}}{{}}{\es}} \\
    \map{\rvar{X}}^{1}_{g} & \defeq 
		\newsp{s}{\appl{z_X}{(\tilde{n}, s)} \Par \bout{\dual{s}}{ z_X} \inact}  \quad (\tilde{n} = g(\rvar{X}))
%\\
\\[1mm]
\noalign{\bf Types:}
%\begin{align*}
	\vtmap{{S}}{1} & \defeq	\lhot{(\btinp{\lhot{\tmap{S}{1}}} \tinact)}
	\\ 
	\vtmap{\chtype{S}}{1} & \defeq	\lhot{(\btinp{\shot{\chtype{\tmap{S}{1}}}} \tinact)}
	\\[1mm]
	\tmap{\btout{U} S}{1} & \defeq \btout{{\vtmap{U}{1}}} \tmap{S}{1}
	\\
	\tmap{\btinp{U} S}{1} & \defeq\btinp{{\vtmap{U}{1}}} \tmap{S}{1}
	\\
%	\tmap{\btsel{l_i: S_i}_{i \in I}}{1} & \defeq \btsel{l_i: \tmap{S_i}{1}}_{i \in I}
%	\\
%	\tmap{\btbra{l_i: S_i}_{i \in I}}{1} & \defeq \btbra{l_i: \tmap{S_i}{1}}_{i \in I}
%	\\
	\tmap{\chtype{S}}{1} & \defeq	\chtype{\tmap{S}{1}} 
		\qquad \quad 
		\tmap{\trec{t}{S}}{1}   \defeq \trec{t}{\tmap{S}{1}}
	\\
		\tmap{\tinact}{1}  & \defeq  \tinact
		\qquad \qquad \quad 
		\tmap{\vart{t}}{1}  \defeq \vart{t}
%    \\
%    \tmap{\trec{t}{S}}{1}  & \defeq \trec{t}{\tmap{S}{1}} \\
%    \tmap{\vart{t}}{1} & \defeq \vart{t} 
  \end{align*}
\end{mdframed}
%
%\vspace{-1mm}
\caption{\label{top:f:enc:hopi_to_ho}Typed encoding of \sessp into \HO, selection from \cite{DBLP:journals/iandc/KouzapasPY19}. 
Above,
$\fn{P}$ is a lexicographically ordered sequence  of free names in $P$.
\longversion{Maps $\vmap{\cdot}$ and 
$\auxmapp{\cdot}{{}}{\sigma}$ are in 
\defref{top:d:auxmap} and \Cref{top:f:auxmap}.}{
  Maps $\vmap{\cdot}$ and 
  $\auxmapp{\cdot}{{}}{\sigma}$ can be found in \cite{AAP21-full}. 
}
} 
%While $\map{\cdot}^{1}_{g}$ encodes processes,  \tmap{\cdot}{1} encodes session types.
% }
%\vspace{-1mm}
%(cf.~\defref{d:enc:fotohorec}).
%Mappings 
%$\map{\cdot}^2$,
%$\mapt{\cdot}^2$, 
%and 
%$\mapa{\cdot}^2$
%are homomorphisms for the other processes/types/labels. 
%\Hlinefig
%\vspace{-4mm}
\end{figure}

\paragraph{From \HO to \sessp}
%\todo[]{Shouldn't this be "Back to \sessp from \HO"?}
The encoding $\map{\cdot}^2$ simulates higher-order communication using first-order constructs, following  Sangiorgi~\cite{SangiorgiD:expmpa}. The idea is to use \emph{trigger names}, which point towards copies of input-guarded server processes that should be activated. 
The encoding of abstraction sending distinguishes two cases: if the abstraction body does not contain any free session names (which are linear), then the server can be  replicated. 
Otherwise, if the value contains session names then its corresponding server name must be used exactly once. 
The encoding of abstraction receiving proceeds inductively, noticing that the variable is now a placeholder for a first-order name. 
The encoding of application is also in two cases; both of them depend on the creation of a fresh session, which is used to pass around the applied name. 
%The encoding on types $\tmap{\cdot}{2}$  maps a higher-order value type  to a shared, first-order input value type. 

\begin{figure}[!t]
\begin{mdframed}
{\bf Terms:} 
\begin{align*}
	 \map{\bout{u}{\abs{x}{Q}} P}^{2}  & \defeq  
	\begin{cases}
		\newsp{a}{\bout{u}{a} (\map{P}^{2} \Par \repl{\binp{a}{y} \binp{y}{x} \map{Q}^{2}})}
		& \text{if $\fs{Q} = \emptyset$}
		\\ 
		& \text{~with  $*P = \recp{X}{(P \Par \rvar{X})}$}
		\\
		\newsp{a}{\bout{u}{a} (\map{P}^{2} \Par \binp{a}{y} \binp{y}{x} \map{Q}^{2})}
		& \text{otherwise} %\dk{Q \textrm{ linear}} \\
	\end{cases}
\\
	 \map{\binp{u}{x} P}^{2} & \defeq  \binp{u}{x} \map{P}^{2}
	%\quad \quad \pmap{\appl{(\abs{x}{P})}{u}}{2} \!\! \defeq \!\! \pmap{P\subst{u}{x}}{2}
	 \\
	 \map{\appl{x}{u}}^{2} & \defeq \newsp{s}{\bout{x}{s} \bout{\dual{s}}{u} \inact}
	\\
	 \map{\appl{(\abs{x}{P})}{u}}^{2}  & \defeq  %\newsp{s}{\bout{a}{s} \bout{\dual{s}}{u} \inact} \\
	\newsp{s}{\binp{s}{x} \map{P}^{2} \Par \bout{\dual{s}}{u} \inact}
 % \\
%  \qquad \quad \text{where: $*P = \recp{X}{(P \Par \rvar{X})}$}
\end{align*}
{\bf Types:}
\begin{align*}
		\tmap{\btout{\lhot{S}}S_1}{2} & \defeq \bbtout{\chtype{\btinp{\tmap{S}{2}}\tinact}}\tmap{S_1}{2}
		\\
		\tmap{\btinp{\lhot{S}}S_1}{2} & \defeq \bbtinp{\chtype{\btinp{\tmap{S}{2}}\tinact}}\tmap{S_1}{2}
%\noindent{\bf Labels:}\ 
%		\mapa{(\nu \tilde{m})\bactout{n}{\abs{ x}{P}} }^2  & \defeq & \news{m} \bactout{n}{m} \\
%		\mapa{\bactinp{n}{\abs{ x}{P}} }^2 &  \defeq & \bactinp{n}{m}
%\quad \quad m \text{ fresh}
%\\[1mm]
%\hline
\end{align*}
\end{mdframed}

\caption{Typed encoding of \HO into \sessp~\cite{DBLP:journals/iandc/KouzapasPY19}. 
% {Here, $*P$ stands for $$}
%While $\map{\cdot}^2$ translates processes, \tmap{\cdot}{2} encodes types. 
\label{top:f:enc:ho_to_sessp}
}
%\vspace{-1mm}
%\Hlinefig
\vspace{-4mm}
\end{figure}

% \thesisalt{
%   \subsection{Labelled Transition System for Processes}
%   \label{top:ss:lts}
%   % \subimport{sources/}{untyped-lts.tex}
%   \input{untyped-lts.tex}
% }{}

\subsection{Minimal Session Types for \HO}
The syntax of \msts for \HO  is in \Cref{top:f:sts} (bottom).
We write \mHO to denote \HO with \msts.
	The decomposition $\D{\cdot}$ in~\cite{APV19} relies crucially on the ability of communicating tuples of values.
Hence, value types are of the form $\shot{\widetilde{C}}$ and $\lhot{\widetilde{C}}$. Similarly, minimal session types for output and input are of the form $\btout{\widetilde{U}} \tinact$ and $\btinp{\widetilde{U}}\tinact$: they communicate tuples of values but lack a continuation.

 Following Parrow~\cite{DBLP:conf/birthday/Parrow00}, $\D{\cdot}$   is defined in terms of a \emph{breakdown function} $\B{k}{\tilde x}{\cdot}$, which translates a process into a composition of \emph{trios processes} (or simply \emph{trios}).
A {trio} is a process with exactly three nested prefixes.
If $P$ is a sequential process with $k$ nested actions, then $\D{P}$ will contain $k$  trios running in parallel: each trio in $\D{P}$ will enact exactly one prefix from $P$; the breakdown function must be carefully designed to ensure that trios trigger each other in such a way that $\D{P}$ preserves the prefix sequencing in $P$.
While trios decompositions elegantly induce processes typable with \msts, they are not goal in themselves; rather, they offer one possible path to better understand sequentiality in session types.

We use  some useful terminology for trios~\cite{DBLP:conf/birthday/Parrow00}.
The \textit{context} of a trio is a tuple of variables $\widetilde x$, possibly empty, which  makes variable bindings explicit.
We use a reserved set of \textit{propagator names} (or simply \emph{propagators}), denoted by $\prop_k, \prop_{k+1}, \ldots$, to carry contexts and trigger the
subsequent trio.
Propagators with recursive types are denoted by $\prop_k^r, \prop_{k+1}^r, \ldots$.
We say that  a \emph{leading trio} is the one that receives a context, performs an action, and triggers the next trio;
 a \emph{control trio} only activates other trios.

The breakdown function works on both processes and values.
The breakdown of process $P$ is denoted by $\B{k}{\tilde x}{P}$, where $k$ is the
index for the propagators $\prop_k$, and $\widetilde x$ is the context to be received by the previous trio.
Similarly,
the breakdown  of a value $V$ is denoted by
$\V{k}{\tilde x}{V}$. 
\Cref{mst:t:bdowncore-ho} gives the breakdown function defined in \cite{APV19} for the sub-language of \HO without recursion---this is the so-called \emph{core fragment}.
In the figure, we include side conditions that use the one-line conditional
$
x = \linecondit{c}{s_1}{s_2}
$
to express that $x = s_1$ if condition $c$ is true, and $x = s_2$ otherwise.
Notice that for session types we have either $C = S$ or $C = \chtype{S}$.
 
To formally define $\D{\cdot}$ in terms of $\B{k}{\tilde x}{\cdot}$, we need some notation. 
Let $\widetilde u = (a,b,s,s',\ldots)$ be a finite tuple of names.
We shall write $\mathsf{init}(\widetilde u)$ to denote the tuple
$(a_1,b_1,s_1,s'_1,\ldots)$.
We say that a process has been \emph{initialized} if all of its names have some index.

\begin{table}[!t]
 \input{ho-decomp-table.tex}
  \caption{The breakdown function for \HO processes and values (core fragment from \cite{APV19}). \label{mst:t:bdowncore-ho}}
  \end{table}

  \begin{comment} 
\begin{table*}
  \begin{tabular}{ |l|l|l|}
    \rowcolor{gray!25}
    \hline
    $P$ &
      \multicolumn{2}{l|}{
    \begin{tabular}{l}
      \noalign{\smallskip}
      $\B{k}{\tilde x}{P}$
      \smallskip
    \end{tabular}
  }  \\
    \hline
  $\bout{u_i}{V}{Q}$ &
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\propinp{k}{\widetilde x}
        \bbout{u_i}{\widehat{V}}
        \apropout{k+l+1}{\widetilde z}   \Par \B{k+\degree+1}{\tilde z}{Q\sigma}$
       \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{ll}
      \noalign{\smallskip}
      $\widehat{V} = \V{k+1}{\tilde y}{V\sigma}$ & \\
      $\widetilde y = \fv{V}$ & 
      $\widetilde z = \fv{Q}$ \\
      $\degree = \len{V}$ & 
      $\sigma = \nextn{u_i}$ 
      \smallskip
    \end{tabular}
    \\
  \hline 
  $\binp{u_i}{y}Q$
  &
    \begin{tabular}{l}
        \noalign{\smallskip}
        $\propinp{k}{\widetilde x}\binp{u_i}{y} \apropout{k+1}{\widetilde x'} \Par \B{k+1}{\tilde x'}{Q\sigma}$
        \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{l}
      \noalign{\smallskip}
    $\widetilde x' = \fv{Q} $ \\
      % $\sigma = \begin{cases}
      % \incrname{u}{i} & \text{if } u_i:S \\
      % \{\} & \text{otherwise}
      % \end{cases}$
      $\sigma = \nextn{u_i}$
      \smallskip
    \end{tabular}
      \\
    \hline
      $\appl{V}{u_i}$ &
    \begin{tabular}{l}
      \noalign{\smallskip}
      $\propinp{k}{\widetilde x}\appl{\V{k+1}{\tilde x}{V}}{\widetilde m}$
      \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{ll}
      \noalign{\smallskip}
      $u_i:C$ &
       $\widetilde{m} = (u_i,\ldots,u_{i+\len{\Gt{C}}-1})$  \\
      $\widetilde x = \fv{V}$ & 
      \smallskip
    \end{tabular}
    \\
    \hline

    $\news{s:C}{P'}$ &
    \begin{tabular}{l}
      \noalign{\smallskip}
     $\news{\widetilde{s}:\Gt{C}}{\,\B{k}{\tilde x}
         {P'\sigma}}$
      \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{ll}
      \noalign{\smallskip}
      $\widetilde{s} = (s_1,\ldots,s_{\len{\Gt{C}}})$ & \\
%      $\sigma = \linecondit{a}{b}{c}$
      $\sigma =\linecondit{C = S}{\subst{s_1 \dual{s_1}}{s \dual{s}}}{\subst{s_1}{s}}$ &  $\widetilde x = \fv{P'}$ 
%    $\sigma = \begin{cases}
%          \subst{s_1 \dual{s_1}}{s \dual{s}} & \text{if} \ C = S \\
%          \subst{s_1}{s} & \text{if} \ C = \chtype{U}
%  \end{cases}
%  $
      \smallskip
    \end{tabular}
    \\
    \hline
    $Q \Par R$ &
    \begin{tabular}{l}
      \noalign{\smallskip}
      $\propinp{k}{\widetilde x} \propout{k+1}{\wtd y}
      \apropout{k+\degree+1}{\wtd z} \Par$ \\ 
      $\B{k+1}{\tilde y}{Q} \Par \B{k+\degree+1}{\tilde z}{R}$
      \smallskip
    \end{tabular}
    &
    %side-conditions
    \begin{tabular}{lll}
      \noalign{\smallskip}
      $\widetilde y  = \fv{Q}$ &
      $\widetilde z = \fv{R}$ &
      $\degree = \len{Q}$ 
      \smallskip
    \end{tabular}
        \\
    \hline
    $\inact$ &
  \begin{tabular}{l}
    \noalign{\smallskip}
    $\propinp{k}{}\inact$
   \smallskip
  \end{tabular}
  &
  \begin{tabular}{l}
    \noalign{\smallskip}
  \smallskip
  \end{tabular}
    \\
    \hline
  \rowcolor{gray!25}
  $V$ &
    \multicolumn{2}{l|}{
  \begin{tabular}{l}
    \noalign{\smallskip}
    $\V{k}{\tilde x}{V}$
    \smallskip
  \end{tabular} } 
  \\
  \hline
  $y$ &
  \begin{tabular}{l}
    \noalign{\smallskip}
    $y$
    \smallskip
  \end{tabular}
  &
  %side-conditions\\
  \begin{tabular}{l}
    \noalign{\smallskip}
    \smallskip
  \end{tabular}
  \\
  \hline
  $\abs{u:\slhotup{C}}P$ &
  \begin{tabular}{l}
    \noalign{\smallskip}
    \begin{tabular}{l}
    $%\abs{\widetilde{y}:{\slhotup{\Gt{C}}}}
    \abs{\widetilde{y}}
    {\news{\widetilde \prop}\big(\apropout{k}{\widetilde x}
      \Par \B{k}{\tilde x}{P \subst{y_1}{y}}}\big)$
     \end{tabular}
    \smallskip
%    \\
%    $\widetilde{\prop} = \begin{cases} 
%          \epsilon & \text{if} \ \leadsto = \multimap \\
%       (\prop_k,\ldots,\prop_{k+\len{P}-1}) & \text{if} \ \leadsto = \rightarrow
%   \end{cases}$ 
%    \smallskip
  \end{tabular}
  &
  %side-conditions\\
  \begin{tabular}{l}
    \noalign{\smallskip}
    $\widetilde x = \fv{V}$ \\
    $\widetilde{y} = (y_1,\ldots,y_{\len{\Gt{C}}})$ 
    \\
    $\widetilde{c} = \linecondit{\leadsto = \rightarrow}{(\prop_k,\ldots,\prop_{k+\len{P}-1})}{\epsilon}$
  \end{tabular}
  \\
  \hline
  \end{tabular}
  \caption{The breakdown function for \HO processes and values (core fragment from \cite{APV19}). \label{mst:t:bdowncore-ho}}
  \end{table*}
  %\end{center}
\end{comment} 


\begin{definition}[Decomposing Session Types] 
  \label{mst:def:typesdecomp}
  Given the session, higher-order, and shared types of \Cref{top:f:sts}, the \emph{type decomposition function}  $\Gt{-}$ is defined using the auxiliary function $\Rt{-}$ as in \Cref{mst:fig:typesdecomp}. 
We write $\len{\Gt{S}}$ to denote the length of  $\Gt{S}$ (and similarly for $\Rt{-}$).
\end{definition}


\begin{figure}[!t]
\begin{mdframed}
\vspace{-4mm}
	\begin{align*}
  \Gt{\btout{U}{S}} &=
  \begin{cases}
  \btoutt{\Gt{U}}   &  \text{if $S = \tinact$} \\
  \btoutt{\Gt{U}}\, ,\Gt{S} & \text{otherwise}  
\end{cases} 
 \\
 \Gt{\btinp{U}{S}} &=
  \begin{cases}
  \btinpt{\Gt{U}}  &  \text{if $S = \tinact$} \\
  \btinpt{\Gt{U}} \, , \Gt{S} & \text{otherwise}
  \end{cases}   
  \\
  \Gt{\trec{t}{S}} & = 
  \begin{cases} 	
    \Rt{S} & \text{if $\tr(\trec{t}{S})$} \\ 
    \trec{t}{\Gt{S}} & \text{if $\neg\tr(\trec{t}{S})$ and $\Gt{S}$ is a singleton}
 \end{cases} 
 \\
  \Gt{\tinact} &= \tinact 
  \\
   \Gt{\vart{t}} & = \vart{t} 
  \\
  \Gt{\lhot{C}} &= \lhot{\Gt{C}} 
  \\
  \Gt{\shot{C}} &= \shot{\Gt{C}}
  \\
  % \Gt{S_1,\ldots,S_n} &=
  % \Gt{S_1},\ldots,\Gt{S_n} 
  % \\
    \Gt{\chtype{U}} &= \chtype{\Gt{U}}
   \\
   \Rt{\vart{t}} & = \epsilon
  \\
    \Rt{\btout{U}S} &= \trec{t}{\btout{\Gt{U}}} \tvar{t}, \Rt{S}
   \\
   \Rt{\btinp{U}S} & = \trec{t}{\btinp{\Gt{U}}} \tvar{t}, \Rt{S} 
  % & 
  % \Rt{\btout{U}S} = \trec{t}{\btout{\Gt{U}}} \tvar{t}, \Rt{S}
  % \Rt{\btinp{U}S} = \trec{t}{\btinp{\Gt{U}}} \tvar{t}, \Rt{S} 
  % \\ 
  % \Rts{}{s}{\btinp{U}S} &= \Rts{}{s}{S}
  % \\
  % \Rts{}{s}{\btout{U}S} &= \Rts{}{s}{S}
\end{align*}
\end{mdframed}	
\caption[Decomposing session types into minimal session types.]{Decomposing session types into minimal session types (\Cref{mst:def:typesdecomp})   \label{mst:fig:typesdecomp}}
\end{figure}

\begin{newaddenv}
  Given an unfolded recursive session type $S$, the auxiliary function $\indT{S}$ returns the position of the top-most prefix of $S$ within its body.
  \begin{definition}[Index function]
  \label{mst:def:indexfunction}
  Let $S$ be an (unfolded) recursive session type. The function $\indT{S}$ is defined as follows:  
  \begin{align*}
    \indT{S} = \begin{cases}
     \indTaux{S'\subst{S}{\vart{t}}}{0} & \text{if} \ S =\trec{t}{S'} \\
     \indTaux{S}{0} & \text{otherwise}
   \end{cases}
   \qquad
   \indTaux{T}{l} = \begin{cases}
   	\len{\Rt{S}} - l + 1 & \text{if $T=\trec{t}{S}$}
   	\\
   		\indTaux{S}{l+1} & \text{if $T=\btout{U}S$ or $T=\btinp{U}S$}
   \end{cases}
  \end{align*}
%  \noindent where $ \indTaux{S}{l}$:
%  \begin{align*}
%  \indTaux{\trec{t}{S}}{l} & = \len{\Rt{S}} - l + 1
%    \\
% \indTaux{\btout{U}S}{l}  & = \indTaux{S}{l+1}
%  \\
%   \indTaux{\btinp{U}S}{l} & = \indTaux{S}{l+1}
%  \end{align*}
  \end{definition}
\end{newaddenv}

\begin{definition}[Decomposing Processes~\cite{APV19}]
  \label{mst:def:hodecomp}
  \label{mst:def:decomp}
	Let $P$ be a closed \HO process such that $\widetilde u = \fn{P}$.
  The \emph{decomposition} of $P$, denoted $\D{P}$, is
defined as:
  $$
  \D{P} = \news{\widetilde \prop}\big(\propout{k}{} \inact \Par \B{k}{\epsilon}{P\sigma}\big)
  $$
  where:
  $k > 0$;
  $\widetilde \prop = (\prop_k,\ldots,\prop_{k+\len{P}-1})$;
  $\sigma = \subst{\mathsf{init}(\tilde u)}{\widetilde u}$;
  and
  the  {breakdown function} $\B{k}{\tilde x}{\cdot}$, %where $\widetilde{x}$ is a tuple of variables, 
  is as defined  in Table~\ref{mst:t:bdowncore-ho}.
  \end{definition}

% \todo[inline]{We need to recall the decomposition of types from ECOOP (core fragment is enough)}


% \begin{definition}[Decomposing Session Types] 
%   \label{top:def:ho-typesdecomp}
% %  Let $S$ be a session type, $U$ be a higher-order type, $C$ be a name type, and
% %  $\chtype{U}$ be a shared type, all as in \Cref{f:sts}. 
%    The \emph{decomposition function} on the types of \Cref{top:f:sts}, denoted $\Gt{\cdot}$, is defined in 
%    \Cref{top:f:def:ho-typesdecomp}.
      
%    \begin{figure}
%    \begin{mdframed}[style=alttight]
%   \begin{align*}
%     \Gt{\btout{U}{S}} &=
%     \begin{cases}
%     \btout{\Gt{U}}{\tinact}  &  \text{if $S = \tinact$} \\
%     \btout{\Gt{U}}{\tinact}\, ,\Gt{S} & \text{otherwise}
%     \end{cases} \\
%     \Gt{\btinp{U}{S}} &=
%     \begin{cases}
%     \btinp{\Gt{U}}{\tinact}  &  \text{if $S = \tinact$} \\
%     \btinp{\Gt{U}}{\tinact}\, , \Gt{S} & \text{otherwise}
%     \end{cases} \\
% %      \Gt{\tinact} &= \tinact \\
%     \Gt{\lhot{C}} &= \lhot{\Gt{C}} \quad   \Gt{\tinact} = \tinact \\ 
%     \Gt{\shot{C}} &= \shot{\Gt{C}}  \quad \Gt{\chtype{U}} = \chtype{\Gt{U}}\\ 
%    % \Gt{\chtype{U}} &= \chtype{\Gt{U}}\\
%     \Gt{S_1,\ldots,S_n} &=
%     \Gt{S_1},\ldots,\Gt{S_n}
%   \end{align*}
%      \end{mdframed}	
%      \caption{Decomposition of types (cf. \defref{top:def:ho-typesdecomp})}
% \label{top:f:def:ho-typesdecomp}
%    \end{figure}
%   \end{definition}




As already mentioned, the \emph{minimality result}  in \cite{APV19} is that if $P$ is a well-typed \HO process then $\D{P}$ is a well-typed \mHO process. It attests that the sequentiality in the session types for $P$ is appropriately accommodated by the decomposition $\D{P}$. Its proof relies on an auxiliary result establishing the typability of $\B{k}{\tilde x}{P}$. 

%\begin{theorem}[Typability of Breakdown (Excerpt from~\cite{APV19})]
%  \label{t:typecore}
%     Let $P$ be an initialized process. % and $V$ be a value.
%    \begin{enumerate}
%    \item
%    If $\Gamma;\Lambda;\Delta \proves P \hastype \Proc$ then
%    $$\Gt{\Gamma_1};\es;\Gt{\Delta} \cat
%    \Theta \proves \B{k}{\tilde x}{P} \hastype \Proc 
%    \quad 
%    (k > 0)
%    $$ where:
%     $\widetilde x = \fv{P}$;
%     $\Gamma_1=\Gamma \setminus \widetilde x$;
%     and
%     $\balan{\Theta}$ with
%      $\text{dom}(\Theta) = \{\prop_k,\prop_{k+1},\ldots,\prop_{k+\len{P}-1}\} \cup \{\dual{\prop_{k+1}},\ldots,\dual{\prop_{k+\len{P}-1}}\}$ and $\Theta(\prop_k)=
%    \btinp{\widetilde M} \tinact$,
%    where $\widetilde M = (\Gt{\Gamma}\cat\Gt{\Lambda})(\widetilde x)$.
%  
%%    \item If $\Gamma;\Lambda;\Delta \proves V \hastype \lhot{C}$ then
%%    $$\Gt{\Gamma};\Gt{\Lambda};\Gt{\Delta} \cat \Theta \proves \V{k}{\tilde
%%    x}{V} \hastype \lhot{\Gt{C}}
%%      \quad 
%%    (k > 0)
%%    $$ where:
%%    $\widetilde x = \fv{V}$;
%%  %  $k > 0$;
%%    and $\balan{\Theta}$ with
%%    $$\text{dom}(\Theta) =  \{\prop_k,\ldots,\prop_{k+\len{V}-1}\}
%%     \cup \{\dual{\prop_{k}},\ldots,\dual{\prop_{k+\len{V}-1}}\}$$
%%    and $\Theta(\prop_k)= \btinp{\widetilde M} \tinact$
%%    and $\Theta(\dual{\prop_k})= \btout{\widetilde M} \tinact$,
%%    where $\widetilde M = (\Gt{\Gamma}\cat\Gt{\Lambda})(\widetilde x)$.
%%  
%%    \item If $\Gamma;\es;\es \proves V \hastype \shot{C}$ then
%%    $\Gt{\Gamma};\es;\es \proves \V{k}{\tilde x}{V} \hastype \shot{\Gt{C}}$, where $\widetilde x = \fv{V}$
%%    and $k > 0$.
%%  
%  \end{enumerate}
%  \end{theorem}
%
%
%Using the above theorem, we then have:

% \begin{newaddenv}
  
\begin{restatable}[Typability of $\B{\text{-}}{\text{-}}{\text{-}}$~\cite{APV19}]{lemm}{typerec}
  \label{mst:t:typecore}
  Let $P$ be an indexed \HO process and $V$ be a value.
  \begin{enumerate}
  \item
  If $\Gamma;\Lambda;\Delta \circ  \envR \proves P \hastype \Proc$ then
  $\Gt{\Gamma_1}\cat \envPropR;\es;\Gt{\Delta} \cat \Theta \proves \B{k}{\tilde x}{P} \hastype \Proc$, 
  where: 
  \begin{itemize}
  \item $k > 0$
  \item $\widetilde r = \text{dom}(\envR)$
  \item $\envPropR = \prod_{r \in \tilde r} c^r:\chtype{\lhot{\Rts{}{s}{\envR(r )}}}$
  \item $\widetilde x = \fv{P}$ 
  \item $\Gamma_1=\Gamma \setminus \widetilde x$ 
  \item $\text{dom}(\Theta) =
  \{\prop_k,\ldots,\prop_{k+\plen{P}-1}\} \cup
  \{\dual{\prop_{k+1}},\ldots,\dual{\prop_{k+\plen{P}-1}}\}$
  \item $\Theta(\prop_k)=
  \btinpt{U_1, \ldots, U_n} $, where $(\Gt{\Gamma}\cat\Gt{\Lambda})(\widetilde x) = (x_1 : U_1, \ldots, x_n : U_n)$
  \item $\balan{\Theta}$
  \end{itemize}

  \item If $\Gamma;\Lambda;\Delta \circ  \envR \proves V \hastype 
  \lhot{\wtd T}$ then
  $\Gt{\Gamma} \cat \envPropR; \Gt{\Lambda};\Gt{\Delta} \proves 
  \V{k}{\tilde x}{V} \hastype \lhot{\Gt{\wtd T}}$, 
  where: 
  \begin{itemize}
  	\item 
$\wtd x = \fv{V}$ 
\item 
  $\envPropR = \prod_{r \in \tilde r} c^r:\chtype{\lhot{\Rts{}{s}{\envR(r)}}}$
    \end{itemize}

\end{enumerate}
\end{restatable} 
% \end{newaddenv}

% \begin{theorem}[Minimality Result~\cite{APV19}]
% \label{t:decompcore}
% 	Let $P$ be a closed \HO process with $\widetilde u = \fn{P}$ and
% 	$\sigma = \subst{\mathsf{init}(\widetilde u)}{\widetilde u}$.
% 	If $\Gamma;\es;\Delta \proves P \hastype \Proc$ then
% 	$$\Gt{\Gamma \sigma};\es;\Gt{\Delta \sigma} \proves \D{P} \hastype \Proc$$
% \end{theorem}

\begin{restatable}[Minimality Result~\cite{APV19}]{theorem}{decompcore}
  \label{mst:t:decompcore}
	Let $P$ be a closed \HO process (i.e. $\fv{P} = \emptyset$) with $\widetilde u = \fn{P}$.
  % and $\widetilde v
	% = \rfn{P}$. 
	% \\
	If $\Gamma;\es;\Delta \circ  \envR \proves P \hastype \Proc$, 
	%where $\envR$ only involves recursive session types,  
	then $\Gt{\Gamma
	\sigma};\es;\Gt{\Delta\sigma}  \cat \Gt{\envR \sigma} \proves \D{P} \hastype
	\Proc$, where $\sigma = \subst{\mathsf{init}(\widetilde u)}{\widetilde u}$.
\end{restatable}

Having summarized the results on which our developments stand, we now move on to establish the minimality result but for \sessp. 
%We shall follow \cite{APV19} in first defining a breakdown function and then defining a decomposition function for \sessp processes.



==> sources/rec-aux.tex <==
\begin{restatable}[]{lemm}{}
	\label{lem:indexcor}
	Let $\widetilde r$ be tuple of channel names and $S$ a recursive 	session type.
	If $\widetilde r : \Rtsopt{}{s}{\btout{C}S}$ and $k = f(\btout{C}S)$
	then $r_k:\trec{t}\btout{\Gt{C}}\vart{t}$.
\end{restatable}

==> sources/type_system_lt.tex <==
\begin{figure}[t!]
\begin{mdframed}
\[
	\begin{array}{c}
		\inferrule[(T$\pi$-var)]
		{\texttt{un}{(\Gamma)}}
		{\Gamma;x:\tau \proveslt x : \tau}
		\qquad 
		\inferrule[(T$\pi$-val)]
		{\texttt{un}{(\Gamma)}}
		{\Gamma \proveslt \star : \mathtt{Unit}}
		\qquad 
		\inferrule[(T$\pi$-inact)]
		{\texttt{un}{(\Gamma)}}
		{\Gamma \proveslt \inact}
		\vspace*{0.5cm}
		\\ 
		\inferrule[(T$\pi$-par)]
		{\Gamma_1 \proveslt P \quad \Gamma_2 \proveslt Q} 
		{\Gamma_1 \uplus \Gamma_2 \proveslt P \Par Q}
		\qquad 
		\inferrule[(T$\pi$-res1)]
		{\Gamma, x:\ltab{\tilde \tau} \proveslt P}
		{\Gamma \proveslt \news{x} P}
		\qquad 
		\inferrule[(T$\pi$-res2)]
		{\Gamma, x:\ltend \proveslt P}
		{\Gamma \proveslt \news{x} P}
		\vspace*{0.5cm}
		\\
		\inferrule[(T$\pi$-Inp)]{
		\Gamma_1 \proveslt x : \lti{\wtd \tau}
		\quad 
		\Gamma_2, \tilde y : \wtd \tau \proveslt P}
		{\Gamma_1 \uplus \Gamma_2 \proveslt \binp{x}{\tilde y}P}
		\qquad 
		\inferrule[(T$\pi$-Out)]{
		\Gamma_1 \proveslt x : \lto{\wtd \tau}
		\qquad 
		\wtd \Gamma_2 \proveslt \tilde v : \wtd \tau 
		\quad 
		\Gamma_3  \proveslt P}
		{\Gamma_1 \uplus \wtd \Gamma_2 \uplus \Gamma_3 
		\proveslt \bout{x}{\tilde v}P}
		\vspace*{0.5cm}
		\\
		\inferrule[(T$\pi$-LVal)]
		{\Gamma \proveslt v : \tau_j 
		\quad
		j \in I}
		{\Gamma \proveslt l_j\_v : \ltbra}
		\qquad 
		\inferrule[(T$\pi$-Case)]
		{\Gamma_1 \proveslt v :  \ltbra
		\quad \Gamma_2, x_i:\tau_i \proveslt P_i
		\quad 
		\forall i \in I} 
		{\Gamma_1 \uplus \Gamma_2 \proveslt 
		\ltcase{v}{l_i}{x_i}{P_i}{i \in I}
		% \textbf{case} \ v \ \textbf{of}
		% \ \{l_i\_(x_i) \triangleright P_i\}_{i \in I}
		}
		\end{array}
\]
\end{mdframed}
%\vspace{-3mm}
\caption{Typing Rules for linearly-typed $\pi$.
%See \appref{app:types} for a full account.
\label{top:fig:typeslinear}}
%\Hline
%\vspace{-1mm}
\end{figure}
%\myparagraph{Typing System of \HOp}


% \begin{remark} We derive polyadic rules for typing \sessp as an 
% 	expected extension of \sessp typing rules in~\Cref{top:fig:typerulesmyspoly}.  
% 	\begin{figure}[t!]
% 		\begin{mdframed}
% 	\[
% 		\begin{array}{c}
% 			\inferrule[(PolyVar)]{}{\Gamma \cat \wtd x : \wtd M_x;\wtd y : \wtd M_y \proves 
% 			\wtd x \wtd y \hastype \wtd M_x \wtd M_y} \\[4mm]
% 	%		~~\inferrule[(Sh)]{}{\Gamma \cat u:C;\es \proves u \hastype C}
% 	%		\\[4mm]
% 	%		\inferrule[(RVar)]{}
% 	%		{\Gamma \cdot X : \Delta;\Delta \proves X \hastype \Proc}
% 	%		~~\inferrule[(Nil)]
% 	%		{}
% 	%		{\Gamma;\emptyset \proves \inact \hastype \Proc}
% 	%		~~\inferrule[(Rec)]
% 	%		{\Gamma \cdot X : \Delta;\Delta \proves P \hastype \Proc}
% 	%		{\Gamma;\Delta \proves \recp{X}P \hastype \Proc}
% 	%		\\[4mm]
% 			\inferrule[(PolySend)]{
% 					%	\begin{array}{c}
% 	%					u:S \in \Delta_1 
% 	%					\quad
% 				\Gamma; \Delta_1 \cat u:S \proves P \hastype \Proc
% 				\quad
% 				\Gamma; \Delta_2 \proves \wtd x \hastype \wtd C
% 				%\end{array}
% 			}{
% 				\Gamma; \Delta_1 \cat \Delta_2 \cat u:\btout{\wtd C} S \proves \bout{u}{\wtd x} P \hastype \Proc
% 			}
% 	%		\\[4mm]
% 			\qquad 
% 			\inferrule[(PolyRcv)]{
% 			\begin{array}{c}
% 				\Gamma; \Delta_1 \cat u: S \proves P \hastype \Proc
% 				\quad
% 				\Gamma; \Delta_2 \proves {\wtd x} \hastype {\wtd C}
% 				\end{array}
% 			}{
% 				\Gamma \backslash \wtd x; \Delta_1 \setminus \Delta_2 \cat u: \btinp{\wtd C} S \vdash \binp{u}{{\wtd x}} P \hastype \Proc
% 			}
% 			\\[4mm]
% 			\inferrule[(PolyResS)]
% 			{\Gamma;\Delta \cat \wtd s:\wtd S_1 \cat  \wtd{\dual{s}}:\wtd S_2 \proves P \hastype \Proc
% 			\quad S_1 \dualof S_2}
% 			{\Gamma;\Delta \proves \news{\wtd s}P \hastype \Proc}
% 			\qquad 
% 			\inferrule[(PolyRes)]
% 			{\Gamma;\Delta \cat \wtd a:\wtd C  \proves P \hastype \Proc}
% 			{\Gamma;\Delta \proves \news{\wtd a}P \hastype \Proc}
% 			~~ 
% 			\\[4mm]
% 	%		\inferrule[(Sel)]
% 	%		{\Gamma;\Delta \cat u:S_j \proves P \hastype \Proc 
% 	%		\qquad j \in I}
% 	%		{\Gamma;\Delta \cat u: \btsel{l_i:S_i}_{i \in I} \proves 
% 	%		\bsel{u}{l_j}P \hastype \Proc}
% 	%		\\[4mm]
% 	%		\inferrule[(Bra)]
% 	%		{ \forall i \in I \qquad \Gamma;\Delta \cat u:S_i \proves P_i \hastype \Proc}
% 	%		{\Gamma;\Delta \cat u: \btbra{l_i:S_i}_{i \in I} \proves 
% 	%		\bbra{u}{l_i:P_i}_{i \in I}}
% 	%		~~\inferrule[(Par)]
% 	%		{\Gamma;\Delta_i \proves P_i \hastype \Proc \qquad i = 1,2}
% 	%		{\Gamma;\Delta_1 \cat \Delta_2 \proves P_1 \Par P_2 \hastype \Proc}
% 	%		\\[4mm] 
% 			\inferrule[(Req)]{
% 				\begin{array}{c}
% 					\Gamma;  \es \proves u \hastype \chtype{\wtd S}
% 					\quad
% 					\Gamma; \Delta_1 \proves P \hastype \Proc
% 					\\
% 					\Gamma;  \Delta_2 \proves \wtd x \hastype \wtd S
% 				\end{array}
% 			}{
% 				\Gamma;  \Delta_1 \cat \Delta_2 \proves \bout{u}{\wtd x} P \hastype \Proc
% 			}
% 			\qquad 
% 			\inferrule[(Acc)]{
% 				\begin{array}{c}
% 					\Gamma; \emptyset \proves u \hastype \chtype{\wtd S}
% 					\quad
% 					\Gamma;  \Delta_1 \proves P \hastype \Proc
% 					\\
% 					\Gamma; \Delta_2 \proves \wtd x \hastype \wtd S\\
% 					   \end{array}
% 			}{
% 				\Gamma\backslash \wtd x; \Delta_1 \setminus \Delta_2 \proves \binp{u}{\wtd x} P \hastype \Proc
% 			}
% 			\end{array}
% 	\]
% 	%\vspace{-3mm}
% 		\end{mdframed}
% 	\caption{Polyadic typing rules for $\pi$.
% 	%See~\cite{KouzapasPY17} for a full account.
% 	\label{top:fig:typerulesmyspoly}}
% 	%\Hline
% 	%\vspace{-1mm}
% 	\end{figure}
% 	\end{remark}




